Modeling Psychotherapy Dialogues with Kernelized Hashcode Representations: A Nonparametric Information-Theoretic Approach

We propose a novel dialogue modeling framework, the first-ever nonparametric kernel functions based approach for dialogue modeling, which learns kernelized hashcodes as compressed text representations; unlike traditional deep learning models, it handles well relatively small datasets, while also scaling to large ones. We also derive a novel lower bound on mutual information, used as a model-selection criterion favoring representations with better alignment between the utterances of participants in a collaborative dialogue setting, as well as higher predictability of the generated responses. As demonstrated on three real-life datasets, including prominently psychotherapy sessions, the proposed approach significantly outperforms several state-of-art neural network based dialogue systems, both in terms of computational efficiency, reducing training time from days or weeks to hours, and the response quality, achieving an order of magnitude improvement over competitors in frequency of being chosen as the best model by human evaluators.

==> MIResults.tex <==
{\color{red}

\input{tabHashDialogModelsCompare.tex}

\paragraph{Info-theoretic Metrics.}
Next, we took a deep dive into evaluation of hashing approaches with respect to how well they actually model the alignment between the responses 

%the performance of a kernel-hashing model varies for a random initialization of $\bs{S}^R$, we perform multiple trials in that case, and report numbers for the trial which gives the median value for MI LB.
% 	
For \emph{RkNN-Kernel} hashing, we vary sizes of the reference set $\bs{S}^R$, i.e. $M \in \{ 30, 100, 300\}$. For $M=30$, MI LB~(-11.5) and Entropy UB~(5.7) values are low when selecting the reference set elements randomly~(\emph{Random Selection}).
 
% also, the quality of hashcodes is poor~(Quality metric) for some of the trials partly due to the high redundancies between the hashcode bits~(TC Bound), and also from the low marginal entropies~(Marginal E.); inference is also poor across the five trials as the values for the marginal conditional entropy bound~(C.E. Bound) are not reduced enough compared to the marginal entropies. 
On the other hand, if the reference set is optimized~(\emph{MI LB Optimal}), MI LB~(4.4) and Entropy UB~(30.1) are of much higher values, as desired.
% 
% , and so is the case for the Quality and Inference metrics. Though, TC Bound remains of high value even with optimization of the reference; this is understandable as low value of $M$ can lead to high~(nonlinear) correlations/redundancies between the bits. Surprisingly the optimization leads to very high value for Marginal E., though C.E. Bound also remains high, thus leading to high value for Quality, yet relatively lower value for metric Inference. In the discussion below, we see that the latter two metrics (Quality and Inference) are more balanced w.r.t. each other for $M \in \{ 100, 300 \}$.
% 
% We find that accuracy metric is not as informative as the other proposed metrics for the evaluation. 
% 	
% 
% 	
% If the value of Inference metric is high, the performance of RF classifiers, over the random baseline also increases. For instance, for MI LB Opt, we have high value of Inference metric, compared to the random selection trials; correspondingly, the accuracy gap for MI LB Opt is also high compared to the Random trials.   
% 
% 
% \todo{talk about the accuracy metric, and the random baseline accuracy as well.}
% 
% 
% 
% \paragraph{Reference set of size 100}
% 
For $M=100$, MI LB values increase significantly compared to the values for $M=30$; thus high value of $M$ is advantageous. We see the benefits of optimizing the reference set~(MI LB: 13.6, Entropy UB: 26.2), compared to the Random Selection case~(MI LB: 9.8, Entropy UB: 19.9), for $M=100$ too.
% 
% For the case of random selection of reference set, the bound values vary significantly across the five trials while the optimized reference set leads to MI LB higher than what we obtain from most of the trials; same applies for the metrics, Quality and Inference. The total correlation between the bits is much lower for $M=100$, compared to $M=30$, as expected. Though the interesting part is that the optimization doesn't lead to a further decrease in the value of TC Bound but rather compensates through an increase in the marginal entropies, while maintaining similar values for C.E. Bound.
% 
% \paragraph{Reference set of size 300}
For a further increase in the size of the reference set, $M=300$, 
% that can be computationally expensive if responses contains thousands of words as observed for patient responses in the dataset, 
we obtain even higher values for MI LB~(15.7), though not a significant increase in Entropy UB~(24.0), especially when selecting the reference set randomly. In this setting, the advantage of optimizing the reference set is somewhat marginal.
% ~(MI LB increases from 15.2 to 15.7).
% compared to most of the random selection trials. 
For robustness, it is always good to optimize the set rather than a random selection. 
	
For \emph{kernel-RMM}, we use $M=100$, obtaining similar results as with kernel-RkNN hashing. Here it is interesting to see that the ratio of MI LB~(11.4) w.r.t. its baseline of MI LB for shuffled pairs~(2.8), is significantly higher~(4.1) than other models. This ratio should serve as another metric derived from MI LBs, to judge the quality of a dialogue model~(higher value of the ratio is better).
		
With an increase in $M$ when selecting the reference set randomly, we observe decrease in baseline accuracy since the Entropy UB increases in value. Also, when optimizing the reference set instead of Random selection, Entropy UB increases, and therefore the baseline accuracy decreases.  
Overall, when the difference between Entropy UB and MI LB~(quantifying inference quality) is high, the positive gap between the accuracy numbers and the baseline accuracy numbers is more significant. Variance for accuracy is high because for some bits in hashcodes, the distribution of 0s and 1s is imbalanced~(say, 99\%-1\%), making the inference very challenging for those bits.
% 
% data points assigned bit value 1).  
% 				
% \todo{talk about accuracy and the baseline accuracy}
% 
% \todo{talk about results for RMM.}
% 
% The random baseline accuracy numbers are highly correlated to the numbers for metric Marginal E., as expected.
% 
% , i.e., for high marginal entropies, the accuracy numbers drop.
% ; this is as expected. 
% The accuracy improvements of our RF classifiers over the corresponding baseline accuracy numbers
% % , that reflects how well the RF classifiers are performing in inferring the hashcode bits, 
% are correlated to Inference metric, as desired.
% 	        
% % \paragraph*{}
% Overall, as per the above discussions, from the greedy optimization of the reference set, we observe that MI LB increases with an increase in $M$, from 30 to 100, and up to 300; the gain is marginal for adding the 200 additional elements to the optimized set of 100 elements. 
% % The same marginal gain is seen for the case of random selection of reference set. 
% This suggests that MI LB may have submodular properties, justifying the greedy algorithmic choice, though theoretically formalizing such properties would be an independent work for the future.

Herein, it is also interesting to observe MI LB values for the ``Shuffled" setting~(presented in brackets), i.e. computing MI LB for random pairings of patient/therapist responses. This should serve as a good metric to analyze a hashing based dialogue model as well. Since we are modeling responses from all therapy sessions put together into a single set, one should expect that a good model should have low value of MI LB for the shuffled setting; though, it is natural to expect a minimal value of mutual information even between randomly paired responses of patient \& therapist, from different sessions, due to the common theme of depression psychotherapy across the sessions.


\subsubsection{Neural-Hashing}
% 
For the optimization of Neural-RLSTM hashing model, \algoref{alg:opt_nn_layers} gives a simple LSTM architecture of [16, 64, 16, 8], i.e. four layers, with 16 LSTM units in the first layer~(bottom layer receiving the inputs), 64 LSTM units in the second layer, and so on.
% 
% , across all the LSTM models~(hash functions). 
% 
% It is interesting to see that the algorithm picks a simple model of only two layers although the maximum limit on the number of layers is five, with maximum possible units 40. This can be attributed to the low number of training examples~($2\alpha$ samples are used for training each LSTM model as a hash function) for which a simple model suffices.
% 
% In \tabref{tab:results},  the optimized model is denoted as \emph{[20,20]-MI LB Opt}. 
For this model, we obtain relatively higher values for MI LB~(17.2), compared to the kernel-hashing above.
% although the improvement of accuracy~(58.1) over the accuracy of the baseline classifier~(54.5) is marginal. 
Besides the optimized architecture for LSTM models, we also tried manually built architectures; for instance, if using simple LSTM model of single layer with 10 units for each hash function, we obtain MI LB value, 6.7, that is significantly lower compared to the optimized Neural-RLSTM model~(17.2), and many of the kernel-hashing models above.
% 
% , baseline accuracy decreases with an increase in Entropy UB.
% 
% Besides the automated architecture selection above, we also fined tuned LSTM models manually, to architecture [10, 10], i.e. two layers with 10 units each. We obtain equally good results for this model as well. As a random selection, we also tried a simpler LSTM model, with single layer of 10 units~([10]), and observe much lower value of MI LB. 

% As we can see, when using a single layer LSTM of 10 units~([10]), MI LB is low, although the Entropy UB is still high. For LSTM of two layers with 10 units each~([10,10]), we obtain much higher value of MI LB, that is also higher than what we obtain with the kernel-hashing models discussed above. 


	
The above results demonstrate that our approach of optimizing hashing functions by maximizing our novel MI LB leads to higher values for the evaluation metrics as desired, across the kernel- as well as neural-hashing models.    
% 
There is a trade off between kernel-hashing and neural-hashing. In kernel-hashing, as per the selected responses in the optimized reference set, one can get insights on what patterns are relevant for a dialog; for e.g., see \tabref{tab:reference_responses}. On the other hand with neural-hashing, one can take advantage of the vast variety of neural language models available. 
% Overall, our approach of modeling dialog responses as binary hashcodes brings in a new perspective, that can be especially helpful for analyzing dialogues for complex domains such as psychotherapy. 

Further, 
% even though we provide results only for inferring hashcode for a therapist response, 
we can map an inferred hashcode to textual responses using a repository of indexed sentences. See \tabref{tab:gen_responses}.
	
\noindent{\bf Results on Larry King Dataset.\\}
Some selected results for the Larry King dataset are presented in \tabref{tab:results_larry_king}. Herein, it is interesting to see that we get very high value of MI LB, and Entropy UB with our neural hashing approach~(optimized architecture is [8,32]), in comparison to our kernel hashing. Also, mean accuracy with neural hashing is significantly higher than the baseline accuracy number. Though, NMI LB values for the two hashing approaches are relatively close.


\noindent{\bf Results on Twitter dataset.\\}
Optimized architure is [8, 32, 16].



  For Twitter dataset, we used  the    same setup for evaluation of our model as provided in \cite{serban2017hierarchical}, and compare with the results  published in that paper.
}


% \todo{MI for moving window of patient-therapist response pairs, for each session. MI should increase as the session goes. Consistent dynamic across sessions, globally. What are the pattersn ? Effect of therapy sessions ?}

% \todo{Discuss neural hashing results here.}   
    
% Although we use a greedy algorithm for the optimization, along with stochastic sampling for computing the bound as well the candidates selection in each greedy step, these are rather approximations with not concrete theoretical analysis to back up the approximations. So there is scope for improving the optimization procedures, while keeping the same MI LB and the evaluation metrics as we proposed in this paper. Further, the performance would be improvable via invention of better hashing models, be it kernels or neural networks based, etc.
% 	
% 
% From the above, one basic observation is that  the optimization algorithm for the reference set is very useful when the value of $$
% 
% 
% , for both the random selection and optimization of the reference set. 
% 
% \newpage
% \newpage
% - baseline comparisons
% 
% - random hashing
% 
% - other hashing algos
% 
% - aaai18 hashing optimizer
% 
% - random pairs as baseline
% 
% - time series on performance in a session
% 
% - pos count as baseline, suggested by Guille ?
% 
% - bigger picture, training therapists, evaluating therapists, some kind of metric to come up for the sessions
% 
% 
% \begin{table*}[tp!]
% \centering
% \scriptsize
% \renewcommand{\arraystretch}{0.8}% Tighter
% \renewcommand{\tabcolsep}{2.9pt}
% \begin{tabular}{lllllllllll}
% 		\toprule
% 		Configurations&Optimization&F1 Score&P&R&HD&MI&MI LB&M E&Neg TC LB&Neg M CE LB\\
%         \toprule
%         $M=30,\alpha=3$\\
%         \midrule
% &Random&$0.33\pm0.13$&$0.34\pm0.14$&$0.33\pm0.13$&$9.39\pm4.70$&$0.22\pm0.01$&$-4.12$&9.91&-1.56&-12.47\\
% &MI LB Opt*&$0.34\pm0.14$&$0.34\pm0.15$&$0.35\pm0.13$&$24.06\pm12.11$&$0.15\pm0.01$&-2.37&33.40&-10.19&-25.58\\        
% &MI Opt&$0.35\pm0.14$&$0.34\pm0.14$&$0.37\pm0.14$&$23.67\pm11.08$&$0.17\pm0.01$&-73.07&31.82&-8.64&-96.25\\
%        \toprule
%         $M=30,\alpha=10$\\
%         \midrule
% &Random&$0.39\pm0.11$&$0.35\pm0.12$&$0.47\pm0.08$&$27.14\pm12.70$&$0.48\pm0.02$&$-107.36$&27.67&-7.20&-127.82\\
% &MI LB Opt&$0.37\pm0.11$&$0.32\pm0.13$&$0.49\pm0.08$&$42.12\pm16.87$&$0.51\pm0.02$&-21.55&46.41&-14.23&-53.73\\
% &MI Opt&$0.38\pm0.14$&$0.34\pm0.15$&$0.46\pm0.10$&$24.33\pm13.29$&$0.18\pm0.02$&-40.61&24.91&-9.04&-56.48\\
% \toprule
% $M=100,\alpha=3$\\
% \midrule
% &Random&$0.25\pm0.12$&$0.31\pm0.12$&$0.22\pm0.13$&$22.14\pm10.64$&$0.14\pm0.01$&-14.24&37.97&-9.05&-43.16\\
% \toprule
% $M=100,\alpha=10$\\
% \midrule
% &Random&$0.29\pm0.14$&$0.33\pm0.14$&$0.28\pm0.14$&$19.52\pm9.85$&$0.05\pm0.01$&-17.29&30.43&-5.74&-41.98\\
% &MI LB Opt&$0.30\pm0.15$&$0.29\pm0.15$&$0.32\pm0.14$&$19.44\pm11.50$&$-0.13\pm\pm0.01$&-3.08&25.47&-5.27&-23.28\\
% &MI Opt&$0.30\pm0.14$&$0.29\pm0.14$&$0.33\pm0.12$&$22.22\pm14.50$&$-0.10\pm0.01$&-4.05&27.75&-6.49&-25.31\\
% \toprule
% $M=300,\alpha=3$\\
% \midrule
% &Random&$0.31\pm0.16$&$0.37\pm0.14$&$0.27\pm0.16$&$21.41\pm8.83$&$0.25\pm0.01$&$-34.08$&37.19&-7.14&-64.13\\
% \toprule
% $M=300,\alpha=10$\\
% \midrule
% &Random&$0.27\pm0.13$&$0.34\pm0.13$&$0.24\pm0.13$&$19.26\pm9.10$&$0.20\pm0.01$&-13.45&32.67&-5.55&-40.57\\
% \midrule
% &MI LB Opt&$0.29\pm0.14$&$0.30\pm0.15$&$0.29\pm0.13$&$19.90\pm10.69$&$-0.17\pm0.01$&3.13&30.01&-5.20&-21.68\\
% \midrule
% &MI Opt&$0.32\pm0.15$&$0.38\pm0.14$&$0.29\pm0.15$&$19.04\pm8.59$&$0.16\pm0.01$&9.93&31.63&-5.31&-16.39\\
% \toprule
% $M=1000,\alpha=3$\\
% \midrule		&Random&$0.26\pm0.14$&$0.35\pm0.14$&$0.22\pm0.14$&$19.52\pm9.25$&$0.19\pm0.01$&-34.60&34.09&-6.33&-62.36\\
% \toprule
% $M=1000,\alpha=10$\\
% \midrule		
% &Random&$0.26\pm0.17$&$0.33\pm0.14$&$0.23\pm0.17$&$17.91\pm8.97$&$0.09\pm0.01$&9.96&31.73&-5.74&-16.04\\
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation for Dialogues Hashcodes Inference with Our Model. Precision, Recall, F1 scores are weighted as per the binary class for each bit; mean, standard deviation statistics are obtained across all the bits. H=100, $\alpha=3$. *:rerun the optimizer as per new code. Number of samples, for computing estimates during the optimization, as well as the number of candidates samples in each greedy step, is 100.
% }
% \label{tab:results_pubmed45}
% \end{table*}
% 
% \begin{table*}[tp!]
% \centering
% \scriptsize
% \renewcommand{\arraystretch}{0.8}% Tighter
% % \renewcommand{\tabcolsep}{2.5pt}
% \begin{tabular}{lllllllllll}
% \toprule	Configurations&Optimization&Accuracy&MI&MI LB&Marginal E.&Neg TC LB&Neg Marginal C.E. LB\\
% \toprule
% $M=30$\\
% \midrule
% &Random&$0.86\pm0.17$~($0.82\pm0.20$)&-1.11&$-95.43$&27.67&-7.20&-115.90\\
% &MI LB Opt&$0.77\pm0.14$~($0.70\pm0.15$)&-0.90&-7.41&46.41&-14.23&-39.59\\
% &MI Opt&$0.84\pm0.18$~($0.88\pm0.16$)&$-0.98$&-27.55&24.91&-9.04&-43.42\\
% \toprule
% $M=100$\\
% \midrule
% &Random&$0.85\pm0.16$~($0.81\pm0.18)$&-0.31&-12.42&30.43&-5.74&-37.12\\
% &MI LB Opt&$0.89\pm0.14$~($0.85\pm0.16$)&-0.60&5.06&25.47&-5.27&-15.14\\
% &MI Opt&$0.87\pm0.15$~($0.83\pm0.17$)&-0.54&5.02&27.75&-6.49&-16.24\\
% \toprule
% $M=300$\\
% \midrule
% &Random&$0.84\pm0.16$~($0.79\pm0.19$)&-0.18&-9.42&32.67&-5.55&-36.54\\
% % \midrule
% &MI LB Opt&~$0.86\pm0.15$~($0.81\pm0.17$)&$-0.51$&9.61&30.01&-5.20&-15.20\\
% % \midrule
% &MI Opt&$0.84\pm0.18$~($0.80\pm0.20$)&$-0.11$&13.60&31.63&-5.31&-12.72\\
% \toprule
% $M=1000$\\
% \midrule		
% % &Baseline&\\
% &Random&$0.85\pm0.15$~($0.80\pm0.18$)&$-0.16$&13.70&31.73&-5.74&-12.29\\
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation for Dialogues Hashcodes Inference with Our Model. Precision, Recall, F1 scores are weighted as per the binary class for each bit; mean, standard deviation statistics are obtained across all the bits. H=100, $\alpha=10$. *:rerun the optimizer as per new code. Number of samples, for computing estimates during the optimization, as well as the number of candidates samples in each greedy step, is  100. Revised considering both classes, pos and neg, and removing some less relevant metrics. The accuracy numbers in the bracket are from inference purely as per the class distributions of the labels, while ignoring features.~\footnote{http://scikit-learn.org/stable/modules/generated/sklearn.dummy.DummyClassifier.html}
% }
% \label{tab:results_pubmed45}
% \end{table*}
% 
% 
% Ques to investigate: Can we think of ME-TC as a lower bound (or even upper bound) of the joint entropy ?
% 
% - besides the POS features, try Breadth first traversal of the Stanford dependencies, as well as, Abstract Meaning Representations.
% 
% - see if we can use the idea from this paper as a baseline: "Sketching Techniques for Large Scale NLP"
% 
% -\todo{Compare with other hashing algorithms as baseline}
% \todo{Compare with supervised kernel hashing algorithms somehow}
% 
% 

% \todo{See if results improve with bagging RF  based computation of lower bound}

% \subsubsection{Results with Various Kernel Hashing Algorithms}
% \begin{table*}[tp!]
% \centering
% % 
% \scriptsize
% % \tiny
% % \small
% % \renewcommand{\arraystretch}{0.8}% Tighter
% \renewcommand{\tabcolsep}{3pt}
% % 
% \begin{tabular}{lllllllllll}
% \toprule
% \textbf{Hashing Algo.}
% % ~(Optimization)
% &Accuracy~(Random Baseline Accuracy)&\textbf{MI LB}&Marginal E.&TC Bound&C.E. Bound&\textbf{Quality}&\textbf{Inference}\\
% % 
% \toprule
% $\gamma=100,\beta=100$&\\
% % 
% \toprule
% RMM&$69.15\pm11.84$~($61.24\pm10.73$)&$25.54\pm0.43$&$56.99\pm0.19$&$14.10\pm0.29$&$17.35\pm0.30$\\
% % &$\pm$&$\pm$\\
% % 
% % 
% kNN~(one subset)&$90.79\pm13.88$~($87.89\pm15.92$)&$6.00\pm0.19$&$20.28\pm0.22$&$4.41\pm0.24$&$9.88\pm0.18$\\
% % 
% kNN~(two subsets)&$86.50\pm14.96$~($82.33\pm16.76$)&$10.57\pm0.39$&$28.63\pm0.17$&$5.45\pm0.26$&$12.60\pm0.29$\\
% % 
% % 
% \toprule
% $\gamma=100,\beta=1000$&\\
% % 
% \toprule
% RMM&$73.55\pm11.36$~($65.00\pm11.08$)&$21.72\pm0.89$&$52.85\pm0.23$&$14.32\pm0.68$&$16.82\pm0.40$\\
% % &$\pm$&$\pm$\\
% % 
% kNN (two subsets)&$82.74\pm16.15$~($78.35\pm17.30$)&$13.58\pm0.45$
% &$34.42\pm0.20$&$8.22\pm0.35$&$12.63\pm0.29$
% &$26.20\pm0.40$&$21.79\pm0.35$\\
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation for our approach of inferring dialog responses as hashcodes. All models optimized using the MI LB, with configurations $\beta=100, \gamma=100, M=100$.}
% \label{tab:results}
% \end{table*}

% \todo{implement KLSH, optimized, for M=100.}

% \todo{implement random maximum margin, optimized, for M=100.}

% \todo{see the effect if we split the random subset of the reference set into half, instead of sampling two. We can not repeat experiments, however an empirical analysis would be nice.}
	
    
% \todo{See if we can show responses generated by other models as well.}   	
% \todo{show generated therapist textual responses}

% \subsection{Analyzing Mutual Information Across Sessions}

% \todo{MI Lower bound across 407 sessions, using the optimized neural and kernel hash models}

% \todo{Compute MI lower bound across the 407 sessions, using word vectors based sentence embeddings.}

% 

==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/MIResults.tex <==
{\color{red}

\input{tabHashDialogModelsCompare.tex}

\paragraph{Info-theoretic Metrics.}
Next, we took a deep dive into evaluation of hashing approaches with respect to how well they actually model the alignment between the responses 

%the performance of a kernel-hashing model varies for a random initialization of $\bs{S}^R$, we perform multiple trials in that case, and report numbers for the trial which gives the median value for MI LB.
% 	
For \emph{RkNN-Kernel} hashing, we vary sizes of the reference set $\bs{S}^R$, i.e. $M \in \{ 30, 100, 300\}$. For $M=30$, MI LB~(-11.5) and Entropy UB~(5.7) values are low when selecting the reference set elements randomly~(\emph{Random Selection}).
 
% also, the quality of hashcodes is poor~(Quality metric) for some of the trials partly due to the high redundancies between the hashcode bits~(TC Bound), and also from the low marginal entropies~(Marginal E.); inference is also poor across the five trials as the values for the marginal conditional entropy bound~(C.E. Bound) are not reduced enough compared to the marginal entropies. 
On the other hand, if the reference set is optimized~(\emph{MI LB Optimal}), MI LB~(4.4) and Entropy UB~(30.1) are of much higher values, as desired.
% 
% , and so is the case for the Quality and Inference metrics. Though, TC Bound remains of high value even with optimization of the reference; this is understandable as low value of $M$ can lead to high~(nonlinear) correlations/redundancies between the bits. Surprisingly the optimization leads to very high value for Marginal E., though C.E. Bound also remains high, thus leading to high value for Quality, yet relatively lower value for metric Inference. In the discussion below, we see that the latter two metrics (Quality and Inference) are more balanced w.r.t. each other for $M \in \{ 100, 300 \}$.
% 
% We find that accuracy metric is not as informative as the other proposed metrics for the evaluation. 
% 	
% 
% 	
% If the value of Inference metric is high, the performance of RF classifiers, over the random baseline also increases. For instance, for MI LB Opt, we have high value of Inference metric, compared to the random selection trials; correspondingly, the accuracy gap for MI LB Opt is also high compared to the Random trials.   
% 
% 
% \todo{talk about the accuracy metric, and the random baseline accuracy as well.}
% 
% 
% 
% \paragraph{Reference set of size 100}
% 
For $M=100$, MI LB values increase significantly compared to the values for $M=30$; thus high value of $M$ is advantageous. We see the benefits of optimizing the reference set~(MI LB: 13.6, Entropy UB: 26.2), compared to the Random Selection case~(MI LB: 9.8, Entropy UB: 19.9), for $M=100$ too.
% 
% For the case of random selection of reference set, the bound values vary significantly across the five trials while the optimized reference set leads to MI LB higher than what we obtain from most of the trials; same applies for the metrics, Quality and Inference. The total correlation between the bits is much lower for $M=100$, compared to $M=30$, as expected. Though the interesting part is that the optimization doesn't lead to a further decrease in the value of TC Bound but rather compensates through an increase in the marginal entropies, while maintaining similar values for C.E. Bound.
% 
% \paragraph{Reference set of size 300}
For a further increase in the size of the reference set, $M=300$, 
% that can be computationally expensive if responses contains thousands of words as observed for patient responses in the dataset, 
we obtain even higher values for MI LB~(15.7), though not a significant increase in Entropy UB~(24.0), especially when selecting the reference set randomly. In this setting, the advantage of optimizing the reference set is somewhat marginal.
% ~(MI LB increases from 15.2 to 15.7).
% compared to most of the random selection trials. 
For robustness, it is always good to optimize the set rather than a random selection. 
	
For \emph{kernel-RMM}, we use $M=100$, obtaining similar results as with kernel-RkNN hashing. Here it is interesting to see that the ratio of MI LB~(11.4) w.r.t. its baseline of MI LB for shuffled pairs~(2.8), is significantly higher~(4.1) than other models. This ratio should serve as another metric derived from MI LBs, to judge the quality of a dialogue model~(higher value of the ratio is better).
		
With an increase in $M$ when selecting the reference set randomly, we observe decrease in baseline accuracy since the Entropy UB increases in value. Also, when optimizing the reference set instead of Random selection, Entropy UB increases, and therefore the baseline accuracy decreases.  
Overall, when the difference between Entropy UB and MI LB~(quantifying inference quality) is high, the positive gap between the accuracy numbers and the baseline accuracy numbers is more significant. Variance for accuracy is high because for some bits in hashcodes, the distribution of 0s and 1s is imbalanced~(say, 99\%-1\%), making the inference very challenging for those bits.
% 
% data points assigned bit value 1).  
% 				
% \todo{talk about accuracy and the baseline accuracy}
% 
% \todo{talk about results for RMM.}
% 
% The random baseline accuracy numbers are highly correlated to the numbers for metric Marginal E., as expected.
% 
% , i.e., for high marginal entropies, the accuracy numbers drop.
% ; this is as expected. 
% The accuracy improvements of our RF classifiers over the corresponding baseline accuracy numbers
% % , that reflects how well the RF classifiers are performing in inferring the hashcode bits, 
% are correlated to Inference metric, as desired.
% 	        
% % \paragraph*{}
% Overall, as per the above discussions, from the greedy optimization of the reference set, we observe that MI LB increases with an increase in $M$, from 30 to 100, and up to 300; the gain is marginal for adding the 200 additional elements to the optimized set of 100 elements. 
% % The same marginal gain is seen for the case of random selection of reference set. 
% This suggests that MI LB may have submodular properties, justifying the greedy algorithmic choice, though theoretically formalizing such properties would be an independent work for the future.

Herein, it is also interesting to observe MI LB values for the ``Shuffled" setting~(presented in brackets), i.e. computing MI LB for random pairings of patient/therapist responses. This should serve as a good metric to analyze a hashing based dialogue model as well. Since we are modeling responses from all therapy sessions put together into a single set, one should expect that a good model should have low value of MI LB for the shuffled setting; though, it is natural to expect a minimal value of mutual information even between randomly paired responses of patient \& therapist, from different sessions, due to the common theme of depression psychotherapy across the sessions.


\subsubsection{Neural-Hashing}
% 
For the optimization of Neural-RLSTM hashing model, \algoref{alg:opt_nn_layers} gives a simple LSTM architecture of [16, 64, 16, 8], i.e. four layers, with 16 LSTM units in the first layer~(bottom layer receiving the inputs), 64 LSTM units in the second layer, and so on.
% 
% , across all the LSTM models~(hash functions). 
% 
% It is interesting to see that the algorithm picks a simple model of only two layers although the maximum limit on the number of layers is five, with maximum possible units 40. This can be attributed to the low number of training examples~($2\alpha$ samples are used for training each LSTM model as a hash function) for which a simple model suffices.
% 
% In \tabref{tab:results},  the optimized model is denoted as \emph{[20,20]-MI LB Opt}. 
For this model, we obtain relatively higher values for MI LB~(17.2), compared to the kernel-hashing above.
% although the improvement of accuracy~(58.1) over the accuracy of the baseline classifier~(54.5) is marginal. 
Besides the optimized architecture for LSTM models, we also tried manually built architectures; for instance, if using simple LSTM model of single layer with 10 units for each hash function, we obtain MI LB value, 6.7, that is significantly lower compared to the optimized Neural-RLSTM model~(17.2), and many of the kernel-hashing models above.
% 
% , baseline accuracy decreases with an increase in Entropy UB.
% 
% Besides the automated architecture selection above, we also fined tuned LSTM models manually, to architecture [10, 10], i.e. two layers with 10 units each. We obtain equally good results for this model as well. As a random selection, we also tried a simpler LSTM model, with single layer of 10 units~([10]), and observe much lower value of MI LB. 

% As we can see, when using a single layer LSTM of 10 units~([10]), MI LB is low, although the Entropy UB is still high. For LSTM of two layers with 10 units each~([10,10]), we obtain much higher value of MI LB, that is also higher than what we obtain with the kernel-hashing models discussed above. 


	
The above results demonstrate that our approach of optimizing hashing functions by maximizing our novel MI LB leads to higher values for the evaluation metrics as desired, across the kernel- as well as neural-hashing models.    
% 
There is a trade off between kernel-hashing and neural-hashing. In kernel-hashing, as per the selected responses in the optimized reference set, one can get insights on what patterns are relevant for a dialog; for e.g., see \tabref{tab:reference_responses}. On the other hand with neural-hashing, one can take advantage of the vast variety of neural language models available. 
% Overall, our approach of modeling dialog responses as binary hashcodes brings in a new perspective, that can be especially helpful for analyzing dialogues for complex domains such as psychotherapy. 

Further, 
% even though we provide results only for inferring hashcode for a therapist response, 
we can map an inferred hashcode to textual responses using a repository of indexed sentences. See \tabref{tab:gen_responses}.
	
\noindent{\bf Results on Larry King Dataset.\\}
Some selected results for the Larry King dataset are presented in \tabref{tab:results_larry_king}. Herein, it is interesting to see that we get very high value of MI LB, and Entropy UB with our neural hashing approach~(optimized architecture is [8,32]), in comparison to our kernel hashing. Also, mean accuracy with neural hashing is significantly higher than the baseline accuracy number. Though, NMI LB values for the two hashing approaches are relatively close.


\noindent{\bf Results on Twitter dataset.\\}
Optimized architure is [8, 32, 16].



  For Twitter dataset, we used  the    same setup for evaluation of our model as provided in \cite{serban2017hierarchical}, and compare with the results  published in that paper.
}


% \todo{MI for moving window of patient-therapist response pairs, for each session. MI should increase as the session goes. Consistent dynamic across sessions, globally. What are the pattersn ? Effect of therapy sessions ?}

% \todo{Discuss neural hashing results here.}   
    
% Although we use a greedy algorithm for the optimization, along with stochastic sampling for computing the bound as well the candidates selection in each greedy step, these are rather approximations with not concrete theoretical analysis to back up the approximations. So there is scope for improving the optimization procedures, while keeping the same MI LB and the evaluation metrics as we proposed in this paper. Further, the performance would be improvable via invention of better hashing models, be it kernels or neural networks based, etc.
% 	
% 
% From the above, one basic observation is that  the optimization algorithm for the reference set is very useful when the value of $$
% 
% 
% , for both the random selection and optimization of the reference set. 
% 
% \newpage
% \newpage
% - baseline comparisons
% 
% - random hashing
% 
% - other hashing algos
% 
% - aaai18 hashing optimizer
% 
% - random pairs as baseline
% 
% - time series on performance in a session
% 
% - pos count as baseline, suggested by Guille ?
% 
% - bigger picture, training therapists, evaluating therapists, some kind of metric to come up for the sessions
% 
% 
% \begin{table*}[tp!]
% \centering
% \scriptsize
% \renewcommand{\arraystretch}{0.8}% Tighter
% \renewcommand{\tabcolsep}{2.9pt}
% \begin{tabular}{lllllllllll}
% 		\toprule
% 		Configurations&Optimization&F1 Score&P&R&HD&MI&MI LB&M E&Neg TC LB&Neg M CE LB\\
%         \toprule
%         $M=30,\alpha=3$\\
%         \midrule
% &Random&$0.33\pm0.13$&$0.34\pm0.14$&$0.33\pm0.13$&$9.39\pm4.70$&$0.22\pm0.01$&$-4.12$&9.91&-1.56&-12.47\\
% &MI LB Opt*&$0.34\pm0.14$&$0.34\pm0.15$&$0.35\pm0.13$&$24.06\pm12.11$&$0.15\pm0.01$&-2.37&33.40&-10.19&-25.58\\        
% &MI Opt&$0.35\pm0.14$&$0.34\pm0.14$&$0.37\pm0.14$&$23.67\pm11.08$&$0.17\pm0.01$&-73.07&31.82&-8.64&-96.25\\
%        \toprule
%         $M=30,\alpha=10$\\
%         \midrule
% &Random&$0.39\pm0.11$&$0.35\pm0.12$&$0.47\pm0.08$&$27.14\pm12.70$&$0.48\pm0.02$&$-107.36$&27.67&-7.20&-127.82\\
% &MI LB Opt&$0.37\pm0.11$&$0.32\pm0.13$&$0.49\pm0.08$&$42.12\pm16.87$&$0.51\pm0.02$&-21.55&46.41&-14.23&-53.73\\
% &MI Opt&$0.38\pm0.14$&$0.34\pm0.15$&$0.46\pm0.10$&$24.33\pm13.29$&$0.18\pm0.02$&-40.61&24.91&-9.04&-56.48\\
% \toprule
% $M=100,\alpha=3$\\
% \midrule
% &Random&$0.25\pm0.12$&$0.31\pm0.12$&$0.22\pm0.13$&$22.14\pm10.64$&$0.14\pm0.01$&-14.24&37.97&-9.05&-43.16\\
% \toprule
% $M=100,\alpha=10$\\
% \midrule
% &Random&$0.29\pm0.14$&$0.33\pm0.14$&$0.28\pm0.14$&$19.52\pm9.85$&$0.05\pm0.01$&-17.29&30.43&-5.74&-41.98\\
% &MI LB Opt&$0.30\pm0.15$&$0.29\pm0.15$&$0.32\pm0.14$&$19.44\pm11.50$&$-0.13\pm\pm0.01$&-3.08&25.47&-5.27&-23.28\\
% &MI Opt&$0.30\pm0.14$&$0.29\pm0.14$&$0.33\pm0.12$&$22.22\pm14.50$&$-0.10\pm0.01$&-4.05&27.75&-6.49&-25.31\\
% \toprule
% $M=300,\alpha=3$\\
% \midrule
% &Random&$0.31\pm0.16$&$0.37\pm0.14$&$0.27\pm0.16$&$21.41\pm8.83$&$0.25\pm0.01$&$-34.08$&37.19&-7.14&-64.13\\
% \toprule
% $M=300,\alpha=10$\\
% \midrule
% &Random&$0.27\pm0.13$&$0.34\pm0.13$&$0.24\pm0.13$&$19.26\pm9.10$&$0.20\pm0.01$&-13.45&32.67&-5.55&-40.57\\
% \midrule
% &MI LB Opt&$0.29\pm0.14$&$0.30\pm0.15$&$0.29\pm0.13$&$19.90\pm10.69$&$-0.17\pm0.01$&3.13&30.01&-5.20&-21.68\\
% \midrule
% &MI Opt&$0.32\pm0.15$&$0.38\pm0.14$&$0.29\pm0.15$&$19.04\pm8.59$&$0.16\pm0.01$&9.93&31.63&-5.31&-16.39\\
% \toprule
% $M=1000,\alpha=3$\\
% \midrule		&Random&$0.26\pm0.14$&$0.35\pm0.14$&$0.22\pm0.14$&$19.52\pm9.25$&$0.19\pm0.01$&-34.60&34.09&-6.33&-62.36\\
% \toprule
% $M=1000,\alpha=10$\\
% \midrule		
% &Random&$0.26\pm0.17$&$0.33\pm0.14$&$0.23\pm0.17$&$17.91\pm8.97$&$0.09\pm0.01$&9.96&31.73&-5.74&-16.04\\
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation for Dialogues Hashcodes Inference with Our Model. Precision, Recall, F1 scores are weighted as per the binary class for each bit; mean, standard deviation statistics are obtained across all the bits. H=100, $\alpha=3$. *:rerun the optimizer as per new code. Number of samples, for computing estimates during the optimization, as well as the number of candidates samples in each greedy step, is 100.
% }
% \label{tab:results_pubmed45}
% \end{table*}
% 
% \begin{table*}[tp!]
% \centering
% \scriptsize
% \renewcommand{\arraystretch}{0.8}% Tighter
% % \renewcommand{\tabcolsep}{2.5pt}
% \begin{tabular}{lllllllllll}
% \toprule	Configurations&Optimization&Accuracy&MI&MI LB&Marginal E.&Neg TC LB&Neg Marginal C.E. LB\\
% \toprule
% $M=30$\\
% \midrule
% &Random&$0.86\pm0.17$~($0.82\pm0.20$)&-1.11&$-95.43$&27.67&-7.20&-115.90\\
% &MI LB Opt&$0.77\pm0.14$~($0.70\pm0.15$)&-0.90&-7.41&46.41&-14.23&-39.59\\
% &MI Opt&$0.84\pm0.18$~($0.88\pm0.16$)&$-0.98$&-27.55&24.91&-9.04&-43.42\\
% \toprule
% $M=100$\\
% \midrule
% &Random&$0.85\pm0.16$~($0.81\pm0.18)$&-0.31&-12.42&30.43&-5.74&-37.12\\
% &MI LB Opt&$0.89\pm0.14$~($0.85\pm0.16$)&-0.60&5.06&25.47&-5.27&-15.14\\
% &MI Opt&$0.87\pm0.15$~($0.83\pm0.17$)&-0.54&5.02&27.75&-6.49&-16.24\\
% \toprule
% $M=300$\\
% \midrule
% &Random&$0.84\pm0.16$~($0.79\pm0.19$)&-0.18&-9.42&32.67&-5.55&-36.54\\
% % \midrule
% &MI LB Opt&~$0.86\pm0.15$~($0.81\pm0.17$)&$-0.51$&9.61&30.01&-5.20&-15.20\\
% % \midrule
% &MI Opt&$0.84\pm0.18$~($0.80\pm0.20$)&$-0.11$&13.60&31.63&-5.31&-12.72\\
% \toprule
% $M=1000$\\
% \midrule		
% % &Baseline&\\
% &Random&$0.85\pm0.15$~($0.80\pm0.18$)&$-0.16$&13.70&31.73&-5.74&-12.29\\
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation for Dialogues Hashcodes Inference with Our Model. Precision, Recall, F1 scores are weighted as per the binary class for each bit; mean, standard deviation statistics are obtained across all the bits. H=100, $\alpha=10$. *:rerun the optimizer as per new code. Number of samples, for computing estimates during the optimization, as well as the number of candidates samples in each greedy step, is  100. Revised considering both classes, pos and neg, and removing some less relevant metrics. The accuracy numbers in the bracket are from inference purely as per the class distributions of the labels, while ignoring features.~\footnote{http://scikit-learn.org/stable/modules/generated/sklearn.dummy.DummyClassifier.html}
% }
% \label{tab:results_pubmed45}
% \end{table*}
% 
% 
% Ques to investigate: Can we think of ME-TC as a lower bound (or even upper bound) of the joint entropy ?
% 
% - besides the POS features, try Breadth first traversal of the Stanford dependencies, as well as, Abstract Meaning Representations.
% 
% - see if we can use the idea from this paper as a baseline: "Sketching Techniques for Large Scale NLP"
% 
% -\todo{Compare with other hashing algorithms as baseline}
% \todo{Compare with supervised kernel hashing algorithms somehow}
% 
% 

% \todo{See if results improve with bagging RF  based computation of lower bound}

% \subsubsection{Results with Various Kernel Hashing Algorithms}
% \begin{table*}[tp!]
% \centering
% % 
% \scriptsize
% % \tiny
% % \small
% % \renewcommand{\arraystretch}{0.8}% Tighter
% \renewcommand{\tabcolsep}{3pt}
% % 
% \begin{tabular}{lllllllllll}
% \toprule
% \textbf{Hashing Algo.}
% % ~(Optimization)
% &Accuracy~(Random Baseline Accuracy)&\textbf{MI LB}&Marginal E.&TC Bound&C.E. Bound&\textbf{Quality}&\textbf{Inference}\\
% % 
% \toprule
% $\gamma=100,\beta=100$&\\
% % 
% \toprule
% RMM&$69.15\pm11.84$~($61.24\pm10.73$)&$25.54\pm0.43$&$56.99\pm0.19$&$14.10\pm0.29$&$17.35\pm0.30$\\
% % &$\pm$&$\pm$\\
% % 
% % 
% kNN~(one subset)&$90.79\pm13.88$~($87.89\pm15.92$)&$6.00\pm0.19$&$20.28\pm0.22$&$4.41\pm0.24$&$9.88\pm0.18$\\
% % 
% kNN~(two subsets)&$86.50\pm14.96$~($82.33\pm16.76$)&$10.57\pm0.39$&$28.63\pm0.17$&$5.45\pm0.26$&$12.60\pm0.29$\\
% % 
% % 
% \toprule
% $\gamma=100,\beta=1000$&\\
% % 
% \toprule
% RMM&$73.55\pm11.36$~($65.00\pm11.08$)&$21.72\pm0.89$&$52.85\pm0.23$&$14.32\pm0.68$&$16.82\pm0.40$\\
% % &$\pm$&$\pm$\\
% % 
% kNN (two subsets)&$82.74\pm16.15$~($78.35\pm17.30$)&$13.58\pm0.45$
% &$34.42\pm0.20$&$8.22\pm0.35$&$12.63\pm0.29$
% &$26.20\pm0.40$&$21.79\pm0.35$\\
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation for our approach of inferring dialog responses as hashcodes. All models optimized using the MI LB, with configurations $\beta=100, \gamma=100, M=100$.}
% \label{tab:results}
% \end{table*}

% \todo{implement KLSH, optimized, for M=100.}

% \todo{implement random maximum margin, optimized, for M=100.}

% \todo{see the effect if we split the random subset of the reference set into half, instead of sampling two. We can not repeat experiments, however an empirical analysis would be nice.}
	
    
% \todo{See if we can show responses generated by other models as well.}   	
% \todo{show generated therapist textual responses}

% \subsection{Analyzing Mutual Information Across Sessions}

% \todo{MI Lower bound across 407 sessions, using the optimized neural and kernel hash models}

% \todo{Compute MI lower bound across the 407 sessions, using word vectors based sentence embeddings.}

% 

==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/algo_ngrams_text_gen.tex <==
\begin{algorithm*}[tp!]
\caption{Response Generation via Hashing of N-grams}
% 
\begin{algorithmic}[1]
\REQUIRE Therapist response sentences from the training set, $\bs{S}^t$ and their hashcodes, $\bs{C^t}$; N-grams from the training set, $\bs{S^g}$, and their hashcodes, $\bs{C^g}$; an inferred therapist hashcode, $\bs{c^t_*}$.
%
\STATE $S^t \gets$ samplePrefix($\bs{c^t_*}, \bs{C^t, \bs{S}^t}$)
%
\COMMENT{sampling from therapist responses matching the inferred therapist hashcode.}
% 
\WHILE{True}
% 
\STATE $S^g \gets$ extractSuffixAsNgram($S^t$)
%\COMMENT{An Ngram is extracted from suffix of the generated response.}
\\
% 
\algshade{
\STATE $\bs{c}^g \gets$ computeHashcodeOfNgram($S^g$)
%\COMMENT{Hashcode of the N-gram, using an unsupervised hashing model.}
% 
\STATE $w^g \gets$ inferNextToken($\bs{c}^g, \bs{C^g}$)
\COMMENT{for an Ngram, there are tokens to follow as suffix along with the probabilities. Tokens from all the relevant N-Grams in the training set, matched via hashcodes, are aggregated for sampling.}
}
% 
\STATE $S^t \gets$ appendTokenToResponse($S^t, w^g$)
%\COMMENT{Append the sampled token to the response.}
\\
% 
\algshade{
\STATE $\bs{c}^t \gets$ computeHashcodeOfResponse($S^t$)
%\COMMENT{Hashcode of response using the dialog hashing model.}
% 
\STATE $f^t \gets$ computeLikelihood($\bs{c}^t, \bs{c}^t_*, \bs{C^t}$)
% 
\COMMENT{likelihood per the responses in training set matched via hashcodes, and  hamming distance w.r.t. the inferred hashcode.}
}
% 
\IF{$f^t$ is high}
\RETURN $S^t, f^t$
\COMMENT{return the therapist response.}
\ELSIF{$f^g$ is very low}
\algshade{
\STATE $S^t \gets$ backtrack($S^t$)
\COMMENT{Some of the tokens in the suffix are removed from the response.}
}
\ENDIF
\ENDWHILE
\end{algorithmic}
\label{alg:response_generation}
\end{algorithm*}


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/background.tex <==
% \vspace{-0.1in}
\section{
Dialog Modeling via Kernelized Hashcode Representations
% Problem Formulation and  Background
}
% 
We now present a novel framework for  dialogue modeling using binary hash functions. We will refer to the two dialogue agents as to a patient and a therapist, respectively, although the approach is generally applicable to a wider  variety of dialogue settings, as demonstrated later in the empirical section on datasets such as TV show interviews and Twitter dialogues.

\subsection{Problem Formulation and Approach Overview}
% 
We consider a dialogue dataset consisting of $N$ samples, $\bs{S}^{pt} = \{ S_i^p, S_i^t \}_{i=1}^N$, where each sample is a pair of a patient  and a therapist responses,  $S_i^p$ and $S_i^t$, respectively; we will also use the following notation: $\bs{\bar{S}}= \{ S_1^p, \cdots, S_N^p, S_1^t, \cdots, S_N^t \}$, $\bs{S}^p= \{ S_1^p, \cdots, S_N^p \}$, $\bs{S}^t= \{ S_1^t, \cdots, S_N^t \}$. Each response is a natural language structure which can be simply a text, or a text   with part of speech tags (PoS), or a syntactic/semantic parsing of the text. 

    
Given response  $S_i^p$, the dialogue generation task is  to  produce the  response $S_i^t$. We approach this task as a three-stage problem: first, we learn a representation model, based on {\em locality sensitive hashing}, which maps each text response $S_i$ into some binary hashcode  vector   $\bs{c}_i  \in \{0, 1\}^{H}$; second, we train a classifier to infer   the therapist's hashcode $\bs{c}_i^{t*}$ given the patient's hashcode $\bs{c}_i^p$, so that the inference takes place in the abstract representation space; \emph{hashcode representation  aims   at capturing, in a compressed form, the semantic essence of the responses while leaving out irrelevant details}; finally, we produce a   textual response based on the predicted hashcode representation.
% 
% \footnote{As mentioned earlier,  we   simply   choose the nearest hashcode based on training samples ~(sublinear  algorithms can be used for efficient similarity search   in hamming spaces~\cite{norouzi2014fast,komorowski2017random}); 
% alternatives  include  various unsupervised   generative  generation model, e.g. \cite{bowman2015generating,jozefowicz2016exploring,semeniuta2017hybrid,yu2017seqgan}.}.
    
Our objective is to choose  a hashcode-based text representation model %essence of our approach is to select hashing-based representation  models, from a large model space determined by multitude of hyper-parameters described later,
so that consecutive responses of the dialogue participants are maximally relevant to each other,  as measured by the  mutual information between the corresponding hashcode representations; from another perspective, this will also make the response of the  second's person   more predictable given the first person's response. %, i.e. we prefer representations which 
% (see Figure \ref{fig:klsh_max_mi}). 
%From another perspective, this  objective is also aimed at learning representations making the second response maximally predictable given the first response. 
    

\subsection{Background: Kernelized Locality Sensitive Hashing}
\label{sec:lsh}
% 
The main idea behind locality sensitive hashing is that, data points which are similar to each other as per some features, are assigned hashcodes within a short Hamming distance to each other, and vice versa  \cite{grauman2013learning,zhao2014locality,wang2017survey}. Such hashcodes can be used as  generalized representations of language structures, e.g. responses of dialogue participants.
%Since locality sensitive hashing ensures that natural language structures, that are assigned hashcodes with low hamming distance to each other, are similar to each other, locality sensitive hashcodes should serve as generalized representations of language structures~(a similarity/distance function implied as per the locality sensitive hashing model learned for a given task),
% ~\footnote{A similarity function doesn't imply a semantic similarity function here. For instance, as per a learned locality sensitive hashing model, the implied (valid) similarity function may account for matching of only certain patterns in textual responses.}, 
%and so for the responses in a dialogue.
There are multiple  hash functions   proven to be locality sensitive \cite{wang2017survey}. Kernelized locality-sensitive hashing approaches have also been developed~\cite{kulis2009kernelized,joly2011random}, which are recently shown to be applicable for learning representations of natural language \cite{garg2018efficient,garg2019nearly}. These techniques rely  on a convolution kernel similarity  function $K(S_i,S_j; \bs{\theta})$ defined for any pair of structures $S_i$ and $S_j$ with kernel parameters $\bs{\theta}$ \cite{srivastava2013walk,mooney2005subsequence,haussler1999convolution}. 
% 
% Note that the approach of kernelized hashcodes, despite its low computational cost, is not meant to be used just as an approximate alternative to the traditional kernel-methods. Rather, it offers a novel paradigm for learning nonparameteric representations of text, shown to outperform methods like kernel-SVM, kernel-kNN, for information extraction tasks~\cite{garg2018efficient,garg2019nearly}. While the traditional kernel-methods suffer from the issue of computing similarities accounting for all the patterns in text including non-relevant ones~(noise), hashcodes can be optimized intelligently for capturing similarities only based on relevant patterns.
% 
% , in an information theoretic manner.
% 
% 
% see the supplementary materials for more details.

    
% \begin{figure}[tp!]
% \centering
% \includegraphics[width=0.9\columnwidth]{Slide02.png}
% \label{fig:hash_app}
% \vspace{-3.5mm}
% \caption{
% \csizenine
% An illustration of RMM technique, using max-margin (kernel-SVM) classifiers to learn a collection of hash functions, each determined by a particular random split of the reference set into positive (red) and negative (blue) samples.}
% \vspace{-3.75mm}
% \label{fig:klsh_eg}
% \end{figure}

In order to construct hash functions for  mapping textual responses to   hashcodes,   we will first select from a training dataset a random subset of text structures (responses) $\bs{S}^R \subset \bs{\bar{S}}$ of size $|\bs{S}^R|=M$, called a {\em reference set}. Further, let $h_l(S_i)$, $l=1,\cdots, H$, denote a set of $H$ binary-valued hash functions, and  
let $\bs{h}(S_i)$ denote  vector $\{h_l(S_i)\}_{l=1}^H$.  The hashcode representation of response $S_i$ will be given as $\bs{c}_i=\bs{h}(S_i)$. 
    
To generate a hash function $h_l(S_i)$, for each bit $l$, we first select a random  subset  $\bs{S}^R_l \subset \bs{S}^{R}$ of the reference set,  $|\bs{S}^R_l|=2\alpha$. Next, we assign label 0 to $\alpha$ randomly selected elements of $\bs{S}^R_l$, and label 1 to the remaining $\alpha$ elements of that set, creating an artificial binary-labeled training dataset~\footnote{For a more sophisticated methodology to assign the artificial binary labels, and to select the random subsets of $\bs{S}^{R}$, refer to the recent work by \cite{garg2019nearly}.}, which can be now fed into any binary classifier to learn a function $h_l(S_i)$. 
% 
% For example, \figref{fig:klsh_eg} illustrates this approach using the   Random Maximum Margin~({\em LSH-RMM}) method \cite{joly2011random}, where maximum-margin classifier (SVM) is applied to random splits of the reference set into blue (label 0) and red (label 1) points, respectively. 
% 
We generate $H$ such random splits of the reference set, and learn the corresponding $H$ binary classifiers, as hash functions. We also tried  kernelized k-nearest neighbor classifier (kNN),  resulting into hashing approach  we refer to as {\em LSH-RkNN}.
  
        
Overall, to obtain a hashcode of a given response $S_i$,  we must compute $M$  kernel similarities, $K(S_i, S_j),  \forall S_j \in \bs{S}
^R$. For a limited  size~($M$) of the reference set $\bs{S}^R$,  hashcodes can be computed  efficiently, with the computational cost linear in $H$; also, note that LSH techniques described above are easily  parallelizable.
% ~\footnote{One can also use other kernel based classifiers like Gaussian processes~\cite{rasmussen2006gaussian} to build hash functions within LSH. The approach of \cite{kulis2009kernelized} also comes under the same LSH framework. In their work, a hash function $h_l(.)$ is built as a random linear hyperplane in the kernel implied feature space, that is computed approximately using the random subset $\bs{S}^R_l$.}
                
%Since an arbitrary classifier can be used in the  above generic approach,
% ~\footnote{While theoretical guaranties for locality sensitivity of the above described hashing scheme are missing in the literature, the principle of randomizing each hash function by learning it on a very small subset of samples~($\bs{S}^R_l$ of size $2\alpha \ll M$), should suffice in practice~\cite{wang2014hashing}.},
Finally, our {\em LSH-RLSTM} model uses LSTM language model   for generating hashcodes;  no reference set optimization is required here, since  LSTM  easily handles large training datasets; however, other hyperparameters, including    network's architecture,  need to be optimized.  


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/experiments.tex <==
% \vspace{-0.05in}
\section{Empirical Evaluation}
\label{sec:exp}

Several variants of the proposed   hashing based dialog model, using kNN, SVM or LSTM to build hashcodes, respectively, were evaluated    on three different datasets and compared with  three state-of-art dialog generation approaches of \cite{serban2017hierarchical,serban2016building} and \cite{vinyals2015neural}. Besides several standard evaluation metrics adopted by those approaches, we also %used several hashcode-model specific metrics; most importantly, we also
report the {\em model rankings obtained by human evaluators}  via Amazon Mechanical Turk.
	
% \vspace{-0.05in}
\subsection{Experimental Setup}
% 
\subsubsection{Datasets\\}
% 
The three datasets used in our experiments include (1) depression therapy sessions, (2) Larry King TV interviews and (3) Twitter dataset.   
    
\input{tab_generative_hash_comparison.tex}

The {\em depression therapy dataset}\footnote{{\small {https://alexanderstreet.com/products/counseling-and-psychotherapy-transcripts-series}}} consists of transcribed recordings of nearly 400 therapy sessions between multiple therapists and  patients. Each patient response $S_i^t$ followed by therapist response $S_i^p$ is treated as a single sample; all such pairs, from all sessions, were combined into one set of   N=42000 samples. We select 10\% of the data randomly as a test set (4200 samples), and then perform another random 90/10 split of the remaining  38,000 samples  into  training and validation subsets, respectively. We follow the experimental setup from prior work cited above when comparing the respective neural network models with our hashing based approaches: all models    are  trained  only once using the same training and validation datasets, and evaluated on the same test set. However, for our hashing model metrics introduced below,   we average the estimates over  10 random subsets using  95\% of test samples each time.
    
The {\em Larry King dataset}~\footnote{  {\small http://transcripts.cnn.com/TRANSCRIPTS/lkl.html}}
contains transcripts of interviews with the guests of  TV talk shows, conducted by   Larry King, the host. Similarly to the depression therapy dataset, we put together all pairs of guest/host responses from 69 sessions into a single set of size 8200. The data are split into training, validation and test subsets as described earlier.


Next, we experimented with the   {\em Twitter Dialogue Corpus} \cite{ritter2010unsupervised}.
Considering the original tweet and the following comments on it, in the same session, the task is to infer the next tweet.  Note that we consider all utterances preceding that tweet as one long utterance, i.e. as the first  ``response'' $S_i^A$, mapped to one hashcode,   while the next tweet is the second ``response''  $S_i^B$, which is different from the approach of \cite{serban2017hierarchical} we compare with, where   the previous   utterances in a session are explicitly viewed as a sequence.
The number of tweet sessions (each viewed as a separate sample, i.e.  $\{ S_i^A, S_i^B \}$ pair of responses),   in training, validation, and test subsets are, respectively, 749060, 93633, and 93633.

\subsubsection{Task\\} 
% 
For all datasets, the task is to train a model on a set of training samples, i.e. response pairs $(S_i^A,S_i^B)$, where $S_i^A$ is a response of person A, followed by the corresponding response of  a person B. Then each test sample is given as a response of person A, and the task is to generate the response    of a person B.

% \input{tabCompareAllModels.tex}

\subsubsection{Hashing Models\\}

{\em Step 1: Representation Learning. }	
We evaluate three different hashing models: the first two, based on    kernel locality sensitive hashing (KLSH) \cite{joly2011random,garg2018efficient}, are  called \emph{LSH-RMM} and \emph{LSH-RkNN}, and  use, respectively, Max-Margin (SVM)  classifier  (with C=1 parameter) or kNN classifier~(k=1), to compute each   hash function.
% R stands for random data splits.
%used to compute each hash function. 
The third model, \emph{LSH-RLSTM}, uses LSTM  for hash function computation.
% 
We use hashcode vectors of dimensionality H=100. 
% 
For \emph{LSH-RkNN} and \emph{LSH-RMM}, we use as a reference set a  random subset of M=300 samples from the training dataset, to reduce the computational complexity of training those models, but for \emph{LSH-RLSTM}  we use the whole training dataset as a reference set.
%\footnote{The optimized architectures found by LSH-RLSTM were:  for  Depression Therapy, a four-layer network [16,64,16,8] having  16, 64, 16, and 8  nodes, respectively, in the 1st, 2nd, 3rd and 4th hidden layers; for  Twitter dataset, a 3-layer net [8, 32, 16], an for Larry King dataset, only a two-layer net: [8, 32].}. 
Parameters $\bs{\theta}$ for  LSH models are obtained by   maximizing the proposed MI LB criterion.
%, using  $\gamma=1000$.
% 
% See the supplementary material for more experimental details on the LSH models.
        	

{\em Step 2: Hashcode prediction.}
We now map  all responses, of both participants A and B,  in both training and test sets, to the corresponding hashcodes using one of the above hashcode-based representation models.  
Next, to predict the   response hashcode of a person B given a hashcode of a person A, we train  separate Random Forest (RF) classifiers (each containing 100 decision trees) for each  hashcode bit (i.e. 100 such RF classifiers, since H=100).
 
 {\em Step 3: Textual response generation.}
 Given a hashcode of a response inferred by RF classifier above, mapping it to an actual text can be performed in multiple ways; by default, we find a match of the generated hashcode in the set of all hashcodes corresponding to the person B responses in our training data as this approach is highly suitable for depression therapy like dialogues. In addition, we also provide human evaluation for generating new responses using the N-grams hashing based language model proposed in \secref{sec:gen_response}.
%
% As it was already mentioned before, {\em better generative models remain the direction of future work, while this simple method is used to validate our main contribution, a hashcode-based representation and response prediction model driven by mutual information maximization.}
    	

\subsubsection{Baseline: Neural Network Dialog Generation Models\\}
% 
We compare our dialog generation method with the state-of-art {\em VHRED} approach of \cite{serban2017hierarchical}, as well as with the two other approaches, {\em HRED} \cite{serban2016building}, and {\em LSTM} \cite{vinyals2015neural}, also used as  baselines in the VHRED paper. We adopt  the same hyperparameter settings as those used in   \cite{serban2017hierarchical}. For the  Twitter dataset, we compare with  the results presented in the above paper, while on the other two datasets, we train the above models ourselves. The vocabulary size for the input is set via grid search between values 1000 to 100000. The neural network structures are chosen by an informal search over a set of architectures and we set maximum gradient steps to 80, validation frequency to 500 and step-size decay for SGD is 1e-4.


% \vspace{-0.05in}
\subsubsection{Evaluation Metrics\\}

{\em Embedding-based metrics.}
% 
We compare our methods with the state-of-art neural network approaches listed above using three word embedding-based topic similarity metrics -  {\em embedding  average},    {\em embedding greedy}, and {\em embedding  extrema} \cite{liu2016not}, adopted  by \cite{serban2017hierarchical}. Following the prior art, we used  Google News Corpus to train the embeddings.
% \footnote{https://code.google.com/archive/p/word2vec/}. 
% 
The mean and standard deviation statistics for each metric are computed over 10 runs of the experiment, as mentioned above.
% ; in the case of the accuracy metric, the statistics are computed over  all (100)   hashcode bits and over 10 trials.

% Given a textual response $S^M$~(of Person B) generated by a particular  method, and the true textual response $S^A$~(of person A), all words are first mapped to their corresponding embeddings. An average across the words in each response is computed, and the cosine between the two resulting vectors constitutes the {\em embedding average} similarity metric. 

% Another approach to computing    response-level embeddings is to use  vector extrema, where, for each dimension
% of the word vectors, we select the most extreme value amongst all word vectors in the response, and use that value in the response-level embedding; the cosine similarity is then computed between the corresponding response-level embeddings, resulting into a metric called {\em embedding extrema} \cite{liu2016not}.

% Finally, the third metric, {\em embedding greedy}, does not compute response-level embeddings. Instead, given two responses $S^M$ and $S^A$, each token $w \in S^M$ is greedily matched with a token $w' \in S^A$ having maximum cosine similarity of the corresponding  word embeddings, and the total score is averaged across all words $w$~\cite{liu2016not}.

\input{tabHashDialogModelsCompare.tex}

\noindent{\em Human evaluation.}
% 
Using Amazon Mechanical Turk, we obtained model rankings from 108 human readers (annotators).  For each test sample, we showed to the reader all   responses produced the six models evaluated here, in random order for each instance, and without specifying which model produced which response. We asked the annotator to choose two most appropriate responses; then,  for each model,  we computed across all test samples the  percent of the readers who voted for that model.  Furthermore, in a separate session, we also asked the person which model produced the most diverse responses; in this case we listed the model's names and associated responses.

% \shrink{%%%%%%%%%%%%}
\noindent{\em Information-theoretic metrics.}
% 
The second group of metrics directly evaluates the quality of hashcodes obtained using our models.  For each method, we will report the  proposed MI lower bound~(\emph{MI LB}) from \thmref{thm:mi_lb}, as well as its normalized version~(NMI LB). For each of the metrics, \emph{higher values} mean better performance. 
% 
We also report the {\em hashcode inference accuracy (HIA)},  i.e. the accuracy of predicting hashcode bits of response B using  RF classifiers. We also obtain the baseline accuracy~(\emph{Baseline}), using a trivial classifier that always chooses the most-frequent class label.
% }


% 
% ~\todo{Irina, we should mention explicitly number of instance. We randomly sample a large fraction of test instances for human evaluation for both datasets, i.e. 906 for Depression dataset, and 180 for Larry king dataset. We can round figure the numbers. In terms of amazon turker sessions, we had 151 evaluation sessions for depression and 30 for Larry king, with 6 instances per session.}
 


% \vspace{-0.05in}
\subsection{Results}
% 
\subsubsection{Computational Efficiency\\}
% 
First of all,  we observed that {\em the hashing models are much more computationally efficient than the neural network approaches we compared with}:   it takes from several days (for smaller datasets such as Depression therapy and Larry King dataset containing about 42,000 and 8,200 samples) to more than two weeks (on Twitter, with roughly 749,000 samples) to train a neural network model, even on a 1000-core GPU, whereas an LSH model is typically optimized within several hours (e.g., less than 5-6 hours for Twitter),  on a 16-core CPU.

\subsubsection{Embedding-based Metrics\\}
% 
Table \ref{tab:results} summarizes performance of all methods with respect to the embedding-based metrics, with the best results for each metric/column shown in boldface. Overall, the proposed hashing approaches are quite  competitive with the neural net  methods in terms of those metrics as well: on all three datasets, our LSH methods always outperform their competitors in terms of the {\em average} similarity metric (which is the most intuitive among the three metrics in terms of reflecting the topic similarity between the true and system-generated responses); moreover, our methods also achieve best performance w.r.t. the {\em greedy} metric on Twitter dataset, and w.r.t. {\em extrema} metric on the Depression dataset.  
    
\subsubsection{Human Evaluation\\}
% 
We  also performed an extensive human evaluation of the dialog generation quality (as described earlier in section 5.1), on two relatively smaller datasets, Depression and Larry King. The results are shown in Table \ref{tab:human}a and \ref{tab:human}b, respectively.  {\em The hashcode-based approaches considerably outperform the neural net models, by one-two orders of magnitude,  in terms of the responses being both more appropriate and more diverse}\footnote{See several examples in the supplementary material.}. Amongst the three hashing models, LSH-RkNN seem to be performing the best.
		
Further, we performed another human evaluation of LSH-RkNN, for a comparison between response generation vs response selection, and their comparison w.r.t. the baseline neural models. As we observe in \tabref{tab:human_gen}, both response selection and response generation seem to give equally good responses in terms of appropriateness, and significantly outperform the neural baselines. Low diversity of generated responses remains an issue, as also known to be the case for neural models.

%Note that, similarly to other studies, we observe that those commonly used metrics cannot  truly capture   the quality of the produced dialogues,  and human evaluation is still hard to replace. For example, on Depression dataset, due to its relatively small size, none of the neural net models managed to actually learn how to generate good responses, as the human evaluation results in Table \ref{tab:human} showed which are discussed in the following, despite  relatively good embedding-based metric results. Those models kept generating practically {\em similar responses, of questionable quality}  on the majority of test samples (see an example below), 
%% \todo{don't be so frank, that would mean that the evaluated models are not good choices as baselines.}
%%; see several examples of actual dialogues 
%while  hashing methods often produced much more meaningful responses:

% \todo{we don't need to show these responses in the paper, but supplementary, as we are doing human evaluation itself.}
%% 
%%
%%
%\begin{scriptsize}
%\begin{verbatim}
%<patient> I did lose three pounds, did you notice that?
%<therapist> That's great, I did notice that.
%-------------- Hashing models: -----------------------
%<LSH-RMM> Yes, you did.
%<LSH-RkNN> To help you with your diet?
%<LSH-RLSTM> Okay what's the explanation?
%-------------- Neural network  models: ---------------
%<LSTM> I don't want to be a lot a lot ... of the way
%<HRED> Yeah. you
%<VHRED> Uh-huh. you
%\end{verbatim}
%
%%\shrink{%%%%%%%%%
%\begin{verbatim}
%-------------
%-------------
%<patient> ...Which is stupid because like, ya know, I guess 
%if it's not what they like, then it's not what they like 
%and they can like do something else, but like  ya know 
%there's some psychiatrists who charge like $300 an hour...
%<therapist> I'm sorry you're having such trouble getting 
%... getting access to the care that you need.
%-------------- Hashing models: -----------------------
%<LSH-RMM> You got to do.
%<LSH-RkNN> Oh yeah, you never tried Lithium?
%<LSH-RLSTM> And you ought not to just shove it away out 
%of your life because you will need it again.
%-------------- Neural network  models: ---------------
%<LSTM> Uh-huh. you
%<HRED> Yeah. you
%<VHRED> Uh-huh. you
%\end{verbatim}
%%}%%%%
%\end{scriptsize}
% 
%
%   
% at https://tinyurl.com/y6gefz8k.

% For more examples, see Appendix.

% See Appendix for more examples of actual dialogues; 
%While some of the responses generated by hashing methods were making less sense than others, overall they appeared to be at least to some degree relevant to the conversation, even in relatively small datasets such as Depression and Larry King, not handled well by neural net approaches. 


% \shrink{%%%%%%%%%%%%%%%%%%%%
\subsubsection{Information-theoretic Metrics\\}
% 
Next, we took a deep dive into evaluation of hashing approaches with respect to how well they actually model the alignment between the responses; the results are summarized in Table \ref{tab:results2}, presenting the mutual information lower bound (MI LB), normalized MI LB, and hashcode inference accuracy (HIA) as discussed before; note that besides presenting chance-level baseline classifier accuracy (i.e., selecting the most-frequent class), we also present a similar baseline for MI LB and NMI LB metrics, using  randomly permuted (shuffled) pairings between responses of person A and person B. We now look at the  difference between each  metric and its corresponding baseline, shown in parenthesis, and highlight the largest, most significant differences between the means of both metrics in boldface. 
    
Overall, {\em LSH-RMM} method appear to be the best on all datesets  in terms of most significant improvement over the baseline in terms of normalized MI LB and prediction accuracy, although {\em LSH-RLSTM} is the best in term of the raw MI LB on Twitter and Larry King datasets.
    
% \footnote{The optimized architectures obtained by   LSH-RLSTM approach were as follows:  for  Depression Therapy, a four-layer network [16,64,16,8] having  16, 64, 16, and 8  nodes, respectively, in the 1st, 2nd, 3rd and 4th hidden layers; for  Twitter dataset, a 3-layer net [8, 32, 16], an for Larry King dataset, only a two-layer net: [8, 32].}.

% }%%%%%%%%%%%%%%%%%%%

% {\bf Reference Set Selection. \\}
% Moreover, in  \tabref{tab:results_ref_set_sel} we demonstrate some model improvement in terms of information-theoretic metrics   when using optimized rather than randomly selected reference set in our kernel-based models; when the reference set size is small (M=100 used in our experiments), optimization can provide clear benefits over random subset selection. In the supplementary material, we show the optimized reference set for LSH-RkNN for Depression Therapy dataset.
        
% % 
% \paragraph{MI Evolution over Therapy Sessions.}
% % 
% Finally, we provide an initial evaluation of our (normalized) MI LB metric~(using RkNN model) as a proxy  of developing alliance between the patient and therapist during therapy sessions, on Depression dataset. The NMI LB metric evolution  over the course of  a session is computed  using moving window of size 20, for    170 sessions of sufficient length (at least 100 samples, i.e. patient/therapist response  pairs); next, we warp the obtained  varying-length time series   onto a uniform 1,000-dimensional grid using linear interpolation, so that the first and the last entries of each session are mapped to the first and last element of the grid. We then compute SVD on the resulting  matrix. \figref{fig:mi_svd} shows the first (temporal)  SVD component (i.e. the mean across the sessions), which accounts for 30\% of the variance.   Note an interesting  temporal evolution of the metric, which can potentially be used as a proxy for evaluating  alliance development (or the lack of it) during therapy sessions, as discussed earlier.

% % 
% \begin{figure}[tp!]
% \centering
% \includegraphics[
% width=0.9\columnwidth]{svd.pdf}
% \vspace{-5.0mm}
% \caption{
% Evolution of (normalized) mutual information (lower bound) over the course of a therapy session in Depression dataset (1st SVD component, accounting for 30\% of the variance, that also corresponds to mean across 170 sessions).
% }
% \label{fig:mi_svd}
% \end{figure}

% \begin{table}[tp!]
% \centering
% \tabsize
% % \renewcommand{\arraystretch}{0.8}% Tighter
% \renewcommand{\tabcolsep}{2.5pt}
% % 
% \begin{tabular}{lllllllll}
% \toprule	
% \bf{Model}
% % &\bf{Reference Set}
% &MI LB~(Shuffled)
% % & Entropy UB
% &NMI LB
% % ~(Shuffled)
% &HIA~(Baseline)
% % &Average
% % &Greedy
% % &Extrema
% \\
% % 
% % \toprule
% % % 
% % LSH-RkNN~(M=30)
% % &Random Sel.
% % % 
% % &-2.3$\pm$0.2~(-2.5$\pm$0.3)
% % % & 5.3$\pm$0.2
% % &-0.43~(-0.47)
% % % &0.97$\pm$0.08~(0.95$\pm$0.10)
% % % &0.27$\pm$0.24
% % % &0.33$\pm$0.24
% % % &0.16$\pm$0.18
% % \\
% % % 
% % \midrule
% % % 
% % LSH-RkNN~(M=30)
% % &MI LB Opt.
% % &0.4$\pm$0.2~(-0.9$\pm$0.2)
% % % & 9.5$\pm$0.2
% % &0.04~(-0.09)
% % % &0.95$\pm$0.11~(0.93$\pm$0.13)
% % % &0.59$\pm$0.37
% % % &0.56$\pm$0.34
% % % &0.35$\pm$0.24
% % \\
% % % 
% % 
% \toprule
% % 
% LSH-RkNN~(Rnd.)
% % ~(M=100)
% % &Random Sel.
% &5.1$\pm$0.1~(1.9$\pm$0.2)
% % & 13.5$\pm$0.2
% &0.38~(0.14)
% &0.92$\pm$0.13~(0.89$\pm$0.15)
% % &0.53$\pm$0.35
% % &0.47$\pm$0.28
% % &0.28$\pm$0.20
% \\
% % 
% \midrule
% % 
% LSH-RkNN~(Opt.)
% % ~(M=100)
% % &MI LB Opt.
% &{\bf9.2$\pm$0.4~(1.2$\pm$0.5)}
% % &25.5$\pm$0.4
% &{\bf 0.36~(0.05)}
% &{\bf0.79$\pm$0.17~(0.75$\pm$0.19)}
% % &0.46$\pm$0.38
% \\
% %
% % 
% % 
% % % 
% % \toprule
% % % 
% % LSH-RkNN~(M=300)
% % &Random Sel.
% % &0.57~(0.27)
% % &0.5$\pm$0.39
% % \\
% % % 
% % \midrule
% % % 
% % LSH-RkNN~(M=300)
% % &MI LB Opt.
% % &0.46~(0.21)
% % &0.55$\pm$0.38
% % \\
% % %
% % % 
% % 
% % 
% % 
% % 
% % \toprule
% % % 
% % LSH-RMM~(M=30)
% % &Random Sel.
% % &
% % \\
% % % 
% % \midrule
% % % 
% % LSH-RMM~(M=30)
% % &MI LB Opt.
% % &
% % \\
% % % 
% % % 
% % 
% \toprule
% % 
% LSH-RMM~(Rnd.)
% % ~(M=100)
% % &Random Sel.
% &13.4$\pm$0.4~(-1.1$\pm$0.3)
% % & 35.3$\pm$0.4
% &0.38~(-0.03)
% &{\bf{0.68$\pm$0.10~(0.59$\pm$0.09)}
% % &0.57$\pm$0.40
% % &0.54$\pm$0.34
% % &0.31$\pm$0.25
% \\
% % 
% \midrule
% % 
% LSH-RMM~(Opt.)
% % ~(M=100)
% % &MI LB Opt.
% &{\bf16.2$\pm$0.3~(0.1$\pm$0.4)}
% % &35.6$\pm$0.2
% &{\bf0.46~(0.01)}
% &0.66$\pm$0.11~(0.58$\pm$0.10)
% % &0.41$\pm$0.40
% \\
% %
% % 
% % 
% \toprule
% \end{tabular}
% \vspace{-3.0mm}
% \caption{
% % \csizenine
% Analysis for MI LB based optimization of reference set $\bs{S}^R$~(of size, M=100) w.r.t. the random selection baseline within LSH-RkNN \& LSH-RMM, using Depression Therapy dataset.
% }
% \label{tab:results_ref_set_sel}
% % \vspace{-5.5mm}
% \end{table}

% \subsubsection{Model Selection using MI LB}

% \subsubsection{Analyzing Therapy Sessions with MI LB}


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/fig_framework.tex <==
\begin{figure}[tp!]
\centering
\includegraphics[
width=\columnwidth]{dialogue_model_framework.pdf}
\label{fig:hash_app}
\vspace{-5.25mm}
\caption{
\csize
An intuitive illustration of the kernelized hashcodes based framework for dialog modeling. It involves three steps. In the first step~(top), we learn a hashing model to obtain hashcode representations of dialogue utterances; the objective behind learning a hashing representation via maximizing the  mutual information between a patient (left) and therapist (right) responses is to find a compressed encoding of those responses which preserves the mutually relevant content while ignoring irrelevant details; e.g., in the example above, we would expect a good representation model to capture  the content highlighted in  boldface as essential to the conversation.
% 
% 
In step 2~(bottom left), we train a ensemble of decision tree classifiers so as to infer hashcode for a therapist response, given the hashcode representation of the corresponding patient utterance~(input).
% 
% 
In step 3~(bottom right), having the inferred therapist hashcode, we map it to a textual response. One can choose a response from the training set of therapist responses, the one for which its hashcode has low hamming distance w.r.t. the inferred therapist hashcode. Or, we can generate a novel response using N-Grams based language modeling, generalized with kernelized hashing of N-Grams.
% 
% \todo{compress step 2, more details in step 3. Add response selection itself. Remove actual hashcode digits in the step 3. Generic component to connect a hashcode to n-grams or sentence in training set.}
}
% 
\vspace{-4.75mm}
\label{fig:klsh_max_mi}
\end{figure}



==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/hashingAlgo.tex <==
\begin{algorithm}[tp!]
\caption{
\csize
% Generic 
Generalized Algorithm for Constructing
% ~(Kernel) 
Locality Sensitive Hash Functions, with Kernel Functions or Neural Networks}
\csizenine
\begin{algorithmic}[1]
\REQUIRE Reference set $\bs{S}^R$, of size $M$; sub-sampling parameter, $\alpha$; number of hash functions, $H$.
% 
% \COMMENT{Random subsets, fixed across structure inputs}
% 
\STATE $\bs{z} \gets \{ \bs{0}_{\alpha}, \bs{1}_{\alpha} \}$
% 
% \COMMENT{labels for hash code bit}
% 
% \STATE $\bs{K}_{RR} \gets$ computeKernel($\bs{S}^R$, $\bs{S}^R$)
% \COMMENT{kernel matrix of size $M \times M$}
\FOR{$l=1 \to H$}
% 
\STATE $\bs{S}^R_l \gets$ randomSubset($\bs{S}^R$, $2\alpha$)
% 
\COMMENT{random subset from $\bs{S}^R$ of size $2\alpha$, $\bs{S}^R_l$}
% 
\STATE $\cH_l(.) \gets$ TrainBinaryClassifierAsHashFunction$\left(\bs{S}^{R}_l, \bs{z}\right)$
\ENDFOR
% 
\RETURN $\bs{\cH(.)} = \{ \cH_1(.), \cdots, \cH_H(.) \}$
% 
\end{algorithmic}
\label{alg:our_algo_klsh_codes}
\end{algorithm}


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/human_eval.tex <==
\begin{table*}[tp!]
\centering
% \csizenine
% \tabsize
% \renewcommand{\tabcolsep}{2.0pt}
\subtable[Depression Dataset]
{
\centering
\begin{tabular}{llllllllllll}
\toprule	
% 
&LSTM&HRED&VHRED&LSH-RkNN&LSH-RMM&LSH-RLSTM\\
% 
% 
% % 
% \textbf{Model}&Appropriate~(\%)&Diverse~(\%)
% % &Least Diverse~(\%)
% \\
% \toprule
% \textbf{LSTM~\cite{vinyals2015neural}} &3.7&0.7
% % &18.4
% \\
% \midrule
% \textbf{HRED~\cite{serban2016building}} &8.6&9.3
% % &30.6
% \\
% \midrule
% \textbf{VHRED~\cite{serban2017hierarchical}} &9.5&0.7
% % &30.6
% \\
% \toprule
% \textbf{LSH-RkNN}& \textbf{28.7}&35.1
% % &12.2
% \\
% \midrule
% \textbf{LSH-RMM} &24.1&13.2
% % &\textbf{2.0}
% \\
% \midrule
% \textbf{LSH-RLSTM}&25.4&\textbf{41.1}
% % &6.1
% \\
% 
% \toprule
% 
% total 151 pages
% 1812 count total
% counts
% &67&156&172&520&436&461\\
% 
\toprule
% percent
Appropriate~(\%)&3.7&8.6&9.5&\textbf{28.7}&24.1&25.4\\
% 
% 
% % 100 pages
% &11&45&39&163&161&181\\
% &18&34&50&194&152&152\\
% \midrule
% % 49 pages
% &17&39&42&69&60&67\\
% &21&37&38&86&60&52\\
% \midrule
% % 2 pages
% &0&1&1&4&3&3\\
% &0&0&2&4&0&6\\
% 
% 
% most diverse responses
% total
% 151
% &1&14&1&53&20&62\\
% 
\midrule
% percent
Diverse~(\%)&0.7&9.3&0.7&35.1&13.2&\textbf{41.1}\\
% 
% 
%
% least diverse
% 49
% &9&15&15&6&1&3\\
% percent
% &18.4&30.6&30.6&12.2&2.0&6.1\\
% 
% 
\toprule
\end{tabular}
}
% 
% \vspace{-5mm}
% 
\subtable[Larry King  Dataset]
{
\centering
\begin{tabular}{llllllllllll}
\toprule	
% 
% 
&LSTM&HRED&VHRED&LSH-RkNN&LSH-RMM&LSH-RLSTM\\
% 
% 
% \textbf{Model}&Appropriate~(\%)&Diverse~(\%)
% % &Least Diverse~(\%)
% \\
% \toprule
% \textbf{LSTM~\cite{vinyals2015neural}} &5.3&3.3\\
% \midrule
% \textbf{HRED~\cite{serban2016building}} &3.9&13.3\\
% \midrule
% \textbf{VHRED~\cite{serban2017hierarchical}} &5.3&0.0
% \\
% \toprule
% \textbf{LSH-RkNN}&\textbf{31.7}&\textbf{36.7}\\
% \midrule
% \textbf{LSH-RMM} &25.6&10.0\\
% \midrule
% \textbf{LSH-RLSTM}&28.3&\textbf{36.7}\\
% % 
% 
% count
% first row
% &11&8&8&64&50&39\\
% second row
% &8&6&11&50&42&63\\
% total count fro two rows
% 360
% &19&14&19&114&92&102\\
% percent
\toprule
Appropriate~(\%)&5.3&3.9&5.3&\textbf{31.7}&25.6&28.3\\
% 
% 
% most diverse
% 30
% &1&4&0&11&3&11\\
\midrule
Diverse~(\%)&3.3&13.3&0.0&\textbf{36.7}&10.0&\textbf{36.7}\\
% 
% 
\toprule
\end{tabular}
}
% 
% \vspace{-2.5mm}
% 
\caption{
% \csizenine
Human evaluation scores on (a) Depression dataset 
% (906 test samples) 
(900 test samples) 
and (b) Larry King dataset~(180 test samples).
}
\label{tab:human}
% \vspace{-2.75mm}
\end{table*}


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/intro.tex <==
% \vspace{-0.1in}
\section{Introduction}
% 
Dialogue modeling and generation is an active research area  of great practical importance  as it provides a solid basis for building successful conversational agents in a wide range of applications.  However, despite recent successes of deep neural dialogue models,   the open dialog generation problem is far from being solved~\cite{vinyals2015neural,li2016deep,serban2016building,serban2017hierarchical,li2017adversarial,zhao2018unsupervised,wu2018learning,zhang2018generating,xu2018diversity,park2018hierarchical,jiang2018sequence,pandey2018exemplar,tao2018get,xing2018hierarchical,chen2018hierarchical,shen2018improving,shi2018toward,du2018variational,li2019insufficient,gupta2019insights}.
        
                    
Therefore, it is important to continue exploring novel types of models   and  model-selection criteria, beyond today's deep neural dialogue systems, in order to better capture the  structure of different types of dialogues and to overcome certain limitations of neural models, including dependence  on large training datasets, long training times, and difficulties incorporating non-standard objective functions, among others. Along those lines, in this paper, we propose a \emph{first-ever nonparametric approach}~\cite{wasserman2006all}, i.e. based on \emph{convolution kernel similarity} functions~\cite{haussler1999convolution,mooney2005subsequence,scholkopf2001learning}, for modeling and generation of dialogues.
                    
Moreover, different applications may possess specific properties which suit some approaches better than others.
% 
%Moreover, specific applications may impose certain structure which could make dialogue modeling   more tractable  than modeling a completely open dialogue.
% 
%  
In this work, one of the motivating applications is a fast-growing area of  (semi-)automated \emph{psychotherapy}:  easily accessible, round-the-clock psychotherapeutic services provided by a conversational agent. The importance of this area cannot be underestimated:   according to recent statistics, mental health disorders affect one in four adult Americans, one in six adolescents, and one in eight children; predicted by the World Health Organization, by 2030 the amount of worldwide disability and life loss attributable to depression may become greater than for any other condition, including cancer, stroke, heart disease, accidents, and war. 

However, many people do not receive an adequate treatment. One of the major factors here is  limited availability of mental health care professionals, as compared to the number of potential patients; thus, automating at least some aspects of the treatment is a promising  direction.
% 
%Thus, creating automated systems providing mental health services is becoming an increasingly important area of research and development.  
% 
%However, existing conversational systems in this domain are still primarily rule-based, and lack sophisticated dialogue modeling and generation capabilities based on actual text understanding.

% \input{./tab_response_hashcodes.tex}

One of the domain-specific challenges in automated therapy is {\em difficulty obtaining large training datasets} which are often necessary for neural dialogue models; this limitation may require developing alternative approaches.   Another domain-specific property  of therapeutic dialogues, which can  potentially  simplify dialogue generation, is the classical pattern of relatively long patient's utterances (up to thousands of words) followed by much shorter  therapist's responses.   Therapist's responses are often high-level, generic statements,   confirming and/or summarizing  patient's responses; they {\em can be viewed as semantic ``labels" to be  predicted from patient's ``input samples"}.
    
%Note that, rather than  generating a specific response sentence directly, a more effective, modular approach can be to first infer a conceptual, high-level representation reflecting the essence of the ``most relevant" response to the patient, and then use a separate mapping from such semantic representation to textual response.

%Thus,  inspiring models which try to {\em capture the semantics of the whole   patient's and therapist's responses in their respective vector representations}, and view dialogue generation as predicting therapist's response vector from the  patient's  response vector -- an approach adopted in this work.
%which map each whole response  observation giving an inspiration for predictive model mapping representation into ther model which maps the whole response  may try to  Generating such a short, constrained  response can be a somewhat easier task than solving the open-domain dialogue challenge. 

\input{fig_framework.tex}

Furthermore, a therapy session is  typically  an example of a   {\em collaborative dialogue}, unlike  debates, political arguments, and so on.
Indeed, a fundamental concept in psychotherapy is the working alliance between the therapist and the patient~\cite{bordin1979generalizability}. The alliance involves 
%several cognitive and emotional components of the relationship between these two agents, including
 the agreement on the goals to be achieved and the tasks to be carried out, and the bond, trust and respect to be established over the course of the therapy. While an encompassing formalization of working alliance is a challenging task, we propose {\em maximizing  mutual information between the patient's and therapist's responses} as a simple criterion helping us capture, to some extent, the dynamics of agreement expected to develop in most therapies, and, more generally, in other types of dialogues\footnote{Note that imbalanced response length between the two participants, as well as collaborative property, are   shared with some other types of dialogues, e.g., TV show interviews such as Larry King dataset analyzed in this paper, where the guest of a show produces long responses, with the host inserting relatively short comments facilitating the interview.}. Furthermore, {\em  maximizing mutual information}  between the patient's and therapist's can  {\em improve the   predictability of the latter from the former},  thus facilitating better dialogue generation.%Furthermore, it is desirable to optimize 
%representation models with the objective of increasing relevance, or coherence, between the consecutive responses, as well as predictability of one response from another, to facilitate better dialog generation -- the objective likely to be  captured by the notion of {\em mutual information} between the responses.
                
Motivated by above considerations, we introduce here  a novel dialogue modeling framework, the \emph{first-ever nonparametric approach for dialogue modeling}, where responses are represented as \emph{locality-sensitive kernelized hashcodes}~\cite{kulis2009kernelized,joly2011random,garg2018efficient,garg2019nearly}, and the hashing models are optimized using a {\em novel mutual-information lower bound}, since exact mutual information computation is intractable in high-dimensional spaces; one can also use neural networks for learning the hashcode representations, as we demonstrate in the experiments section. Using hashcode representations allows for a more tractable way of  predicting responses in a compressed, general representation space instead of direct generation of textual responses. (Previously, kernelized hashcode representations were  successfully applied in the prior works on  information-extraction   \cite{garg2018efficient,garg2019nearly}.) Once the compressed representation of the response is inferred, any separately trained generative model can be plugged in to produce an actual textual response. See \figref{fig:klsh_max_mi} for an illustration of the framework.
% 
% \footnote{Herein we used a quick and  easy approach to text generation, simply selecting the nearest neighbor of the inferred response from the training dataset, while the main objective was to validate the proposed representation learning and representation prediction  techniques; exploring better  text-generation models remains the topic of future work.}
%  
Note that separating response inference in the representation space from the actual text generation increases method's flexibility, while mutual information criterion facilitates better alignment between the responses of two subjects and higher predictability of the proper response. 
    % 
It is also important to note that,  while the  psychotherapy domain was our primary motivation, the proposed approach is generally   applicable to a wider range of   domains as demonstrated in empirical section. 

Overall, our  \emph{key contributions} include:
% 
(1) a novel  generic framework for dialogue modeling and generation using \emph{kernelized locality sensitive hash functions};
(2) a \emph{novel lower bound on the Mutual Information~(MI)} between the hashcodes of the responses from the two agents used as an optimization criterion for the locality sensitive hash functions; (3) a language model to generate therapist responses, generalizing from the traditional N-grams based language modeling approach via kernelized hashing of N-grams.
% of any length.
                                
We provide an extensive empirical evaluation on three different dialogue domains, from depression therapy to TV show interviews and Twitter data,  demonstrating {\em advantages   of our approach} when compared with the state-of-art neural network based dialog systems, both in terms of the {\em higher quality of generated responses} (especially on relatively small datasets (thousands of samples), including therapy sessions and Larry King TV interviews), as well as   {\em computational efficiency, reducing the training time from days or even weeks (e.g. on near-million-sample Twitter dataset) to a few hours}.
  


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/intro_AISTATS.tex <==
\section{Introduction}
% 
Dialogue modeling and generation is an area of active research, and of great practical importance, as it provides a basis for building successful conversational agents in a wide range of applications.  While an open-domain dialogue remains a highly challenging open problem,  developing dialogue systems for particular applications can be more tractable,  due to specific properties of the application domain.

In our work, one of the motivating application is a fast-growing area of  (semi-)automated psychotherapy:  easily accessible, round-the-clock psychotherapeutic services provided by a conversational agent. According to recent estimates, mental health disorders affect one in four adult Americans, one in six adolescents, and one in eight children. Furthermore, as  predicted by the World Health Organization, by 2030 the amount of worldwide disability and life loss attributable to depression may become greater than for any other condition, including cancer, stroke, heart disease, accidents, and war. However, many people do not receive an adequate treatment; one of the major factors here is  limited availability of mental health care professionals, as compared to the number of potential patients. Thus, creating automated systems providing mental health services is becoming an increasingly important area of research and development; nevertheless, existing conversational systems in this domain are still primarily rule-based, and lack sophisticated dialogue modeling and generation capabilities based on actual text understanding.

\begin{table}
\centering
% \tabsize
% \csizeten
\csizenine
% \fontsize{8}{8}\selectfont
% \renewcommand{\arraystretch}{0.9}% Tighter
% \scriptsize
\begin{tabular}{p{7.75cm}}
\toprule
% % CLIENT: 
% But for the next person I mean. I deal with - that's part of what I do is I train people. I'm always - I'm either training people on this computer or what I like to do more is training people how to understand and train.
% And so I have - I feel bad when I give up on a trainer, you know. I just don't think she has it. It's - and I have met people who have had tremendous, tremendous abilities of being able to like grasp concepts and communicate them to others who I had more belief in, you know. [00:16:13]
% Does that make - I guess that...
% ((Crosstalk))\\
% 0101001111001011111110101101111111011011100011101100111000101011110111001001011011001110001010100100
% \\
% \\
% \thp{
% % THERAPIST: 
% For now it's just you don't - can't see like A, (inaudible at 00:16:25) a look at yourself and B, can't see her dealing well with anybody else.}\\
% \thp{
% 0101001111011011111100101101111110011011100001000100111100101000110111001001011111001110001000001000
% }
% \\
% \midrule
% % CLIENT: 
% My dad actually seems in, um, better shape health-wise than he has in a while. I was worried about him the last time I was down there, but the one thing I told him, I said, you know - we were - they had already been in town a few hours. I said, "You know, you haven't told me one story that you've already told me before." I said, "I don't know if you've changed your diet or something, but you're not as senile as you used to be." (Laughing.)\\
% % [00:03:27]\\
% 010100111100101111110010110111111001101110001100010011110010100
% % 1110111001101011111011110001000000000
% \\
% \\
% \thp{
% % THERAPIST: 
% (Laughing.)
% }
% \\
% \thp{
% 010110011011101111111011110011011010111111101111011011100010110
% % 1100011101010011011001110101000100000
% }
% \\
% \midrule
% PT:	
% I'll stay on the Restoril, I mean it takes me a while to go to sleep but I'll stay on the Restoril.
% \\
% 0101001111101111111110101101011110011010100011100101111000101011110111001001011011001110001010000110
% \\
% \\
% \thp{
% % DR:	
% Let's nudge the Pamelor up a little bit.  We could also check a blood level.
% }
% \\
% \thp{
% 0111001111001011111100101100111110011010110001001100111100101101010111001011011011111110001100000000
% }

% \thp{
% 010101011010111111111010110101111001101110000110010011100010101
% % 1110111001001011011001110001010100010
% }
% \\
%\midrule
% PATIENT: 
\textit{
Its all my fault. It's like getting hit in the stomach and trying to catch your breath. You can't catch it. You struggle, move around, you just can't get your breath. That just really knocks me off balance. You begin to generate this feeling of a kind of negativism...
%And that's why it really being hurt. I never allowed myself to think negative, accept everybody else. I am the only one giving back to the "be quiet time." I had to have something to make do with that.
}
\\
{\bf 0101001111001011111110101101011110011011100011101}
% 1001110
% 0010100
% 1110111101011011011001110001000000000
\\
\thp{
% COUNSELOR: 
\textit{
OK. Maybe that fits into the whole pattern then.
}
}\\
\thp{
0111001101001011111100011111111110001010110011001
% 1001110
% 0010110
% 0010111101010011011011110001100001000
}
\\
% \midrule
% CLIENT: 
% \textit{
% Well I talked to a friend of mine whom I think is promiscuous and she told me about a man that came to see her at her apartment. So I gave him my phone number. I don't have any hang up about morals. I don't know. I told a couple of my friends about this. I must admit I'm a little shy talking about it now.
% % [0:23:27.1]
% }
% \\
% 010100011010101111111010110101111001101110000110010011100010100
% % 1110111001011011011001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% I see. You mean it's embarrassing to tell me about it.
% }
% }
% \\
% \\
% \midrule
% % PT: 
% \textit{
% Yeah.  I didn't think she was going to die.
% }
% \\
% 010100011010101111111010110001111001001110001110010011100010101
% % 1110111101001011011001110001000100010
% \\
% \\
% \thp{
% % DR: 
% \textit{
% Yeah.
% }
% }\\
% \thp{
% 010110011011100111111010110001111110101111100110011011110010111
% % 1010111101010011010101110101010100010
% }
% \\
% 
% \midrule
% CLIENT: So I filed a bug report on Wednesday.\\
% \\
% THERAPIST: Yeah.\\
% 
% \midrule
% % PATIENT: 
% \textit{
% I'm sitting here just thinking about things. Should I think out loud? (chuckles)
% }
% \\
% 01010001111010111111001111011111110010111000011001
% 00111000101011110111001101011001001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% Sure. If you want to.
% }
% }
% \\
% \thp{
% 11010011001110111111001011011101110100111000111011
% 00111100101001110111101100011001001110001010000000}
% \\
% \midrule
% % CLIENT: 
% \textit{
% Because it's almost a year of my life.
% }
% \\
% 01010011110010111111001011010111101100101100110011
% 00111100101101110111101011011011011110001000100000\\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% All this is. It's a good chunk of time.
% }
% }\\
% \thp{
% 01010011010010111111001011010111101010101000110011
% 00111100101101110111101011011011001110001000100000
% }\\
% 
% \midrule
% % PATIENT: 
% \textit{
% Most of it is small bills. There's one 50 dollar check, and that's the only thing that's really large. The rest of it's like ten or twelve dollars each.
% }\\
% 010100110100101111110010110111111001101111001100110011110010110
% % 0110111101011011011011110001000101000
% \\
% \\
% \thp{
% % THERAPIST: 
% \textit{
% But it adds up.
% }
% }
% \\
% \thp{
% 010101111110101111111011110101111000101110000110010011100010100
% % 111011110
% % 1111011011001110001010100010
% }
% \\
\toprule
\end{tabular}
\vspace{-3.25mm}
\caption{
\small
% \fontsize{8}{8}\selectfont
An example of patient/therapist responses in a depression therapy session, with associated binary hashcodes; patient's hashcode will be used as a feature vector to predict the bits of the  therapist hashcode. 
%In this table, we show pairs of patient and therapist~(Blue) responses.
% , randomly sampled from different sessions.
% ; the responses of therapists are in red. 
%For each response, we obtain a locality sensitive hashcode as its representation.
% , of 100 bits each. 
%The hashcode of a patient response is used as feature representation to infer the hashcode of the corresponding therapist response.
% as multi-class labels.
}
\label{tab:therapy_session_hashcoded}
\vspace{-6mm}
\end{table}%
% 
% \input{tabResponseHashcodes.tex}

An interesting feature of therapeutic dialogues appears to be a classical pattern of a relatively long monologue of  a patient followed by a considerably shorter  response of  a therapist; this property is also shared with some other types of dialogues, e.g., TV show interviews such as Larry King dataset analyzed in this paper, where the guest of a show produces relatively long monologues, with the host inserting relatively short comments. Moreover, therapist's responses tend to be rather  high-level, generic statements, typically summarizing/confirming the patient's response, and can be viewed as a ``category label" being ``assigned" to a patient's text ``sample". Generating such a short, constrained  response can be a somewhat easier task than solving the open-domain dialogue challenge. 

Rather than  generating a specific response sentence directly, a more effective approach can be to first infer a conceptual, high-level representation reflecting the essence of the ``most relevant" response to the patient. Furthermore, it is desirable to optimize representation models with the objective of increasing relevance, or coherence, between the consecutive responses, as well as predictability of one response from another, to facilitate better dialog generation -- the objective likely to be  captured by the notion of {\em mutual information} between the responses.

Note that a fundamental concept in psychotherapy is the working alliance between the therapist and the patient or, more generally, the client seeking help~\cite{bordin1979generalizability}. The alliance involves several cognitive and emotional components of the relationship between these two agents, including the agreement on the goals to be achieved and the tasks to be carried out, and the bond, trust and respect to be established over the course of the therapy. While an encompassing formalization of working alliance is a challenging task, it is however reasonable to consider that the  mutual information criterion may capture, to some extent, the dynamics of agreement expected to develop in most therapies, and, more generally, in other types of dialogues.
            
Motivated by above considerations,  we  introduce here  a novel dialogue modeling framework where responses are represented as \emph{locality-sensitive binary hashcodes}~\cite{kulis2009kernelized,joly2011random,garg2018efficient}, and the hashing models are optimized using a {\em novel mutual-information lower bound}, as mutual information computation is intractable in high-dimensional spaces. Using hashcode representations may allow for 
a more tractable way of  predicting responses in a compressed, general representation space instead of direct generation of textual responses.
(Note that hashcode representations were  successfully applied in prior work on  information-extraction   \cite{garg2018efficient}). Furthermore, separating inference in representation space from text generation (based on inferred response representation) increases method's flexibility, while mutual information criterion facilitates better alignment between the responses of two parties and higher predictability of the proper response. While the  psychotherapy domain was our primary motivation, the proposed approach is generally   applicable to a wider range of   domains as demonstrated in empirical section. Overall, our  \emph{key contributions} include:
% 
(1) a novel  generic framework for dialogue modeling and generation using \emph{locality sensitive hash functions};
(2) a \emph{novel lower bound on the Mutual Information~(MI)} between the hashcodes of the responses from the two agents used as an optimization criterion for the locality sensitive hash functions;
(3) an extensive empirical evaluation on three different dialogue domains, from depression therapy to TV show interviews and Twitter data,  demonstrating competitiveness   of our approach when compared with the state-of-art neural network based dialog systems, and its clear superiority in case of relatively small datasets (e.g., therapy sessions), both in terms of the quality of generated responses and computational efficiency.
  

==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/lstm.tex <==
\section{Neural Networks}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.46\textwidth]{LSTM_dialog.pdf}
    \caption{Hashcode generation using neural models: To generate hashcodes using neural models, we train the LSTM model to fit the labels for reference set of dialogs. Each dialog in the reference set is input as a sequence of individual word embeddings into an LSTM/GRU model with $k$ layers, each layer containing a specific number of LSTM units. The model is then evaluated on the rest of the dialogues to obtain a single bit in the hashcode. The process is repeated with different reference sets to generate the hashcode.}
    \label{fig:schema}
\end{figure}
In addition to kernel similarity functions, we explore using neural networks to generate hashcodes. For each reference set defined above, we learn a recurrent neural network model to predict the randomly assigned labels. The model learns a non-linear mapping which is then used to obtain a single hashcode bit for the remaining text. For kernel based methods we optimize the reference set of dialogs. However, for neural models, we optimize the hyperparameters of the model which consists of the number of layers and the number of neurons in each layer. For each configuration, we compute the mutual information of responses and use the parameters which generate the highest value. For simplicity, we do not vary the activation function and learning rate. We train our model using Adam~\cite{kingma2014adam} and the gradients are calculated using back propagation.
	
In our experiments, we vary the neural network model size. We test models with 1 to 3 layers. To determine the number of neurons for each layer, we perform a grid search over $[8, 16, 32, 64, 128]$. As the number of instances in our training data is very small, the above configurations suffice in capturing the data. We use a sigmoid layer for final prediction and a fixed learning rate of $10^{-3}$.

==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/mainTable.tex <==
\begin{table*}[tp!]
\centering
\tabsize
% \renewcommand{\arraystretch}{0.8}% Tighter
\renewcommand{\tabcolsep}{2.0pt}
% 
\begin{tabular}{llllllllllll}
\toprule	
Hashing Func.&Hash Config.
% ~(Optimization)
&Model
& \textbf{MI LB}~(Shuffled)
&\textbf{Entropy UB}
% 
% &MI LBs Ratio
% 
&NMI LB (Shuffled)
% 
% &Marginal CE UB
% &\textbf{Inference}~(Marginal MI LB)
&Accuracy~(Baseline)
% Accuracy)\\
% &Marginal E.
% &TC Bound
\\
% 
\midrule
% 
% \textbf{
Kernel-RkNN&M=30, $\alpha$=10&
% }
\\
% \midrule
% &Random*&$82.61\pm17.85$~($77.84\pm20.55$)&$-13.83\pm1.57$&$33.49\pm0.12$&$17.45\pm1.54$&$29.88\pm0.12$\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% 
% 
% % &
% &$-14.6\pm2.6$
% &$15.3\pm2.6$
% % &$3.6\pm0.2$
% &$82.6\pm17.9$~($77.8\pm20.6$)
% %&$33.49\pm0.12$
% % &$18.22\pm2.55$
% % &$29.85\pm0.10$
% \\
% % 
% 
% &
&$-12.1\pm4.4$~($-12.1\pm2.4$)
&$5.1\pm4.6$
%
% &1.0
&N.A.
% 
% &$17.2\pm0.4$
% 
% &$1.7\pm0.5$
&$93.6\pm8.6$~($89.4\pm12.2$)
%&$18.87\pm0.36$
% &$13.14\pm4.69$
\\
% 
% 
% % &
% &$-8.2\pm5.3$
% &$19.5\pm5.3$
% % &$6.0\pm0.3$
% &$85.2\pm14.0$~($79.0\pm16.3$)
% %&$33.68\pm0.25$
% % &$14.17\pm5.27$
% % &$27.68\pm0.19$
% \\
% 
% 
% % &
% &$-9.7\pm1.0$
% &$5.6\pm1.0$
% % &$1.1\pm0.4$
% &$93.7\pm10.5$~($90.4\pm14.2$)
% %&$16.36\pm0.27$
% % &$10.78\pm0.98$
% % &$15.30\pm0.25$
% \\
% 
% 
% % &
% &$-11.7\pm0.8$
% &$17.2\pm0.9$
% % &$3.4\pm0.3$
% &$85.2\pm15.5$~($79.8\pm18.2$)
% %&$32.27\pm0.19$
% % &$15.06\pm0.91$
% % &$28.92\pm0.20$
% \\
%
% 
% &&$\pm$~($\pm$)&$-7.88\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$-9.38\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$-6.04\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% 
% \midrule
% 
% 
% &MI LB Opt~($\gamma=100,\beta=300$)&$87.27\pm15.80$~($82.90\pm18.51$)&$-6.66\pm0.39$&$27.22\pm0.25$&$10.72\pm0.42$&$23.16\pm0.27$&$16.5\pm$&$4.06\pm$\\
% % 
% % 
% &MI LB Opt~($\gamma=300,\beta=300$)&$90.42\pm11.44$~($85.75\pm14.88$)&$-4.71\pm0.65$&$24.10\pm0.25$&$9.26\pm0.64$&$19.55\pm0.20$&$14.84\pm$&$4.55\pm$\\
% % 
% % 
% &MI LB Opt~($\gamma=1000,\beta=300$)&$91.54\pm10.86$~($87.11\pm15.09$)&$-3.99\pm0.49$&$21.54\pm0.15$&$6.94\pm0.53$&$18.60\pm0.26$\\
% % 
% % 
% &MI LB Opt~($\gamma=300,\beta=1000$)&$\pm$~($\pm$)&$-4.65\pm1.11$&$\pm$&$\pm$&$\pm$\\
% 
% 
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{-4.2\pm1.2}$~($-9.5\pm0.2$)
&$\bs{30.2\pm1.1}$
% 
% &2.26
% 
&N.A.
% 
% &$34.5\pm0.2$
% 
% &$12.2\pm0.3$
&$\bs{75.3\pm16.5}$~($68.7\pm17.4$)
%&$46.62\pm0.17$
% &$16.57\pm0.75$
\\
% 
% 
% &MI Opt&&&&&\\
% 
\midrule
% 
Kernel-RkNN&M=100, $\alpha$=10\\
% \midrule
% &Random*&$83.13\pm15.76$~($78.57\pm17.38$)&$16.00\pm0.35$&$33.82\pm0.24$&$6.47\pm0.25$&$11.35\pm0.23$\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% 
% 
% % &
% &$16.0\pm0.3$
% &$27.4\pm0.4$
% % &$22.5\pm0.3$
% &$83.1\pm15.8$~($78.6\pm17.4$)
% % &$33.84\pm0.24$
% % &$6.49\pm0.27$
% % &$11.32\pm0.21$
% \\
% 
% 
% % &
% &$7.2\pm0.4$
% &$19.3\pm0.4$
% % &$13.5\pm0.3$
% &$87.6\pm15.8$~($84.3\pm17.4$)
% % &$25.58\pm0.19$
% % &$6.28\pm0.37$
% % &$12.13\pm0.17$
% \\
% % 
% 
% % &
% &$12.2\pm0.3$
% &$21.7\pm0.3$
% % &$16.8\pm0.2$
% &$87.6\pm14.6$~($83.9\pm16.8$)
% % &$26.19\pm0.17$
% % &$4.59\pm0.19$
% % &$9.42\pm0.14$
% \\
% % 
% 
% % &
% &$5.3\pm0.3$
% &$16.9\pm0.3$
% % &$9.8\pm0.4$
% &$90.5\pm13.5$~($87.2\pm15.9$)
% % &$21.35\pm0.27$
% % &$4.49\pm0.13$
% % &$11.53\pm0.23$
% \\
% 
% 
% &
&$9.9\pm0.4$~($4.3\pm0.2$)
&$19.9\pm0.3$
% 
% &2.3
% 
&0.50~(0.22)
% 
% &$10.0\pm0.2$
% 
% &$15.6\pm0.3$
&$88.3\pm13.9$~($84.7\pm16.0$)
% &$25.58\pm0.19$
% &$5.73\pm0.24$
\\
% 
% 
% \midrule
% 
% &MI LB Opt~($\gamma=100,\beta=300$)&$85.15\pm15.44$~($80.89\pm17.77$)&$7.43\pm0.90$&$30.46\pm0.19$&$9.43\pm0.88$&$13.60\pm$0.26&$21.03\pm$&$16.86\pm$\\
% % 
% % \midrule
% &MI LB Opt~($\gamma=300,\beta=300$)&$86.25\pm14.49$~($82.13\pm16.51$)&$11.26\pm0.48$&$29.17\pm0.21$&$7.45\pm0.46$&$10.46\pm0.12$&$21.72\pm$&$18.71\pm$\\
% % 
% % 
% &MI LB Opt~($\gamma=1000,\beta=300$)&$\pm$~($\pm$)&$8.03\pm0.28$&$\pm$&$\pm$&$11.59\pm$\\
% 
% 
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{13.5\pm0.4}$~($5.6\pm0.3$)
&$\bs{26.1\pm0.3}$
% 
% &2.4
% 
&0.52~(0.21)
% 
% &$12.6\pm0.2$
% 
% &$21.8\pm0.4$
&$82.7\pm16.2$~($78.4\pm17.3$)
% &$34.42\pm0.20$
% &$8.22\pm0.35$
\\
% 
% 
\midrule
% 
Kernel-RkNN&M=300, $\alpha$=10&\\
% \midrule
% &Random*&$87.61\pm15.24$~($84.11\pm17.02$)&$13.36\pm0.27$&$26.08\pm0.18$&$4.57\pm0.10$&$8.15\pm0.14$\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% % &
% &$13.4\pm0.2$
% &$21.6\pm0.2$
% % &$17.9\pm0.2$
% &$87.6\pm15.3$~($84.1\pm17.0$)
% % &$26.08\pm0.17$
% % &$4.51\pm0.13$
% % &$8.18\pm0.15$
% \\
% % 
% % &
% &$15.5\pm0.4$
% &$25.3\pm0.3$
% % &$22.6\pm0.3$
% &$84.0\pm15.6$~($79.6\pm17.3$)
% % &$32.45\pm0.17$
% % &$7.16\pm0.28$
% % &$9.82\pm0.24$
% \\
% % 
% &
&$\bs{15.3\pm0.2}$~($8.6\pm0.1$)
&$22.7\pm0.2$
%
% &1.8
% 
&\textbf{0.67~(0.38)}
% 
% &$7.4\pm0.2$
% 
% &$19.0\pm0.3$
&$87.6\pm14.7$~($83.9\pm16.6$)
% &$26.43\pm0.18$
% &$3.83\pm0.18$
\\
% 
% % &
% &$10.3\pm0.2$
% &$17.6\pm0.3$
% % &$14.2\pm0.3$
% &$90.6\pm12.1$~($87.3\pm14.8$)
% % &$21.49\pm0.20$
% % &$3.94\pm0.17$
% % &$7.28\pm0.16$
% \\
% % 
% % &
% &$15.3\pm0.5$
% &$24.6\pm0.5$
% % &$22.7\pm0.3$
% &$84.1\pm15.8$~($79.8\pm17.9$)
% % &$32.06\pm0.14$
% % &$7.43\pm0.47$
% % &$9.38\pm0.22$
% \\
% % 
% 
% \midrule
% &MI LB Opt~($\gamma=100,\beta=300$)&$82.97\pm17.36$~($79.03\pm19.01$)&$17.11\pm0.40$&$32.73\pm0.15$&$6.37\pm0.29$&$9.26\pm0.22$&$26.36\pm$&$23.47\pm$\\
% 
% 
% \midrule
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{15.7\pm0.3}$~($8.4\pm0.2$)
&$\bs{24.0\pm0.3}$
% 
% &1.9
% 
&0.65~(0.35)
% 
% &$8.3\pm0.2$
% 
% &$20.8\pm0.3$
&$85.8\pm16.0$~($82.0\pm17.6$)
% &$29.07\pm0.27$
% &$5.05\pm0.17$
\\
% 
% 
% \toprule
% \textbf{M=100}~(RMM, C=1.0)\\
% \midrule
% % &
% \textbf{Random}\\
% % Reference Set\\
% % 
% % &
% &$73.84\pm12.43$~($65.52\pm12.10$)&$21.63\pm0.62$
% &$52.10\pm0.25$&$13.97\pm0.68$&$16.50\pm0.40$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$23.89\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$23.55\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$24.00\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$25.25\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% \midrule
% % 
% % &
% \textbf{MI LB Opt}
% % ~($\gamma=100,\beta=1000$)
% &$73.55\pm11.36$~($65.00\pm11.08$)&$21.72\pm0.89$&$52.85\pm0.23$&$14.32\pm0.68$&$16.82\pm0.40$\\
% % 
% % 
% 
\midrule
% 
% \toprule
Kernel-RMM&M=100, $\alpha$=10\\
% ~(RMM, C=0.1)\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% 
% % &
% &$10.9\pm0.3$
% &$24.5\pm0.5$
% % &$23.8\pm0.6$
% &$84.2\pm11.7$~($77.4\pm13.0$)
% % &$37.48\pm0.46$
% % &$12.94\pm0.26$
% % &$13.69\pm0.44$
% \\
% % 
% % 
% % &
% &$14.4\pm0.3$
% &$26.4\pm0.4$
% % &$25.2\pm0.5$
% &$83.7\pm13.1$~($77.3\pm14.2$)
% %&$37.16\pm0.40$
% % &$10.76\pm0.18$
% % &$11.97\pm0.31$
% \\
% % 
% 
% &
&$10.0\pm0.5$~($3.5\pm0.1$)
&$23.2\pm0.3$
% 
% &2.9
% 
&0.43~(0.15)
% 
% &$13.3\pm0.4$
% 
% &$21.3\pm0.6$
&$85.9\pm11.5$~($79.3\pm13.3$)
%&$34.50\pm0.45$
% &$11.28\pm0.28$
\\
% 
% % 
% % &
% &$8.4\pm0.4$
% &$21.7\pm0.5$
% % &$20.1\pm0.6$
% &$86.8\pm10.6$~($80.2\pm12.9$)
% %&$33.46\pm0.40$
% % &$11.73\pm0.26$
% % &$13.39\pm0.43$
% \\
% % 
% % 
% % &
% &$7.2\pm0.4$
% &$20.7\pm0.6$
% % &$20.2\pm0.7$
% &$86.6\pm10.9$~($80.1\pm13.2$)
% % &$33.64\pm0.49$
% % &$12.98\pm0.29$
% % &$13.44\pm0.46$
% \\
% % 
% 
% \midrule
% 
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{11.4\pm0.5}$~($2.8\pm0.2$)
&$\bs{26.0\pm0.6}$
% 
% &\textbf{4.1}
% 
&\textbf{0.44~(0.11)}
% 
% &$14.6\pm0.4$
% 
% &$26.4\pm0.6$
&$\bs{82.0\pm11.6}$~($74.5\pm13.2$)
%&$40.96\pm0.41$
% &$15.01\pm0.37$
\\
% 
\midrule
% 
% \toprule
Kernel-RMM&M=300, $\alpha$=10\\
% ~(RMM, C=0.1)\\
% \midrule
% &
&&Random Sel.
% 
&$10.3\pm0.4$~($3.6\pm0.1$)
&$22.1\pm0.3$
&0.47~(0.16)
&$86.2\pm11.9$~($79.9\pm14.0$)
\\
% 
% 
\toprule
% 
Neural-RLSTM
&M=76000, $\alpha$=50
% \\
% 
% &&[10]-Random Selection&$6.7\pm0.3$&$27.1\pm0.5$
% &$68.3\pm10.7$~($62.9\pm9.5$)
% \\
% % 
% % 
% &&[10,10]-Manual Fine Tuned&$\bs{19.8}\pm1.0$&$34.2\pm0.2$
% &$\bs{63.4}\pm11.8$~($56.6\pm9.2$)
\\
% 
&&
% % [20,20]-MI LB Optimal
% MI LB Optimal
% &$\bs{19.1\pm0.7}$~($-0.5\pm0.4$)
% &$\bs{32.3}\pm0.5$
% &$13.2\pm0.2$
% &$61.4\pm13.7$~($56.4\pm11.1$)
% 
% 
% [16, 64, 16, 8]-MI LB Optimal
% 
MI LB Opt.
&$\bs{17.2\pm0.3}$~($8.0\pm0.2$)
&$23.2\pm0.3$
% 
% &2.2
% 
&\textbf{0.74~(0.34)}
% 
% &$6.0\pm0.1$
% 
&$84.6\pm17.2$~($79.9\pm19.9$)
\\
\toprule
\end{tabular}
% \vspace{-3.5mm}
\caption{
Evaluating the quality inference of dialogue responses (hashcodes), for the depression psychotherapy dataset.
}
\label{tab:results}
% \vspace{-5.5mm}
\end{table*}


% \begin{table*}[tp!]
% \centering
% \tabsize
% % \tiny
% % \scriptsize
% % \renewcommand{\arraystretch}{0.85}% Tighter
% % \renewcommand{\tabcolsep}{3pt}
% % 
% \begin{tabular}{lllllllllll}
% \toprule	
% \textbf{Configurations}
% % ~(Optimization)
% &\textbf{MI LB}
% &\textbf{Quality}&\textbf{Inference}
% &Accuracy~(Random Baseline)
% % Accuracy)\\
% % &Marginal E.&TC Bound&C.E. Bound
% \\
% \toprule
% \textbf{M=30~(RkNN)}\\
% % \midrule
% % &Random*&$82.61\pm17.85$~($77.84\pm20.55$)&$-13.83\pm1.57$&$33.49\pm0.12$&$17.45\pm1.54$&$29.88\pm0.12$\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % 
% % 
% % &
% &$-14.59\pm2.62$
% &$15.27\pm2.55$&$3.64\pm0.16$
% &$82.60\pm17.86$~($77.84\pm20.55$)
% %&$33.49\pm0.12$&$18.22\pm2.55$&$29.85\pm0.10$
% \\
% % 
% % 
% % &
% &$-11.47\pm4.64$
% &$5.73\pm4.70$&$1.67\pm0.52$
% &$93.56\pm8.54$~($89.45\pm12.14$)
% %&$18.87\pm0.36$&$13.14\pm4.69$&$17.20\pm0.37$
% \\
% % 
% % 
% % &
% &$-8.16\pm5.25$
% &$19.51\pm5.28$&$6.0\pm0.31$
% &$85.22\pm13.97$~($79.01\pm16.25$)
% %&$33.68\pm0.25$&$14.17\pm5.27$&$27.68\pm0.19$
% \\
% % 
% % 
% % &
% &$-9.71\pm0.95$
% &$5.58\pm1.02$&$1.06\pm0.37$
% &$93.70\pm10.50$~($90.41\pm14.24$)
% %&$16.36\pm0.27$&$10.78\pm0.98$&$15.30\pm0.25$
% \\
% % 
% % 
% % &
% &$-11.72\pm0.79$
% &$17.21\pm0.93$&$3.35\pm0.28$
% &$85.16\pm15.54$~($79.79\pm18.21$)
% %&$32.27\pm0.19$&$15.06\pm0.91$&$28.92\pm0.20$
% \\
% %
% % 
% % &&$\pm$~($\pm$)&$-7.88\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$-9.38\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$-6.04\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% % 
% \midrule
% % 
% % 
% % &MI LB Opt~($\gamma=100,\beta=300$)&$87.27\pm15.80$~($82.90\pm18.51$)&$-6.66\pm0.39$&$27.22\pm0.25$&$10.72\pm0.42$&$23.16\pm0.27$&$16.5\pm$&$4.06\pm$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=300,\beta=300$)&$90.42\pm11.44$~($85.75\pm14.88$)&$-4.71\pm0.65$&$24.10\pm0.25$&$9.26\pm0.64$&$19.55\pm0.20$&$14.84\pm$&$4.55\pm$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=1000,\beta=300$)&$91.54\pm10.86$~($87.11\pm15.09$)&$-3.99\pm0.49$&$21.54\pm0.15$&$6.94\pm0.53$&$18.60\pm0.26$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=300,\beta=1000$)&$\pm$~($\pm$)&$-4.65\pm1.11$&$\pm$&$\pm$&$\pm$\\
% % 
% % 
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$-4.41\pm0.77$
% &$30.05\pm0.77$&$12.16\pm0.28$
% &$75.27\pm16.48$~($68.73\pm17.42$)
% %&$46.62\pm0.17$&$16.57\pm0.75$&$34.46\pm0.22$
% \\
% % 
% % 
% % &MI Opt&&&&&\\
% \toprule
% \textbf{M=100~(RkNN)}\\
% % \midrule
% % &Random*&$83.13\pm15.76$~($78.57\pm17.38$)&$16.00\pm0.35$&$33.82\pm0.24$&$6.47\pm0.25$&$11.35\pm0.23$\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % 
% % 
% % &
% &$16.03\pm0.28$
% &$27.35\pm0.36$&$22.52\pm0.32$
% &$83.12\pm15.77$~($78.56\pm17.38$)
% % &$33.84\pm0.24$&$6.49\pm0.27$&$11.32\pm0.21$
% \\
% % 
% % 
% % &
% &$7.17\pm0.41$
% &$19.30\pm0.42$&$13.45\pm0.25$
% &$87.56\pm15.77$~($84.26\pm17.40$)
% % &$25.58\pm0.19$&$6.28\pm0.37$&$12.13\pm0.17$
% \\
% % 
% % 
% % &
% &$12.18\pm0.30$
% &$21.7\pm0.25$&$16.77\pm0.22$
% &$87.64\pm14.60$~($83.89\pm16.78$)
% % &$26.19\pm0.17$&$4.59\pm0.19$&$9.42\pm0.14$
% \\
% % 
% % 
% % &
% &$5.33\pm0.28$
% &$16.86\pm0.30$&$9.82\pm0.35$
% &$90.45\pm13.54$~($87.18\pm15.88$)
% % &$21.35\pm0.27$&$4.49\pm0.13$&$11.53\pm0.23$
% \\
% % 
% % 
% % &
% &$9.82\pm0.41$
% &$19.85\pm0.31$&$15.55\pm0.28$
% &$88.29\pm13.90$~($84.64\pm16.05$)
% % &$25.58\pm0.19$&$5.73\pm0.24$&$10.03\pm0.21$
% \\
% % 
% % 
% \midrule
% % 
% % &MI LB Opt~($\gamma=100,\beta=300$)&$85.15\pm15.44$~($80.89\pm17.77$)&$7.43\pm0.90$&$30.46\pm0.19$&$9.43\pm0.88$&$13.60\pm$0.26&$21.03\pm$&$16.86\pm$\\
% % % 
% % % \midrule
% % &MI LB Opt~($\gamma=300,\beta=300$)&$86.25\pm14.49$~($82.13\pm16.51$)&$11.26\pm0.48$&$29.17\pm0.21$&$7.45\pm0.46$&$10.46\pm0.12$&$21.72\pm$&$18.71\pm$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=1000,\beta=300$)&$\pm$~($\pm$)&$8.03\pm0.28$&$\pm$&$\pm$&$11.59\pm$\\
% % 
% % 
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$13.58\pm0.45$
% &$26.20\pm0.40$&$21.79\pm0.35$
% &$82.74\pm16.15$~($78.35\pm17.30$)
% % &$34.42\pm0.20$&$8.22\pm0.35$&$12.63\pm0.29$
% \\
% % 
% % 
% \toprule
% \textbf{M=300~(RkNN)}\\
% % \midrule
% % &Random*&$87.61\pm15.24$~($84.11\pm17.02$)&$13.36\pm0.27$&$26.08\pm0.18$&$4.57\pm0.10$&$8.15\pm0.14$\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % &
% &$13.39\pm0.24$
% &$21.57\pm0.21$&$17.90\pm0.23$
% &$87.62\pm15.27$~($84.11\pm17.03$)
% % &$26.08\pm0.17$&$4.51\pm0.13$&$8.18\pm0.15$
% \\
% % 
% % &
% &$15.48\pm0.35$
% &$25.29\pm0.33$&$22.63\pm0.29$
% &$83.99\pm15.60$~($79.59\pm17.33$)
% % &$32.45\pm0.17$&$7.16\pm0.28$&$9.82\pm0.24$
% \\
% % 
% % &
% &$15.19\pm0.26$
% &$22.6\pm0.25$&$19.02\pm0.26$
% &$87.60\pm14.74$~($83.87\pm16.59$)
% % &$26.43\pm0.18$&$3.83\pm0.18$&$7.41\pm0.19$
% \\
% % 
% % &
% &$10.28\pm0.23$
% &$17.55\pm0.26$&$14.21\pm0.26$
% &$90.63\pm12.11$~($87.32\pm14.77$)
% % &$21.49\pm0.20$&$3.94\pm0.17$&$7.28\pm0.16$
% \\
% % 
% % &
% &$15.26\pm0.49$
% &$24.63\pm0.49$&$22.68\pm0.26$
% &$84.05\pm15.77$~($79.79\pm17.89$)
% % &$32.06\pm0.14$&$7.43\pm0.47$&$9.38\pm0.22$
% \\
% % 
% % 
% \midrule
% % &MI LB Opt~($\gamma=100,\beta=300$)&$82.97\pm17.36$~($79.03\pm19.01$)&$17.11\pm0.40$&$32.73\pm0.15$&$6.37\pm0.29$&$9.26\pm0.22$&$26.36\pm$&$23.47\pm$\\
% % 
% % 
% % \midrule
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$15.71\pm0.27$
% &$24.02\pm0.32$&$20.77\pm0.32$
% &$85.82\pm16.03$~($82.04\pm17.56$)
% % &$29.07\pm0.27$&$5.05\pm0.17$&$8.30\pm0.18$
% \\
% % 
% % 
% % \toprule
% % \textbf{M=100}~(RMM, C=1.0)\\
% % \midrule
% % % &
% % \textbf{Random}\\
% % % Reference Set\\
% % % 
% % % &
% % &$73.84\pm12.43$~($65.52\pm12.10$)&$21.63\pm0.62$
% % &$52.10\pm0.25$&$13.97\pm0.68$&$16.50\pm0.40$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$23.89\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$23.55\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$24.00\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$25.25\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % \midrule
% % % 
% % % &
% % \textbf{MI LB Opt}
% % % ~($\gamma=100,\beta=1000$)
% % &$73.55\pm11.36$~($65.00\pm11.08$)&$21.72\pm0.89$&$52.85\pm0.23$&$14.32\pm0.68$&$16.82\pm0.40$\\
% % % 
% % % 
% % 
% \toprule
% % 
% % \toprule
% \textbf{M=100~(RMM)}\\
% % ~(RMM, C=0.1)\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % 
% % &
% &$10.85\pm0.26$
% &$24.54\pm0.53$&$23.79\pm0.64$
% &$84.23\pm11.66$~($77.36\pm13.04$)
% % &$37.48\pm0.46$&$12.94\pm0.26$&$13.69\pm0.44$
% \\
% % 
% % 
% % &
% &$14.43\pm0.33$
% &$26.4\pm0.44$&$25.19\pm0.51$
% &$83.74\pm13.10$~($77.30\pm14.18$)
% %&$37.16\pm0.40$&$10.76\pm0.18$&$11.97\pm0.31$
% \\
% % 
% % 
% % &
% &$9.97\pm0.50$
% &$23.22\pm0.53$&$21.25\pm0.62$
% &$85.92\pm11.49$~($79.35\pm13.28$)
% %&$34.50\pm0.45$&$11.28\pm0.28$&$13.25\pm0.43$
% \\
% % 
% % 
% % &
% &$8.35\pm0.40$
% &$21.73\pm0.48$&$20.07\pm0.59$
% &$86.78\pm10.57$~($80.18\pm12.92$)
% %&$33.46\pm0.40$&$11.73\pm0.26$&$13.39\pm0.43$
% \\
% % 
% % 
% % &
% &$7.23\pm0.44$
% &$20.66\pm0.57$&$20.20\pm0.67$
% &$86.58\pm10.90$~($80.09\pm13.16$)
% % &$33.64\pm0.49$&$12.98\pm0.29$&$13.44\pm0.46$
% \\
% % 
% % 
% \midrule
% % 
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$11.35\pm0.48$
% &$25.95\pm0.55$&$26.36\pm0.60$
% &$81.99\pm11.62$~($74.53\pm13.21$)
% %&$40.96\pm0.41$&$15.01\pm0.37$&$14.60\pm0.44$
% \\
% % 
% % % 
% % 
% % 
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation of
% % for our approach of 
% inferencing dialog responses as hashcodes.
% }
% \label{tab:results}
% \vspace{-6.5mm}
% \end{table*}


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/proofsContent.tex <==
% \section{Theorems for Information Theoretic Bounds}
% \begin{theorem}[Lower Bound for Mutual Information]
% Mutual information between two hashcode distributions, $\cI(\bs{\cC_t}: \bs{\cC_p}; M_h)$, is lower bounded as,     
% % 
% % 
% % \vspace{-3mm}
% \begin{align}
% &
% % \csizenine
% \cI(\bs{\cC_t}: \bs{\cC_p}; M_h)
% % \nonumber
% % \\
% % &
% % &
% \ge
% % \nonumber
% % \\
% % &
% % \csizenine
% % \underbrace{
% \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% -
% \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% % }_{\text{quality of hashcodes as representations}}
% \nonumber
% \\
% &
% % \csizenine
% +
% % \underbrace{
% \sum\limits_j{\left\langle \log q(\bs{\cC_t}(j)|\bs{\cC_p}; M_h)
% \right\rangle_{p(\bs{\cC_t}(j),\bs{\cC_p}; M_h)}}.
% % }_{\text{inference of each hashcode bit}}
% \label{eqn:mi_lb}
% % \vspace{-4mm}
% \end{align}
% % 	
% \noindent The lower bound is cheaper and more accurately computable than the criterion itself.
% % 
% % \vspace{-3mm}
% \begin{align}
% \bs{\cY^*}
% \gets
% \mathop{\arg\max}
% \limits_{\bs{\cY}:|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t}:\bs{\cY}; M_h)
% \label{eqn:corex_opt_thm}
% % \vspace{-4.5mm}
% \end{align}
% % 
% % 
% Herein, $\cT\cC(\bs{\cC_t}:\bs{\cY}; M_h)$ describes the amount of \emph{Total Correlations~(Multi-variate Mutual Information)}~\footnote{The ``total correlation" quantity, also called as multi-variate Mutual Information, or multi-information, was defined in \cite{watanabe1960information,studeny1998multiinformation,kraskov2005hierarchical}.} within $\bs{\cC_t}$ that can be explained by a latent variables representation $\bs{\cY}$; $q(\bs{\cC_t}(j)|\bs{\cC_p}; M_h)$ is a proposal conditional distribution for the $j_{th}$ bit of therapist hashcodes built using a classifier, like a random forest, neural network, etc.
% % 
% % 
% % 
% % \todo{explain the other terms as well.}
% % ~\cite{greg2014discovering}.
% \label{thm:mi_lb}
% % \vspace{-3mm}
% \end{theorem}
	
% % An interesting aspect of the quantity $\cT\cC(\bs{\cC}: \bs{\cY}; M_h)$ is that one can compute $\cT\cC(\bs{\cC}: \bs{\cY}; M_h)$ efficiently 
% % % if $\bs{\cY}$ is such that it maximizes the quantity, i.e., when
% % for optimized $\bs{\cY}$ that explains maximum possible Total Correlations present in $\bs{\cC}$; see \cite{greg2014discovering} for more details on the optimization.
	
% % % In this scenario, $p(\bs{c}|\bs{y}; M_h)$ factorizes, as per the \emph{Naive Bayes} model $p(\bs{c}|\bs{y}; M_h)=\prod_{j}p(\bs{c}(j)|\bs{y}; M_h)$, thus making the optimization of the quantity computationally tractable in \eqnref{eqn:corex_opt_thm}~\cite{greg2014discovering}.
	
% % % \todo{maximizing the lower bound, expecting that the actual quantity should also increase. In certain conditions, if the bound is not tight, mutual information may not increase. however, the good thing is that the lower bound itself is a good objective function, characterizing our goals for the hashing model.}

% % As we observed for the mutual information criterion above, we can also see different terms in the mutual information lower bound having varying roles for the optimization; for instance, the first two terms in \eqnref{eqn:mi_lb} contribute to improve the quality of hashcodes as representations, i.e. maximizing entropy of each hashcode bit while discouraging redundancies between the bits, and the last term of conditional entropies is for improving inference of hashcode bits individually.
	
% % % From the above discussion, we understand that it is very challenging to compute mutual information between two high dimensional variables in practice which is why we proposed a novel lower bound on the mutual information criterion as the objective function to optimize a hashing model for the dialog modeling problem. 
% % % 
% % We argue to use the proposed MI lower bound, for not only optimizing hashing for dialog modeling, but also as an \emph{evaluation metric quantifying the representation quality as well as the inference of hashcodes}. Further, for evaluating representation quality of hashcodes separately,  
% % % 
% % % the lower bound expression involves terms  which can be used for evaluating individually, (i) the inference of hashcodes, and (ii) the representation quality of hashcodes. 
% % % 
% % % \textbf{Evaluating Representation Quality of Hashcodes: 
% % % with Our Tight Upper Bound on Entropy
% % % }
% % % 
% % in \thmref{thm:entropy_ub} below,
% % we present a novel tight upper bound for joint entropy of hashcodes.
% % % 
% % on the therapist hashcodes which we propose to use as a metric for evaluating the representation quality of hashcodes.
% % ~(a surrogate to the entropy term). 
% \begin{theorem}[Upper Bound for Entropy]
% % The expression, $\sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% % -
% % \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)$, that corresponds to the first two terms in the lower bound in \thmref{thm:mi_lb},
% % % representing the quality of hashcodes, 
% % is an upper bound on the 
% % 
% Joint entropy of hashcodes, $\cH(\bs{\cC_t}; M_h)$, is upper bounded as,
% % 
% % with the gap between the bound and the entropy term itself, equal to the conditional total correlation term, $\cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)$.
% % 
% % \vspace{-2mm}
% \begin{align*}
% \cH(\bs{\cC_t}; M_h)
% \leq
% \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% -
% \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% ;
% \\
% \bs{\cY^*}
% \gets
% \mathop{\arg\max}
% \limits_{\bs{\cY}:|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t}:\bs{\cY}; M_h)
% % 
% % \vspace{-4mm}
% \end{align*}
% % 
% % \begin{proof}
% % From the definition of Total Correlation above, we have the following.
% % % 
% % \begin{align*}
% % &
% % \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% % -
% % \cT\cC(\bs{\cC_t}; M_h)
% % =
% % \cH(\bs{\cC_t}; M_h)
% % \\
% % &
% % \cT\cC(\bs{\cC_t}; M_h)
% % =
% % \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% % +
% % \cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)
% % \end{align*}
% % 
% % From these two equations above, we can easily derive the expression as below.
% % % 
% % \begin{align*}
% % &
% % \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% % -
% % \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% % \\
% % &=
% % \cH(\bs{\cC_t}; M_h)
% % +
% % \cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)
% % \end{align*}
% % % 
% % From this derived expression, we can simply obtain the upper bound and the corresponding gap.
% % \end{proof}
% \label{thm:entropy_ub}
% % \vspace{-4.5mm}
% \end{theorem}
% % 
% % Note the similarities between the expressions for proposed the mutual information lower bound, and the joint entropy upper bound; the first two terms match between the two expressions.
% % % 
% % For $\cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)=0$, i.e. when a latent representation $\bs{\cY^*}$ is learned which explains all the total correlations in $\bs{\cC_t}$, the upper bound becomes equal to the entropy term; practically, for the case of hashcodes, learning such a representation should not be too difficult, so the bound should be very tight. This is quite interesting as we are able to judge the representation quality of hashcodes, that we proposed to quantify via the entropy of hashcodes in the above, through the tight upper bound in \thmref{thm:entropy_ub} which is much easier and cheap/accurate to compute than the entropy term itself. Besides the mutual information lower bound, for more detailed analysis, \emph{we propose to use the upper bound as an evaluation metric} for the dialog problem when modeling via hashing functions. 

% % % It is important to 
% % % Note that 
% % The proposed information theoretic bounds are generically applicable for any high dimensional variables.
% % % , beyond the domains of hashcodes, NLP, psychiatry which we considered in this paper.

% % See supplementary material for derivation of the bounds. Next, in  \secref{sec:opt_hash_details}, we discuss details on how to optimize a kernel- or neural-hashing, as per \algoref{alg:our_algo_klsh_codes}, by maximizing the MI LB.
% % \vspace{-2mm}
% 
% 
% 
\section{Derivations of the Information Theoretic Bounds
% LB and Entropy UB
% Derivation
}
\label{sec:bounds_deriv}
% \vspace{-2mm}
% 
Before the discussion of our novel lower bound of mutual information, we introduce the information-theoretic quantity called \textit{Total Correlation}~($\mathcal{TC}$), which captures non-linear correlation among the dimensions of a random variable $\bs{C}$, i.e., 
% 
% \vspace{-2mm}
\begin{align}
&
\cT\cC(\bs{C}) = \sum\limits_j \cH(C_j) - \cH(\bs{C});
\vspace{-4mm}
\end{align}
% 		
For a 2-D random variable, total correlation corresponds to mutual information quantity itself. 
And, $\cT\cC(\bs{C}: \bs{Y})$ is defined as,
% 
\vspace{-3mm}
\begin{align}
\nonumber
\\
&
\cT\cC(\bs{C}: \bs{Y}) = \cT\cC(\bs{C}) - \cT\cC(\bs{C}|\bs{Y}).
\label{eqn:corex}
% \vspace{-4mm}
\end{align}
% 
Intuitively, \eqnref{eqn:corex} describes the amount of information within $\bs{C}$ that can be explained by $\bs{Y}$.
% 
% The interesting aspect of this quantity $\cT\cC(\bs{\cX}: \bs{\cY}; M_h)$ is that one can compute $\cT\cC(\bs{\cX}: \bs{\cY}; M_h)$ efficiently for $\bs{\cY}$ is such that it maximizes the quantity, i.e., when $\bs{\cY}$ explains all the correlations present in $\bs{\cX}$. In this scenario, $p(\bs{x}|\bs{y}; M_h)$ factorizes, as per the \emph{Naive Bayes} model $p(\bs{x}|\bs{y}; M_h)=\prod_{j}p(\bs{x}(j)|\bs{y}; M_h)$, thus making the computations cheap~\cite{greg2014discovering}. 

Along these lines, the mutual information quantity between the hashcodes can be decomposed as in \lmaref{lma:mi_decompose} below.
% 	
% \vspace{-1mm}
\begin{lemma}[Mutual Information Decomposition]
\label{lma:mi_decompose}
Mutual Information between $\bs{C^t}$ and $\bs{C^p}$ is decomposed as follows:
% 
% \vspace{-3mm}
\begin{align}
&
\cI(\bs{C^t}: \bs{C^p})
% \nonumber
% \\
% &
% = \cH(\bs{\cC_t}; M_h) - \cH(\bs{\cC_t} | \bs{\cC_p}; M_h)
% 
% \nonumber\\
% &= \sum\limits_i {\cH(\bs{\cC_t}(i))}-\sum\limits_i {\cH(\bs{\cC_t}(i) | \bs{\cC_p})} \nonumber \\
% &~~~~
% + \cH(\bs{\cC_t}) - \cH(\bs{\cC_t} | \bs{\cC_p}) \nonumber \\
% &~~~~
% - \sum\limits_i {\cH(\bs{\cC_t}(i))}
% +
% \sum\limits_i {\cH(\bs{\cC_t}(i) | \bs{\cC_p})} \nonumber \\
% &
% = \sum\limits_i {\cI(\bs{\cC_t}(i): \bs{\cC_p})} - (\cT\cC(\bs{\cC_t}) - \cT\cC(\bs{\cC_t}|\bs{\cC_p})) 
\nonumber 
\\
&
= \sum\limits_j {\cI(C^t_j: \bs{C^p})} -
\cT\cC(
\bs{C^t}: \bs{C^p}).
\label{eqn:deco_mi}
% \vspace{-3mm}
\end{align}
% \vspace{-4.5mm}
\begin{proof}
\begin{align*}
\cI(\bs{C^t}: \bs{C^p})
&
= \cH(\bs{C^t}) - \cH(\bs{C^t} | \bs{C^p})
\nonumber \\
&
= 
\sum\limits_j
\cH(C^t_j) 
- 
\sum\limits_j
\cH(C^t_j | \bs{C^p})
+ \cH(\bs{C^t}) 
\nonumber \\
&
- \cH(\bs{C^t} | \bs{C^p})
- \sum\limits_j {\cH(C^t_j)}
+
\sum\limits_i {\cH(C^t_i | \bs{C^p})} \nonumber \\
&
= \sum\limits_j {\cI(C^t_j: \bs{C^p})} - (\cT\cC(\bs{C^t}) - \cT\cC(\bs{C^t}|\bs{C^p}))
\nonumber 
\\
&
= \sum\limits_j {\cI(C^t_j: \bs{C^p})} -
\cT\cC(
\bs{C^t}: \bs{C^p}).
\end{align*}
\end{proof}
\end{lemma}
% 	
% \noindent wherein $\bs{\cC_t}(j)$ denotes the $j_{th}$ dimension of $\bs{\cC_t}$ in \eqnref{eqn:deco_mi}.
% 		
Looking at the first term of RHS in \eqnref{eqn:deco_mi}, it is the mutual information between a one-dimensional and multi-dimensional random variable. 

For these terms, since one of the variables is only 1-D, we can use the existing technique of variational bounds for an approximation, as in \lmaref{lma:variational_lb_mi} below.
% 					
% \vspace{-1.0mm}
\begin{lemma}
\label{lma:variational_lb_mi}
Marginal mutual information for each bit in therapist hashcodes, $\cI(C^t_j: \bs{C^p})$, is lower bounded as,
% 
% \vspace{-3mm}
\begin{align}
% &
\cI(C^t_j: \bs{C^p}) 
\ge 
% \nonumber
% \\
% &
\cH(C^t_j)
+
\left\langle \log q(C^t_j|\bs{C^p})
\right\rangle_{p(C^t_j,\bs{C^p})}.
\label{eqn:vmi}
% \vspace{-3mm}
\end{align}
% 
% \todo{mention, we simply use a variational upper bound on the marginal conditional entropy term. Mention the bound gap.}
% 
\label{lma:marginal_mi_lb}
% \vspace{-5.5mm}
\end{lemma}
% 	
\noindent Herein, $\cH(C^t_j)$ is easy to compute because $C^t_j$ is a one-dimensional binary variable. For each of the proposal distributions $q(C^t_j|\bs{C_p})$, we propose to use a Random Forest~(RF) classifier~\cite{gao2016variational}.
            		
In reference to the second term of RHS in \eqnref{eqn:deco_mi}, 
% as mentioned above, 
it is computationally intractable to compute the total correlation expression $\cT\cC(\bs{C^t}:\bs{C^p})$, which denotes the total correlations between bits of $\bs{C^t}$, explainable by $\bs{C^p}$. So, we would also like to obtain an upper bound of $\cT\cC(\bs{C^t}:\bs{C^p})$, which is cheap to compute, that would give us a lower bound for the second term in \eqnref{eqn:deco_mi} because of the negative sign.
% 		
\begin{lemma}
$\cT\cC(\bs{C^t}:\bs{C^p})$ is upper bounded as: 
% \vspace{-2mm}
\begin{align}
\cT\cC(\bs{C^t}:\bs{C^p})
\leq
\cT\cC(\bs{C^t}:\bs{Y^*})
\label{eqn:corex_lb}
% \vspace{-4mm}
\end{align}
% 	
% \begin{align}
% \bs{\cY^*}
% \gets
% \mathop{\arg\max}
% \limits_{\bs{\cY}:|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t}:\bs{\cY}; M_h),
% \label{eqn:corex_opt}
% \end{align}
% 	
% To obtain the upper bound, we aim to solve the optimization problem in \eqnref{eqn:corex_opt} and obtain,
% 	
% 				
\noindent wherein $|.|$ denotes the dimensionality of a random variable.
% in \eqnref{eqn:corex_lb}. 
\label{lma:tc_ub}
% \vspace{-4mm}
\end{lemma}
% 		
% As mentioned previously, 
Although it is intractable to compute the original term $\cT\cC(\bs{C^t}:\bs{C^p})$, it is possible to compute $\cT\cC(\bs{C^t}:\bs{Y^*})$ for a latent variable representation $\bs{Y^*}$ of $\bs{C^t}$ that maximally explains the Total Correlations in $\bs{C^t}$.
% ~\eqnref{eqn:corex_opt}.

% 	
% We discuss more details on obtaining such latent representation in the following.
% 
% 	
We can think of the computation of the upper bound as an unsupervised learning problem. We propose to use an existing algorithm, \emph{CorEx}, for the unsupervised learning of latent random variables representation $\bs{Y^*}$~\cite{greg2014discovering}.
	
% \begin{align}
% \cI(\bs{\cC_t}: \bs{\cC_p}) \ge \sum\limits_i{\cH(\bs{\cC_t}(i)) + \left\langle \log q(\bs{\cC_t}(i)|\bs{\cC_p})\right\rangle_{p(\bs{\cC_t}(i),\bs{\cC_p})}} 
% \\
% - \mathop{\max }\limits_{|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t};\bs{\cY})
% \label{eqn:mi_lb}
% \end{align}

% We can view the last term of RHS in Eq.~\ref{eqn:mi_lb} 
		
It is important to note some practical considerations about the upper bound. In the case of a suboptimal solution to the maximization of $\cT\cC(\bs{C^t}:\bs{Y})$ above, the optimized quantity may not be an upper bound of $\cT\cC(\bs{C^t}:\bs{C^p})$, but rather an approximation. Also, the upper bound would not be tight if $\bs{C^p}$ doesn't explain much of total correlations in $\bs{C^t}$. Further, for even more computation cost reductions during the learning, the dimension of the latent representation $\bs{Y}$ can be kept much smaller than the dimension of hashcodes, i.e. $|\bs{Y}| \ll |\bs{C^p}|$ for $|\bs{C^p}| \gg 1$; this is because even a small number of latent variables should explain most of the total correlations for practical purposes as demonstrated by \cite{greg2014discovering}, and observed in our experiments on hashcodes as well.
		
% \todo{we can keep size of $\cY$ small as many of the remaining latent variables would contribute very low value.}
	
Combining \eqnref{eqn:vmi} and \eqnref{eqn:corex_lb} into \eqnref{eqn:deco_mi}, we get the lower bound in \thmref{thm:mi_lb}.
		    
% \input{theorem_milb.tex}

Along same lines, we can derive the tight upper bound on joint entropy of hashcodes so as to obtain the normalization of the MI LB.
% 
From the definition of Total Correlation above~\eqnref{eqn:corex}, we have the following,
% 
% \vspace{-2.5mm}
\begin{align*}
&
\sum\limits_j{\cH(C^t_j)}
-
\cT\cC(\bs{C^t})
=
\cH(\bs{C^t}),
\\
&
\cT\cC(\bs{C^t})
=
\cT\cC(\bs{C^t}:\bs{Y^*})
+
\cT\cC(\bs{C^t}|\bs{Y^*}),
% \vspace{-4mm}
\end{align*}
% 
and finally the expression below.
% 
% \vspace{-3mm}
\begin{align*}
&
\sum\limits_j{\cH(C^t_j)}
-
\cT\cC(\bs{C^t}:\bs{Y^*})
\\
&=
\cH(\bs{C^t})
+
\cT\cC(\bs{C^t}|\bs{Y^*})
% \vspace{-3mm}
\end{align*}
% 
From this derived expression, we can simply obtain the upper bound and the corresponding gap.
        
\textbf{Previous Lower Bounds for Mutual Information: 
% outside Dialog Modeling Settings
}
Variational lower bounds on the mutual information criterion have been proposed in the past ~\cite{barber2003algorithm,chalk2016relevant,gao2016variational,chen2016infogan,alemi2017deep,garg2018efficient}.
% for settings where one of the two variables is fixed~(say class labels).
% 
% In these settings, for the mutual information lower bound, one needs to only obtain a variational upper bound on the conditional entropy term, while ignoring the entropy term as a constant. This simplifies the derivation significantly, compared to our setting. In our setting, we can not ignore the entropy term as it is a variable. 
% 
% % The idea of variational lower bound for our mutual information objective would not work as such, since neither of the two high-dimensional variables is fixed, but instead functionals of the hashing model, as we explain in the following.
% % ; we will now describe  the computation of the variational lower bound.
% % 
% % 
% % 
% % 	
% % The mutual information  is expressed in terms of the entropy of $\bs{\cC_t}$, and the conditional  entropy of $\bs{\cC_t}$ given the hash codes of patients $\bs{\cC_p}$. 
% For high-dimensional hashcodes, computing $p(\bs{\cC_t}|\bs{\cC_p}; M_h)$ is intractable, and so the computing the conditional entropy term, $\cH(\bs{\cC_t}|\bs{\cC_p}; M_h)$. However, one can use instead a \emph{proposal distribution}, $q(\bs{\cC_t}|\bs{\cC_p}; M_h)$, approximating  $p(\bs{\cC_t}|\bs{\cC_p}; M_h)$, that is cheaper to compute. This leads to the variational lower bound, with tightness of the bound depending upon KL-divergence between the proposal distribution and the true conditional distribution.
% % 
% \begin{align*}
% &
% \cI(\bs{\cC_t}: \bs{\cC_p}; M_h) = \cH(\bs{\cC_t}; M_h) - \cH(\bs{\cC_t} | \bs{\cC_p}; M_h)
% \\
% &
% = \cH(\bs{\cC_t}; M_h) + \left\langle \log p(\bs{\cC_t}|\bs{\cC_p}; M_h)\right\rangle_{p(\bs{\cC_t},\bs{\cC_p}; M_h)}
% \\
% &
% % \cI(\bs{\cC_t}: \bs{\cC_p}; M_h) 
% \geq 
% \cH(\bs{\cC_t}; M_h) 
% + 
% \left\langle \log q(\bs{\cC_t}|\bs{\cC_p}; M_h)
% \right\rangle_{p(\bs{\cC_t},\bs{\cC_p}; M_h)}
% \end{align*}
% 
% 
Their lower bounds works only when one of the variables is fixed, say if $\bs{C^t}$ were fixed. In our objective, not only $\bs{C^t}$ is a functional of the hashing model that we are learning, it is high dimensional. Unless we have a lower bound for the entropy term $\cH(\bs{C^t})$ as well, which should be hard to obtain, we can not use the above mentioned variational lower bounds for our problem as such.
% 
% However, if we apply the variational lower bound directly, the entropy term $\cH(\bs{\cC_t})$ involves high-dimensional variables and is not easy to compute. 
Besides, it is also non-trivial to find an appropriate proposal distribution $q(\bs{C^t}|\bs{C^p})$. Therefore, we adopt a different approach for obtaining a novel lower bound on the mutual information quantity, as described above.

\section{Pseudo Code of Algorithms To Optimize LSH for Dialog Modeling}
% 

In the following, we discuss the optimization of the reference set.
		
{ \bf Optimizing Reference Set. \\}
% 	
\begin{algorithm*}[th]
\caption{
% \small
\csizenine
Optimizing Reference Set in LSH-RkNN or LSH-RMM for Dialogue Modeling 
% by Maximizing Our MI LB
}
% \scriptsize
% \csize
% \small
\csizenine
% 
\begin{algorithmic}[1]
\REQUIRE Training set $\bar{\bs{S}} = \{\bs{S}^p,\bs{S}^t\}$; initial and final size of reference set, $I$ and $M$ respectively; $\beta$ and $\gamma$ are the number of samples, as candidates for the reference set, and for computing the lower bound, respectively.
% \\
% \STATE $\bar{\bs{S}} = \{ S_1^p, \cdots, S_N^p, S_1^t, \cdots, S_N^t \}$
% \COMMENT{patient \& therapist responses in same set as candidates for the reference set}
% % 
% \\
% \STATE $\bs{S}^p = \{ S_1^p, \cdots, S_N^p \}$
% \COMMENT{patient responses}
% % 
% \\
% \STATE $\bs{S}^t = \{ S_1^t, \cdots, S_N^t \}$
% \COMMENT{therapist responses}
% 
\\
\STATE $\bs{r}^d$ $\gets$ randomSubset($2N$, $I$)
\COMMENT{random subset of indices, of size $I$, from $\{ 1, \cdots, 2N \}$ for initialization of reference set}
\\
\COMMENT{optimizing the reference set up to size $M$ greedily}
\FOR{$j=1 \to M$}
% 
% \\
% \COMMENT{Optimize $j^{th}$ element in the reference set}
% 
\IF{$j > I$}
\STATE $\bs{r}^d \gets \{ \bs{r}^d, randomSubset($2N$, 1) \}$
\COMMENT{adding one more element in the reference set, that is to be optimized}
\ENDIF
% 
\STATE $\bs{r}^{ref}$ $\gets$ randomSubset($2N$, $\beta$)\COMMENT{subset of the structures as candidates for the reference set}
% 
\STATE $\bs{r}^{lb}$ $\gets$ randomSubset($N$, $\gamma$)\COMMENT{subset of patient/therapist responses pairs for computing the MI lower bound}
% 
\STATE $\bs{K}^p \gets$ computeKernel($\bs{S}^p(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{d})$)
\COMMENT{$\gamma \!\!\times\!\! j$ size}
% 
\STATE $\bs{K}^t \gets$ computeKernel($\bs{S}^t(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{d})$)
\COMMENT{$\gamma \!\!\times\!\! j$ size}
% 
\STATE $\bar{\bs{K}}^p \gets$ computeKernel($\bs{S}^p(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{ref})$)
\COMMENT{$\gamma \!\!\times\!\! \beta$ size}
% 
\STATE $\bar{\bs{K}}^t \gets$ computeKernel($\bs{S}^t(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{ref})$)
\COMMENT{$\gamma \!\!\times\!\! \beta$ size}
% 
% \STATE $\bs{mi}_{lb}$ $\gets$ $\bs{0}$
% 
\STATE $\bs{mi}_{lb}$ $\gets$ computeMILowerBound($\bs{K}^p, \bs{K}^t, \bar{\bs{K}}^p, \bar{\bs{K}}^t$)
\COMMENT{compute the MI lower bound for all the candidates $\bar{\bs{S}}(\bs{r}^{ref})$, using the kernel matrices, via computation of hashcodes}
% 
% \FOR{$l=1 \to \beta$}
% 
% \STATE $\bs{C}^p \gets$ computeKernelHashcodes($\bs{K}^p$)
% 
% \STATE $\bs{C}^t \gets$ computeKernelHashcodes($\bs{K}^t$)
% 
% \STATE $\bs{mi}_{lb}(l)$ $\gets$ computeMILowerBound($\bs{S}(\bs{r}^{lb})$)
% 
% \ENDFOR
% 
\STATE $\bs{r}^{d}(j)$ $\gets$ maxMILBDataIndex($\bs{mi}_{lb}$, $\bs{r}^{ref}$)
\COMMENT{choose the index with maximum value of MI lower bound, from the set of candidate indices $\bs{r}^{ref}$}
% 
\ENDFOR
% 
\RETURN $\bar{\bs{S}}(\bs{r}^d)$
% 
\end{algorithmic}
\label{alg:opt_ref}
\end{algorithm*}
% 
For hashing models LSH-RkNN and LSH-RMM described in the main paper, we can optimize the reference set, $\bs{S}^R$, for dialog modeling as described in the following.
 
For the selection of elements in $\bs{S}^R$, we use a greedy algorithm maximizing the proposed mutual information lower bound~(in \thmref{thm:mi_lb}); see the pseudo code in \algoref{alg:opt_ref}. We initialize a reference set of small size $I \ll M$, by randomly selecting responses from the training set of patient/therapist responses, i.e. $\bar{\bs{S}} = \{ S_1^p, \cdots, S_N^p, S_1^t, \cdots, S_N^t \}$; though, as noted before, the superset $\bar{\bs{S}}$ for the random selection can be any set of sentences/paragraphs, not necessarily coming from a dataset of patient/therapist responses. First, each element in the initial reference set is optimized greedily, and then more elements are added one by one until the reference set size grows to $M$. When optimizing each element in the set, for computing the MI lower bound, we sample $\gamma$ number of response pairs from the training set of patient/therapist responses pairs, $\{ (S_i^p, S_i^t) \}_{i=1}^N$. For computational efficiency, we adopt the idea of sampling for the candidate set as well, in each greedy optimization step, by sampling a subset of candidates of size $\beta$ from the set $\bar{\bs{S}}$.
	
% 	
The computation cost in the optimization is dominated by the number convolution kernel similarities, i.e. $O(\gamma(M^2+M\beta))$. In practice, we can keep low values of $\gamma$ as well as $\beta$; in our experiments, we use $\beta=1000, \gamma=100$, and vary the value of $M$ from $30$ upto $300$. A similar procedure can be used to optimize kernel parameters. 

	 	
{\bf Optimizing Neural Network Architecture. \\}
% 
% \input{algoNNPseudoCode.tex}
\begin{algorithm*}[tp!]
\caption{
% \small
\csizenine
Optimizing Neural Architecture in LSH-RLSTM for Dialog Modeling
% Neural-Hashing Model for Dialogue Modeling by Maximizing Our MI LB   - {\bf TODO Shorten the title}
}
% 
\csizenine
% 
\begin{algorithmic}[1]
\REQUIRE Training dataset $\{\bs{S}^p$, $\bs{S}^t\}$, with $N$ pairs; maximum number of layers in neural language models, $L$; the number of samples for computing the MI lower bound, $\gamma$; values for units in a layer, $\bs{u} =$ \{4, 8, 16, 32, 64, None\}. 
% \\
% \STATE $\bar{\bs{S}} = \{ S_1^p, \cdots, S_N^p, S_1^t, \cdots, S_N^t \}$
% \COMMENT{patient \& therapist responses in same set as the reference set}
% % 
% \\
% \STATE $\bs{S}^p = \{ S_1^p, \cdots, S_N^p \}$
% \COMMENT{patient responses}
% % 
% \\
% \STATE $\bs{S}^t = \{ S_1^t, \cdots, S_N^t \}$
% \COMMENT{therapist responses}
% 
% \STATE $\bs{r}^d$ $\gets$ randomSubset($2N$, $I$)
% \COMMENT{random subset of indices, of size $I$, from $\{ 1, \cdots, 2N \}$ for initialization of reference set}
% \\
% \STATE $NN \gets [10, None]$\COMMENT{initialization of neural network with 10 units in the first layer}
% 
% \STATE $NU \gets \{10, 20, 40, 80, None\}$\COMMENT{choices for number of units 
% in a layer
% }
\\
\COMMENT{optimizing up to $L$ layers greedily}
\FOR{$j=1 \to L$}
% 
% 
\STATE $\bs{r}^{lb}$ $\gets$ randomSubset($N$, $\gamma$)\COMMENT{subset of patient/therapist responses pairs for computing the MI LB to optimize $j_{th}$ layer}
% \\
% 
% 
\COMMENT{Number of units in $j_{th}$ layer, None not applicable for $1_{st}$ layer}
\FOR{$l \in \bs{u}$}
% 
\STATE $\bs{n}(j) \gets l$\COMMENT{$l$ units in $j_{th}$ layer of neural network}
% 
\STATE $\bs{C}^p \gets$ computeHashcodes($\bs{S}^p(\bs{r}^{lb}), \bs{n}$)
% 
\STATE $\bs{C}^t \gets$ computeHashcodes($\bs{S}^t(\bs{r}^{lb}), \bs{n}$)
% 
\STATE $\bs{mi}_{lb}(l)$ $\gets$ computeMILowerBound($\bs{C}^p, \bs{C}^t$)
% 
% \STATE $\bs{mi}_{lb}$ $\gets$ computeMILowerBound($\bs{K}^p, \bs{K}^t, \bar{\bs{K}}^p, \bar{\bs{K}}^t$)
% \COMMENT{compute the MI lower bound for all the candidates $\bar{\bs{S}}(\bs{r}^{ref})$, using the kernel matrices, via computation of hashcodes}
% 
\ENDFOR
% 
\STATE $\bs{n}(j)$ $\gets$ maxMILBIndex($\bs{mi}_{lb}$, $\bs{u}$)
\COMMENT{choose the units with maximum value of MI LB}
% 
\STATE \textbf{if} $\bs{n}(j)$ is None \textbf{then} break out of loop \textbf{end if}
% 
\ENDFOR
% 
\RETURN $\bs{n}$
% 
\end{algorithmic}
\label{alg:opt_nn_layers}
\end{algorithm*}

% 
For neural networks based LSH~(LSH-RLSTM), we can optimize the number of layers and the units in each layer, by maximizing the proposed MI LB; see pseudo code in \algoref{alg:opt_nn_layers}. 

\section{Experimental Details on LSH Models}
% 
LSTM models for each hash function in \emph{LSH-RLSTM}  are  trained using Adam~\cite{kingma2014adam}, with the learning rate $1e-3$, amsgrad=True, and $l_1$, $l_2$ regularization coefficients set to   $1e-4$.  We initialize a word in a response and its POS tag with a random  vector of size 30; for a single time step processing with in LSTM, word vectors of 10 adjacent words, along with their POS tags, are appended into a vector of size 600; this is required to avoid vanishing gradients since patient responses can be of length up to 8,000 words in the training dataset. For the $H$ number of LSTM models as neural-hash functions, same neural architecture, i.e., same number of layers and units, are used in each model. When optimizing the architecture of the LSTM models with \algoref{alg:opt_nn_layers} by maximizing our proposed MI LB~(\emph{MI LB Optimal}), we add layers one by one greedily up to maximum possible 5 layers~($L=4, \gamma=1000$), and try out different possible numbers of normal units in each layer, i.e., 4, 8, 16, 32, 64. (We keep the number of units small, since $\alpha$ is small. Also, during the optimization, we use $H=30$). When optimizing the Reference set with \algoref{alg:opt_ref}, we keep $\beta=1000, \gamma=100, I=20$.

{\em Similarity metric}. In case of \emph{kernel-hashing}, we use subsequence kernels~\cite{mooney2005subsequence} for computing similarity between two responses (subsequences of length up to 16 are matched), while similarity between a pair of words is computed as cosine between their word vector representations.

\subsection{Subsequence Kernel}
% 
Let $S_i$ and $S_j$ be two sequences of tokens~(words), the convolution kernel similarity between $S_i$ and $S_j$ is defined as below~\cite{mooney2005subsequence}.
            
\begin{align*}
\csizeten
K(S_i, S_j)
=
\sum_{e=1}^{16}
\sum_{\boldsymbol{i}, \boldsymbol{j}: |\boldsymbol{i}|=|\boldsymbol{j}|=e}
\prod_{k=1}^{|\boldsymbol{i}|}
k(S_i(\bs{i}_k), S_j(\bs{j}_k))
\lambda^{l(\boldsymbol{i})+l(\boldsymbol{j})}.
\end{align*}

Here, $k(S_i(\bs{i}_k), S_j(\bs{j}_k))$ is the similarity between the $k_{th}$ tokens in the subsequences $\boldsymbol{i}$ and $\boldsymbol{j}$, of equal length~(up to value 16); $l(.)$ is the actual length of a subsequence in the corresponding sequence, i.e., the difference between the end index and start index~(subsequences do not have to be contiguous); $\lambda \in (0, 1)$ is used to penalize the long subsequences. Dynamic programming is used for efficient computation of the subsequence kernel.
    
We use the following expression for computing the kernel similarity, $k(a,b)$, between two tokens $a$ and $b$ using their respective word vector representations~(real valued column vectors), $\bs{w}_a$ and $\bs{w}_b$.
            
\begin{align}
k(a, b)
=
cs
\left(
1-
\frac{(1-cs)}{(1-\zeta)}
\right)_{+};
\ \ \ 
cs = \frac{\bs{w}_a^T \bs{w}_b}{||\bs{w}_a||_2||\bs{w}_b||_2},
\end{align}

Herein, $cs$ is cosine similarity between the two word vectors, $\bs{w}_a$ and $\bs{w}_b$; $()_{+}$ represents the positive part function; $\zeta \in [-1,1]$ is a parameter for \emph{compact support} of the kernel function.

The parameters $\lambda, \zeta$ are optimized by maximizing the proposed MI LB criterion in our dialog model.

\section{Additional Experiment Details}

\begin{table*}[tp!]
\centering
\tabsize
\begin{tabular}{p{16.75cm}}
\toprule
% 
\patient{I did lose three pounds, did you notice that?}
\\
\therapist{That's great, I did notice that.}
\\
\rmm{Yes, you did.}
% {\bf RMM:} Yes, you did.
\\
\rknn{To help you with your diet?}
\\
\rlstm{Okay what's the explanation?}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of the way
\\
{\bf HRED:} Yeah. you
\\
{\bf VHRED:} Uh-huh. you
\\
% 
% 
% 
\toprule
% 
\patient{Well, first of all, we've never been able to, when I first come to see you in July you highly recommended and I refused to go into this day treatment or some type of a hospital and I refused and you put me on medicine. And the medicine helped a great, great deal. I have been to 4 different psychiatrists and they've put me on Lithium and they've done other things and none of that stuff worked. And when I come to see you I was real skeptic but I was reaching out for help.}
\\
\therapist{Um-hum.}
\\
\rmm{I see.}
\\
\rknn{It does?}
\\
\rlstm{You mean its puzzling why? I suppose it's very depressing too.}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of the way
\\
{\bf HRED:} Okay. you
\\
{\bf VHRED:} Uh-huh.
\\
% 
% 
% 
\toprule
% 
% 
\patient{Which is stupid because like, ya know, (sniffles) I guess if it's not what they like, then it's not what they like and they can like do something else, but like (sniffles) ya know there's some psychiatrists who charge like \$300 an hour. If you did that you would really have to work like...if you worked an hour a day five days a week that would be fifteen hundred dollars a week. Like...you wouldn't have to work at all...like barely. I mean, though, most psychiatrists probably don't charge \$300 an hour...yeah...it's just kinda ridiculous that...}
\\
\therapist{I'm sorry you're having such trouble getting...getting access to the care that you need (pause).}
\\
\rmm{You got to do.}
\\
\rknn{Oh yeah, you never tried Lithium?}
\\
\rlstm{And you ought not to just shove it away out of your life because you will need it again.}
\\
{\bf LSTM:} Uh-huh. you
\\
{\bf HRED:} Yeah. you
\\
{\bf VHRED:}  Uh-huh. you
\\
% 
% 
% 
\toprule
% 
% 
% 
% 
\patient{I don't... I guess that's the problem right now. I guess that's what I'm grappling with. I guess that's what I'm amazed about. I think, you know, the hypothesis that you just presented about what I'm doing probing, you know, fucking you over, you know, all of these things (PAUSE) it's plausible to me. And that's freaky because my experience of it is just, you know, just being pinned to the wall.}
\\
\therapist{Right. So... (PAUSE) Maybe the (PAUSE) sort of... (PAUSE) If I think about the sort of world that that one part is living in, the sort of fucking me over part, I imagine it's a world where that goes both ways, where you can be coming here for months and months and trying and not getting anywhere with this. And, you know, getting up and doing your part and paying money sort of or, you know, you know what I mean. And, you know, and still get nothing. Which is how you felt at some moments recently.}
\\
\rmm{Could be.}
\\
\rknn{Because nobody's helping you.}
\\
\rlstm{The thing, the thing I'm trying to get a feel for is what happened that was good? What happened?}
\\
{\bf LSTM:} Okay, you
\\
{\bf HRED:} M-hmm. you
\\
{\bf VHRED:} Okay, you
\\
% 
% 
% 
\toprule
% 
% 
% 
\patient{Yeah. I mean, it'll start, yknow, like right now, I mean, you're familiar with the weather patterns and things like that. It's not getting, I mean, the light is going to start to diminish, but the cold and having to be stuck in the house and everything all day isn't going to start for another month. Yknow, I'm still fine right now. Um, would you want me to call you then when I was going to start to take the 200 to let you know the beginning of it?}
\\
\therapist{Yeah, of course. Of course, you could do that.}
\\
\rmm{Yeah you probably could.}
\\
\rknn{So you get a little.}
\\
\rlstm{Right? And so just something to think about. It doesn't mean that it has to happen that way, but it can. And so the times where I may think that applies, I may bring it up. Because it's about relating your past relationships to your present relationships. And even how you relate in here with me. And so we may talk about that at some point.}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot
\\
{\bf HRED:} Yeah. you
\\
{\bf VHRED:} Okay. you
\\
% 
% 
% 
\toprule
% 
% 
% 
\patient{The fact that I wanted to do things that he didn't and then he felt guilty and I was like, \"Well, I mean it's not your fault because you're depressed and disappointed, too, and couldn't not be disappointed and stuff, too. Instead just focus on cuddling.}
\\
\therapist{That's not satisfying for you.}
\\
\rmm{Such as?}
\\
\rknn{Yeah.}
\\
\rlstm{One more thing, you just don't look at them enough.}
\\
{\bf LSTM:} Uh-huh. you
\\
{\bf HRED:} M-hmm. you
\\
{\bf VHRED:} Uh-huh. you
\\
% 
% 
\toprule
% 
% 
% 
% 
\patient{ Well I guess because there's truth to it when you go (ph), \"Okay, well what are you avoiding?\" in essence. I mean, there's truth to that. Because I ... because working in here, I agree, that's a thing I want to do is be focused on how I'm feeling. This whole thing with my family not being able to show feelings. By the way, I just have to drive over this scenic outlook and tell you that I, you know, I did talk to my mother about ...}
\\
\therapist{Now why are you doing that now?}
\\
\rmm{It's up to you.}
\\
\rknn{Yeah, people get really provocative.}
\\
\rlstm{How so?}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of the way
\\
{\bf HRED:} M-hmm. you
\\
{\bf VHRED:} Uh-huh. you
\\
% 
% 
\toprule
% 
% 
% 
% 
\patient{I hope so, I don't know what the heck that is, I don't' have any idea what that is, oh well, okay.}
\\
\therapist{Okay.}
\\
\rmm{And doing something that feels more like you.}
\\
\rknn{And you felt like that was - somehow you just couldn't do it I think.}
\\
\rlstm{You thought about that.}
\\
{\bf LSTM:} is a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of
\\
{\bf HRED:} Okay. you
\\
{\bf VHRED:} Okay, you
\\
% 
% 
\toprule
% 
\end{tabular}
\caption{
Textual responses generated by different systems for Depression Therapy dataset, along with ground truth patient and therapist responses.
}
\label{tab:gen_responses}
\end{table*}


\begin{table*}[tp!]
\centering
\csize
\begin{tabular}{p{16.75cm}}
\toprule
Yeah, here's hoping.\\
It's going to keep on being a struggle.\\
There isn't any, really anyone (ph) inside?\\
The Petition is the part that—\\
No, I don't. I really don't except that partly it's a fear of being further condemned by her. I mean, she condemns me for everything I am and everything I do.\\
So that there was again the concern with the - with [NAME].\\
Yeah. And so we didn't talk all the way home at all. And as we didn't talk, I think we were both growing angry. And so then we sat and we did talk for a long time. And that was good. Well, it was good. It was more...we talked more deeply about ourselves and our feelings than we were in the past without being angry at each other.\\
Yeah.\\
You've got your mother and sister.\\
Maybe if things are still horrible. I am hoping by next week they will be\\
When I told you that, did you remember what you felt?\\
And how to use that too.\\
You know people nearby pretty much though is you know? Also I think it's also he cannot ... he's been already like conditioned into, if he gets angry or has any ill feelings towards certain members of the family that's going to be it. Because he is no longer going be, you know ...\\
Well, that's what we're going to talk about.\\
From where?\\
I mean, you've been, I think it's great, you going every week to see [NAME OTHER], just about?\\
What's that, hon?\\
Yes.\\
Well yeah, like they didn't want their kids to be the real dummies in the neighborhood (laughter). But it's not - my father, it's not that he likes to brag on his kids if their not there. I mean he'd never say anything nice about us in front of us. But I guess it's the teachers that really bother me. I mean why get a kid an answer book. I can't - I mean, of course, I could have not cheated, but i And everything else I've done was very easy. My clarinet lessons; [I had beef cattle] (ph); I was in girl scouts. And, I mean, all I had to do was pick them out. I never had do any work. The boys always did the work, and then I went to the fair and got the purple ribbons.\\
Was it like defense-type stuff?\\
When you think of that moment in the car, how true do the words, "I can go on and thrive" feel on a 1-7 scale, with 1 being completely false and 7 being completely true?\\
I'm not seeing anybody right now.  I've got to, I've got to worry about me first.\\
I don't know. I thought of that all the time. Like how I've seen have big boxes of Kleenex usually expect the girls to cry.\\
It's easier with the groups you so about.\\
And same at your church I think.\\
Yeah.\\
Okay.\\
And with that sort of a person.  But because he is your biological father, there's a certain obligation and you are kind enough to do what has to be done.  That for you to have feelings wouldn't make much sense to me.  Of course, where, where are the feelings to come from?  The feelings would come from the acts of kindness and caring, compassion.  If they were not there, what should you feel?  But you are, nevertheless, kind enough to do the decent thing.  So, so that's one thing.  But how do you feel about that?  What I've just said?\\
I want a safe place out there.\\
No.  I had it during finals my first year of grad school and during my second year probably for like four months towards the end.\\
Yeah. I get that.\\
Okay, that's okay.\\
Once they send you the check -\\
It all seems so bad to you, it's a disillusion.\\
Yeah.\\
I said you don't want what I'm thinking on your tape.\\
So after I took one half at night, I was able to get up in the morning.\\
If I had asked you beforehand what they were going to do...?\\
You drink because you're lonely.\\
That's all right.\\
Yeah, in other words maybe I shouldn't have gotten so upset. Whereas it wasn't the most pleasant thing I should do. And like he was trying to say, you know, can't you just stay here tonight and leave tomorrow for college, see your girlfriend. And I've forgotten, it wasn't until like I just got the mail just before I came here and I was really, I didn't want to open it. It was just two Valentine's. It didn't say anything, you know, except love, Daddy and [NAME] and love, [NAME], but...\\
You went out\\
Um-hum.\\
Let's just pretend for a moment. Let's pretend that I'm your boss.\\
Okay. How old are you now?\\
Right. Well, a lot of it was like, before Christmas I was really, really snowed under with stuff and I had to work every day and I had to work late almost every day, and somehow even just the hour coming here was really a lot. Plus, I was really functioning on, 'let me just get through with work' because I had so many hours that I had to get through by Christmas or I couldn't go home for Christmas, and it was sort of, 'let me just get through that and think about things later'.\\
I was starting, you know, itching, it's almost for a month, a month and a half, I keep itching a lot over here in my face.\\
I feel like I've lost credentials and hope over...\\
Will you try out something again right now what you would find to be a response to Shelley given the fact of last week for example?\\
The rapport was good enough for that.\\

\toprule
\end{tabular}
% \vspace{-3mm}
\caption{
% \csize
We show first 50 responses~(in raw text format) that are selected greedily for the reference set~($\bs{S}^R$) in \emph{LSH-RkNN} model, out of 76,000 responses from the train set, with \algoref{alg:opt_ref}.}
\label{tab:reference_responses}
% \vspace{-1.5mm}
\end{table*}


% \input{dialogueGenerated.tex}

% \input{refSetRMM.tex}



==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/related.tex <==
% \vspace{-0.1in}
\section{Related Work}
\label{sec:rw}
% \vspace{-0.03in}
% 
Therapy chatbots, such as  Woebot \cite{fitzpatrick2017delivering}  and similar systems,  % based on   Cognitive Behavioral Therapy (CBT) \cite{lewinsohn1990cognitive}), 
are becoming increasingly popular; however, these agents have  limited ability to  understand free text and have to resort to a fixed set of preprogrammed responses to choose  from~\cite{di2017chatbots,ly2017fully,schroeder2018pocket,morris2018towards,hamamura2018standalone}. (Also, see \cite{jurafsky2014dialog} for an overview.)
    
For dialogue modeling in general domains, several recently proposed neural network based approaches are considered state-of-art ~\cite{serban2016generative,serban2017hierarchical,shao2017generating,asghar2017deep,wu2017sequential,li2017adversarial,zhao2018unsupervised,wu2018learning,xu2018diversity,park2018hierarchical,jiang2018sequence,tao2018get,xing2018hierarchical,chen2018hierarchical,shi2018toward,du2018variational}. However, those approaches usually require very large training datasets, unavailable in many practical applications; 
%often unavailable and may not perform well on relatively small datasets, such as transcribed therapy sessions (as we observe in this paper);
furthermore, they are not typically explored in  dialogue settings such as therapy including very long responses (up to tens of thousands of words).  Also, evaluating the effectiveness of the therapist's response  requires some  notion of relevance (e.g., mutual information) which goes beyond the standard measures of its semantic features~\cite{papineni2002bleu,liu2016not,li2017neural,lowe2017towards,li2017adversarial}.
%; we consider here an information-theoretic approach to capture this notion.

Unlike  task-driven dialogue~\cite{zhai2014discovering,wen2016network,althoff2016large,lewis2017deal,he2018decoupling},   an immediate response quality metric may not   be available in our settings, since the effect of therapy is harder to evaluate and multiple sessions are often required to achieve the desired outcome.
%; thus, some intermediate criteria  must be introduced. 
Attention to specific parts of the response, as well as background knowledge, explored in neural network based dialogue modeling~\cite{kosovandialogue} can be helpful in therapeutic dialogues; those aspects  are, to some extent, implicitly captured by learning the hashing models. 
% 
% Note that in related work by \cite{bartl2017retrieval}, hashcodes are only used for the nearest neighbor search, instead of serving as response representation as proposed here. 
% 
%representations of the responses, and are  only used for the nearest neighbor search,  unlike the approach proposed here.  
    
In \cite{he2018decoupling}, an approach is presented to a task-driven (e.g., negotiation) dialogue which consists in  mapping a response to an ordered list of rules, where each rule represents a task-specific intent; this does not apply to our more open-ended dialogues without the specific tasks.
    
While mutual information has been previously considered in dialogue modeling during testing \cite{li2016diversity}, it was not used as a model selection criterion for  learning representations.
% 
% Moreover, popular  BLEU score~\cite{papineni2002bleu} does not  measure relevance between the responses,  but rather tries to capture all  information  when comparing the ground truth with the produced text.
    
Finally,  there are multiple approaches for  estimating mutual information   from data
%, there are many  approaches based on k-Nearest Neighbors, Random Forest, ensemble models, etc~
\cite{kraskov2004estimating,koeman2014mutual,singh2014generalized,gao2015efficient}. However, these estimators are highly expensive  in high-dimensional settings, and can be quite inaccurate when the number of samples is  small. There is a recent approach of neural estimation of mutual information on two high dimensional continuous variables, though not applicable to discrete variables like hashcodes~\cite{belghazi2018mine}. For discrete variables, theoretical analysis has been limited to one dimensional case~\cite{jiao2017maximum}. Previously, several mutual information lower bounds have been proposed for classification problems~\cite{chalk2016relevant,gao2016variational,alemi2017deep}, assuming one-dimensional class label; unfortunately, they do not apply in our setting where the predicted response is a high-dimensional  vector. 

\shrink{ %%% temporary commented out to check the space  %%
\todo{for Sahil, add references suggested by AISTATS reviewers}

\todo{For Sahil, mention recent estimators for mutual information, such as MINE, which are relevant for continous variables whereas we have binary~(hashcode) representations in this work.}
\todo{For Sahil, add recent citaions from 2018, replacing older ones.}
} %%%
% recent bounds
% mcallester2018information
% oord2018representation


% Unsupervised Discrete Sentence Representation Learning for Interpretable Neural Dialog Generation
% 
% A retrieval-based dialogue system utilizing utterance and context embeddings
% 
% An Ensemble of Retrieval-Based and Generation-Based Human-Computer Conversation Systems
% 
% Learning Matching Models with Weak Supervision for Response Selection in Retrieval-based Chatbots
% 
% Insufficient Data Can Also Rock! Learning to Converse Using Smaller Data with Augmentation
% 
% Response Generation by Context-Aware Prototype Editing
% 
% Skeleton-to-Response- Dialogue Generation Guided by Retrieval Memory
% 
% Towards Building Large Scale Multimodal Domain-Aware Conversation Systems
% 
% Two are Better than One- An Ensemble of Retrieval- and Generation-Based Dialog Systems
% 
% Why are Sequence-to-Sequence Models So Dull
% 
% 
% 

==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/secLearnHashDialog.tex <==
% \section{Kernelized Hashcodes based Dialog Modeling}
% % 
% \todo{motivate, saying first kernel based model. suitable for psychiatry related problems where nonparameteric models allow interpretability, less chances for overfitting.}

% \vspace{-0.1in}
\subsection{Learning Kernelized Hashcode Representations for Dialog Modeling}
% \vspace{-0.05in}
\label{sec:oa}

Given that each specific hashing model described above  involves several model-selection choices, our task  will be to optimize those choices using the  information-theoretic criterion proposed below.

\subsubsection{Optimizing LSH Model Parameters\\}
% 
As per the discussion of LSH above, an LSH model involves the function $\bs{lsh}(.; \bs{\theta}, \bs{S}^R)$ for mapping text responses to hashcodes: % 
$
\bs{c}_i = 
\bs{lsh}(S_i; \bs{\theta}, \bs{S}^R)$, where 
$\bs{c}_i = \bs{h}(S_i) = (h_l(S_i))_{l=1}^H,$
% 
and where each hash function $h_l(.)$ is built based on a random subset of $\bs{S}^R$ using either a kernel (kNN, SVM) or a neural network (LSTM) classifier. For the case of kernel-based LSH,  $\bs{\theta}$ are the parameters of a convolution kernel similarity function $K(S_i, S_j)$. For neural hashing (LSH-RLSTM), $\bs{\theta}$ refers to the  neural architecture hyperparameters (number of layers, the number of units in a layer, type of units, etc.); $\bs{\theta}$ also includes LSH-specific parameters such as  $\alpha$. 

When learning LSH models on a training datset, the (hyper) parameters   $\bs{\theta}$ as well as the reference set $\bs{S}^R$  will be optimized with respect to the information-theoretic objective introduced below.
Namely, for LSH-RkNN and LSH-RMM, the kernel parameters $\bs{\theta}$ are optimized via grid search. For LSH-RLSTM, $\bs{\theta}$ reflects the neural architecture, i.e. the number of layers and the number of units in each  layer, optimized by greedy search. Similarly, $\bs{S}^R$ is also constructed via a greedy algorithm. 
% 
% Pseudo codes for the greedy algorithms are presented in the supplementary material.
% 
% ~\footnote{Since parameters under optimization are \emph{shared} between all the hash functions jointly, this allows keeping individual hash functions randomized~(built from small random subsets of $\bs{S}^R$), which should possibly help in learning hashcode-based representations that are more robust to over-fitting a dialog training dataset. Further, although it is theoretically difficult to establish, this inherent randomization of hash functions, despite the learning of the shared parameters, should help towards keeping hashcodes locality-sensitive~(an important property for hashcodes to be good feature representations).}

\input{algo_ngrams_text_gen.tex}

\subsubsection{Information-Theoretic Objective Function\\}
% 
The objective function for hashcode-based model selection in dialog generation should (1) characterize the quality of hashcodes as generalized/compressed representations of dialogue responses and  (2) favor  representation models leading to higher-accuracy response generation.
    
Mutual information $\cI(S^p : S^t)$ between the dialog responses $S^p$ (e.g, patient) and $S^t$ (e.g., therapist) is a natural candidate objective as it implies   higher predictability of one response from another. Though,  it   is hard to compute in practice as the joint distribution over all pairs of textual responses is not available. However, we can attempt to approximate it using hashcode representations. If $\bs{h}(.)$ represents a function from the space of all statements to the hashing code space, then the {\em data processing inequality} implies that $\forall \bs{h}(.), \cI(S^p : S^t) \geq \cI(\bs{h}(S^p) : \bs{h}(S^t))$, and   maximizing the quantity on the right can be more computationally feasible.
    
Thus we  will maximize the \emph{mutual information (MI)} between the response hashcodes, over LSH model parameters; it turns out that MI  reflects   both the inference accuracy as well as the representation quality, as we will see below:

% \vspace{-0.1in}
\begin{align}
&
\mathop{\arg\max}_{\bs{\theta}, \bs{S}^R}\ \ 
\cI(\bs{C^p}:\bs{\cC^t});
\\
&
\bs{C^p}=\bs{lsh}(S^p; \bs{\theta}, \bs{S}^R),\ 
\bs{C^t}=\bs{lsh}(S^t; \bs{\theta}, \bs{S}^R)
\\
&
\cI(\bs{C^p}\!:\bs{C^t}) 
=
\cH(\bs{C^t})
- 
\cH(\bs{C^t}|\bs{C^p})
\label{eqn:dialogues_mi}
\end{align}
	
\noindent Herein, $\bs{C^p}$ and $\bs{C^t}$ are the multivariate binary random variables associated with the hashcodes of patient and therapist   responses, respectively. Minimizing the conditional entropy, $\cH(\bs{C}^t|\bs{C}^p)$,   improves the predictive accuracy when inferring  therapist response hashcode, while maximizing the entropy term, $\cH(\bs{\cC}^t)$, should ensure good quality of the hashcodes as generalized representations of text responses; thus MI objective satisfies both criteria stated at the beginning of this section.
% ~\footnote{If we were learning LSH parameters by minimizing the conditional entropy term~($\cH(\bs{C}^t|\bs{C}^p)$) only, entropy of the hashcodes~($\cH(\bs{C}^t)$) could also reduce since the latter reduction would lead to a decrease in the intrinsic dimension of the hashcodes inference problem itself, thus making the inference more accurate, corresponding to low conditional entropy. This kind of decrease in the conditional entropy would not be desirable as the problem of inferring hashcodes itself would be somewhat artificial.}

\input{word_embedding_eval.tex}

\subsubsection{Mutual Information Lower Bound for Efficiency\\}
\label{sec:mi_lb}
% 
Since computing mutual information between two high-dimensional variables can be both computationally expensive and  inaccurate if the number of samples is small~\cite{kraskov2004estimating,walters2009estimation,singh2014generalized,gao2015efficient}, we develop a (novel) lower bound on the mutual information which is easy to compute.
For derivation details,  see the supplementary material.
% \footnote{Supplementary material: https://tinyurl.com/y6gefz8k.}.

We will first introduce the information-theoretic quantity called \emph{Total Correlation}~\cite{watanabe1960information},  $\cT\cC(\bs{C}) = \sum\limits_j \cH(C_j) - \cH(\bs{C})$, which captures non-linear correlation among the dimensions of a random variable $\bs{C}$; given an additional  random variable $\bs{Y}$, $\cT\cC(\bs{C}: \bs{Y})$ is defined as:
 
\begin{align}
\cT\cC(\bs{C}: \bs{Y}) = \cT\cC(\bs{C}) - \cT\cC(\bs{C}|\bs{Y}).
\end{align}


\begin{theorem}[Lower Bound on Mutual Information]
Mutual information between two random hashcode variables, $\cI(\bs{C^p}: \bs{C^t})$, can be bounded from  below as follows:
% \\
% $\cI(\bs{C^t}: \bs{C^p})
% \ge$

{
\csizenine
% 
\begin{align*}
\cI(\bs{C^p}: \bs{C^t})
\ge
&
\sum\limits_j{\cH(C^t_j)}
-
\cT\cC(\bs{C^t}:\bs{Y^*})
%\nonumber \\
%&
+
% \sum\limits_j{\left\langle \log q(C^t_j|\bs{C^p})
% \right\rangle_{p(C^t_j, \bs{C^p})}}.
\sum\limits_j{\left\langle \log q(C^t_j|\bs{C^p})
\right\rangle}.
% 
\end{align*}
% % 
% \vspace{-0.1in}
% \begin{align*}
% \bs{Y^*}
% \gets
% \mathop{\arg\max}
% \limits_{\bs{Y}:|\bs{Y}|=|\bs{C^p}|} \cT\cC(\bs{C^t}:\bs{Y})
% \label{eqn:corex_opt_thm}
% \end{align*}
}
% 
Herein, $\cT\cC(\bs{C^t}:\bs{Y})$ describes Total Correlations within $\bs{C^t}$ that can be explained by a latent variables representation $\bs{Y}$; $q(C^t_j|\bs{C^p})$ is a proposal conditional distribution for the $j_{th}$ bit of the hashcode $\bs{C^t}$ predicted using a probabilistic classifier, like a Random Forest model.
\label{thm:mi_lb}
% \vspace{-3mm}
\end{theorem}

As discussed in \cite{greg2014discovering}, $\cT\cC(\bs{C^t}: \bs{Y}^*)$ can be computed  efficiently.
% ~\footnote{Also note that, for computational efficiency as well as to avoid overfitting a dialog training dataset, we use small random subsets of size $\gamma$~($\gamma=1000$ in experiments) from a training set for stochastic empirical estimates of the mutual information lower bound. Further, for practical purposes, the dimensionality  of latent representation $\bs{Y}$ can be   much smaller than the dimension of hashcodes.}
    
Note that the first two terms in the MI lower bound contribute to improving the quality of hashcodes as response representations,  maximizing entropy of each hashcode bit while discouraging redundancies between the bits, while the last term containing conditional entropies aims at improving inference of individual hashcode bits.

    
Moreover, one can use the proposed MI LB as an \emph{evaluation metric of the dialog quality on test data}, i.e. the alignment/relevance between the responses of two dialog agents.

\input{human_eval.tex}

Also, note that mutual information criterion has been used previously to optimize kernelized hashcode representations for binary classification problems~\cite{garg2018efficient,garg2019nearly}. The approximation of mutual information proposed in those prior works are not applicable for dialog modeling.

% , motivating the need for developing the novel lower bound for mutual information, as introduced above. 
% See the related works in \secref{sec:rw} discussing neural dialog models using similar information-theoretic objectives, as well as other approaches for approximate estimation of mutual information.
                    
We also use a normalized metric, dividing MI LB by an upper bound on joint entropy,

\begin{align}
\cH(\bs{C^t})
&=
\sum\limits_j{\cH(C^t_j)}
-
\cT\cC(\bs{C^t})
\\
&
\leq
\sum\limits_j{\cH(C^t_j)}
-
\cT\cC(\bs{C^t}:\bs{Y^*}).
\end{align}

For $\cT\cC(\bs{C^t}|\bs{Y^*})=0$, i.e. when a latent representation $\bs{Y^*}$ is learned which explains all the Total Correlations in $\bs{C_t}$, the upper bound becomes equal to the entropy term; practically, for the case of hashcodes, learning such a representation should not be difficult, so the bound should be tight. 

% \subsection{Inference of Therapist Responses}
% 
% \paragraph{Inferring Therapist Hashcodes as Multi-Class Labels}


Having learned a model to hash patient or therapist utterances, we train a Random Forest classifier, or any classifier, to infer hashcode for a therapist response given the input of a hashcode of a patient  utterance, as illustrated in \figref{fig:klsh_max_mi}. For mapping the inferred therapist hashcode to a textual response, we have two choices. One simple choice, which works well for therapeutic dialog like problems, is to select a therapist response from the training set by matching its hashcode w.r.t. the inferred hashcode. Second choice is to generate a new response given the inferred hashcode, for which we propose a novel approach in the following section.
	
\subsection{Dialogue Generation with Kernelized Hashing of N-grams}
% 
\label{sec:gen_response}
% 

For generation of a therapist dialogue response, given the input of its kernelized hashcode representation, we propose a new language model by generalizing the traditional approach of N-grams language modeling with kernelized hashing of N-grams.
%
%The basic principle behind the traditional N-gram models was to generate N-grams from text sentences in a training set, and then one could compute probability of any N-gram based on its occurrence across all the sentences in the training corpus. Further, one can use N-grams probabilities statistics to correspondingly compute conditional probabilities for seeing a token, thus generating a new token conditioning upon the sequence of tokens generated previously. 
%
The fundamental problem with the traditional N-grams based language models is that the approach is restricted to N-grams of short length~\cite{pauls2011faster,bengio2003neural,brown1992class}. As we increase the length of N-grams, it becomes difficult to generalize the applicability of N-grams from a training corpus to test settings due an explosion in the number of possible N-grams.
%Therefore, despite the vast literature on N-grams language modeling, a nonparametric approach, it had become less popular for problems where there is need for capturing long range dependencies in text.
    
In light of the recent developments on learning kernelized hashcode representations of natural language~\cite{garg2018efficient,garg2019nearly}, it is possible to generalize the existing N-gram language models via kernelized hashing of N-grams. While it is low probable to exactly match an N-gram of large length w.r.t. the ones in a training corpus, it is feasible to find a match for its hashcode representation. This is because N-grams sharing relevant patterns are assigned same kernelized hashcode. Along these lines, instead of N-grams, probabilities are computed for hashcodes of N-grams per the occurrence statistics of N-grams assigned same hashcode, and so it applies for the conditional probabilities, which gives us the basic language model for generating therapist responses; see the pseudo code in \algoref{alg:response_generation}.

For hashing of N-grams, we use an unsupervised kernelized hashing model; the supervised dialog hashing model, that we proposed in the previous section, is used only for hashing of dialogue utterances, not N-grams. In \cite{garg2019nearly}, an information theoretic approach for nearly-unsupervised learning of kernelized representations is proposed for  information extraction task, that is easily extensible for unsupervised learning settings.


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/tabHashDialogModelsCompare.tex <==
\begin{table*}[tp!]
\centering
% \tabsize
% \renewcommand{\tabcolsep}{3.6pt}
% 
\subtable[
Depression Therapy Dataset
]
{
\centering
\begin{tabular}{llllllllllll}
\toprule	
% 
\textbf{Model}
& MI LB~(Shuffled)
% & Entropy UB
& NMI LB
% ~(Shuffled)
&HIA~(Baseline)
\\
% 
\toprule
% &
% Our Kernel-
LSH-RkNN
% ~(M=300)
% &16.4$\pm$0.3~(8.2$\pm$0.2)
% % &26.2$\pm$0.1
% &0.63~(0.31)
% &{\bf 0.84$\pm$0.16~(0.79$\pm$0.18)}
% \\
% 
&$12.8\pm$0.5~(6.1$\pm$0.2)
% &22.6$\pm$0.4
&0.57~(0.27)
&0.87$\pm$0.16~(0.82$\pm$0.18)
\\
% 
% 
% LSH-RkNN
% (POS)
% % ~(M=300)
% &25.2$\pm$0.3~(13.3$\pm$0.4)
% % &26.2$\pm$0.1
% &0.67~(0.35)
% % &0.84$\pm$0.16~(0.79$\pm$0.18)
% \\
% 
% 
% \midrule
% % &
% % Our Kernel-
% RkNN~(PoS)
% % ~(M=300)
% &24.1$\pm$0.3~(12.6$\pm$0.4)
% % &35.8$\pm$0.3
% &0.67~(0.35)
% &0.79$\pm$0.14~(0.72$\pm$0.16)
% \\
% 
% 
\midrule
% &
% Our Kernel-
LSH-RMM
% ~(M=300)
% &6.0$\pm$0.4~(-4.2$\pm$0.4)
% % &30.5 $\pm$ 0.4
% &0.2~(-0.14)
% &0.76$\pm$0.06~(0.65$\pm$0.05)
% \\
% 
%
&{\bf13.7$\pm$0.2~(-1.0$\pm$0.3)}
% &34.8 $\pm$ 0.3
&{\bf0.39~(0.0)}
&{\bf0.68$\pm$0.10~(0.59$\pm$0.10)}
\\
% 
% 
% % 
% \midrule
% % &
% % Our Kernel-
% RMM~(PoS)
% % ~(M=300)
% &$\pm$
% &$\pm$
% &$\pm$
% \\
% 
% 
% 
% \midrule
% Our Kernel-RMM~(M=1000)
% &
% &
% &
% \\
% 
\midrule
% &
% Our Neural-
LSH-RLSTM
&20.3$\pm$0.3~(10.6$\pm$0.2)
% &26.8$\pm$0.3
&0.76~(0.40)
&0.82$\pm$0.19~(0.79$\pm$0.21)
\\
% 
\toprule
\end{tabular}
}
% 
% 
\subtable[
Twitter Dataset
]
{
\centering
\begin{tabular}{llllllllllll}
\toprule	
% \textbf{Datasets}
% 
% &
% 
% 
\textbf{Model}
&
MI LB~(Shuffled)
% & Entropy UB
& NMI LB
% ~(Shuffled)
&HIA~(Baseline)
\\
% 
% 
\toprule
% Our Kernel-
LSH-RkNN&
% % % ~(M=100)
% 16.0$\pm$0.1~(9.2$\pm$0.1)
% % &23.4$\pm$0.1
% &0.68~(0.39)
% &0.87$\pm$0.15~(0.83$\pm$0.18)
% \\
% 
% % % ~(M=300)
17.3$\pm$0.1~(9.1$\pm$0.1)
% &23.0$\pm$0.1
&0.75~(0.40)
&0.85$\pm$0.18~(0.81$\pm$0.21)
\\
% 
% \midrule
% \\
% 
\midrule
% Our Kernel-
LSH-RMM&
% % % ~(M=300)
{23.4$\pm$0.2~(11.2$\pm$0.3)}
% &33.0$\pm$0.2
&{\bf0.71~(0.34)}
&{\bf0.80$\pm$0.14~(0.72$\pm$0.16)}
\\
% 
% \midrule
% \\
% 
\midrule
% Our Neural-
LSH-RLSTM&
{\bf 41.9$\pm$0.1~(24.3$\pm$0.1)}
% &50.3$\pm$0.1
&0.83~(0.48)
&0.69$\pm$0.16~(0.63$\pm$0.16)
\\
% 
% 
\toprule
\end{tabular}
}
% 
% 
% 
% 
\subtable[
Larry King Dataset
]
{
\centering
\begin{tabular}{llllllllllll}
\toprule	
% \textbf{Datasets}
% 
% &
\textbf{Model}
& 
MI LB~(Shuffled)
% & Entropy UB
& NMI LB
% ~(Shuffled)
& HIA~(Baseline)
\\
% 
% 
\toprule
% Our Kernel-
LSH-RkNN&
% % % ~(M=100)
% &
9.4$\pm$0.3~(5.1$\pm$0.3)
% &15.0$\pm$0.3
&0.63~(0.34)
&0.91$\pm$0.14~(0.89$\pm$0.16)
\\
% 
% 
% \midrule
% \\
% 
\midrule
% Our Kernel-
LSH-RMM&
% % % ~(M=300)
% &
% 8.1$\pm$0.2~(4.4$\pm$0.2)
% % &14.2$\pm$0.3
% &0.57~(0.31)
% &0.92$\pm$0.13~(0.90$\pm$0.16)
% \\
%
% 
22.4$\pm$0.9~(4.5$\pm$1.2)
% &35.9$\pm$0.8
&{\bf0.62~(0.13)}
&{\bf0.69$\pm$0.11~(0.59$\pm$0.10)}
\\
% 
% 
% \midrule
% \\
% 
\midrule
% Our Neural-
LSH-RLSTM
% &
&{\bf 48.9$\pm$0.3~(28.4$\pm$0.5)}
% &60.9$\pm$0.1
&0.80~(0.47)
&0.62$\pm$0.10~(0.54$\pm$0.07)
\\
% 
% 
\toprule
\end{tabular}
}
% 
% \vspace{-3.75mm}
% 
\caption{
% \csizenine
Hashcode models quality as measured by the alignment between the hashcodes of person A and person B responses  (mutual information lower bound and its normalized version), as well as by the predictability of B's responses given A's response. 
% 
% 
% \todo{mention that the values in the brackets are computed for randomly paired responses across different sessions.}
% 
% 
% HIA refers to Hashcodes Inference Accuracy; DR refers to some metric we need to reflect the diversity of text responses. 
% PoS denotes Part of Speech Tags.
}
\label{tab:results2}
% \vspace{-1.25mm}
\end{table*}


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/tab_generative_hash_comparison.tex <==
\begin{table*}[tp!]
\centering
% \csize
% \renewcommand{\tabcolsep}{2.0pt}
\centering
\begin{tabular}{llllllllllll}
\toprule	
% 
&LSTM&HRED&VHRED&LSH-RkNN&\textbf{LSH-RkNN-Gen}\\
% 
\toprule
%
% % first choice
% &8&39&45&113&95\\
% % second choice
% &14&34&36&108&108\\
% total votes
% &22&73&81&221&203\\
% 
Appropriate~(\%)&3.7&12.2&13.5&36.8&33.8\\
% 
\midrule
% 
% &0&2&2&6&40\\
% 
Diverse~(\%)&0.0&4.0&4.0&80&12.0\\
% 
\toprule
\end{tabular}
% 
% \vspace{-2.5mm}
\caption{
% \csizenine
Human evaluation scores on Depression dataset~(300 test samples) for our generative hashing model~(LSH-RkNN-Gen) w.r.t. the baseline models, and our response selection based hashing model~(LSH-RkNN).}
\label{tab:human_gen}
% \vspace{-3.25mm}
\end{table*}



==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/tab_response_hashcodes.tex <==
\begin{table}
\centering
\tabsize
% \fontsize{8}{8}\selectfont
% \renewcommand{\arraystretch}{0.9}% Tighter
% \scriptsize
\begin{tabular}{p{7.75cm}}
\toprule
% % CLIENT: 
% But for the next person I mean. I deal with - that's part of what I do is I train people. I'm always - I'm either training people on this computer or what I like to do more is training people how to understand and train.
% And so I have - I feel bad when I give up on a trainer, you know. I just don't think she has it. It's - and I have met people who have had tremendous, tremendous abilities of being able to like grasp concepts and communicate them to others who I had more belief in, you know. [00:16:13]
% Does that make - I guess that...
% ((Crosstalk))\\
% 0101001111001011111110101101111111011011100011101100111000101011110111001001011011001110001010100100
% \\
% \\
% \thp{
% % THERAPIST: 
% For now it's just you don't - can't see like A, (inaudible at 00:16:25) a look at yourself and B, can't see her dealing well with anybody else.}\\
% \thp{
% 0101001111011011111100101101111110011011100001000100111100101000110111001001011111001110001000001000
% }
% \\
% \midrule
% % CLIENT: 
% My dad actually seems in, um, better shape health-wise than he has in a while. I was worried about him the last time I was down there, but the one thing I told him, I said, you know - we were - they had already been in town a few hours. I said, "You know, you haven't told me one story that you've already told me before." I said, "I don't know if you've changed your diet or something, but you're not as senile as you used to be." (Laughing.) [00:03:27]\\
% 0101001111001011111100101101111110011011100011000100111100101001110111001101011111011110001000000000
% \\
% \\
% \thp{
% % THERAPIST: 
% (Laughing.)
% }
% \\
% \thp{
% 0101100110111011111110111100110110101111111011110110111000101101100011101010011011001110101000100000
% }
% \\
% \midrule
% PT:	
% I'll stay on the Restoril, I mean it takes me a while to go to sleep but I'll stay on the Restoril.
% \\
% 0101001111101111111110101101011110011010100011100101111000101011110111001001011011001110001010000110
% \\
% \\
% \thp{
% % DR:	
% Let's nudge the Pamelor up a little bit.  We could also check a blood level.
% }
% \\
% \thp{
% 0111001111001011111100101100111110011010110001001100111100101101010111001011011011111110001100000000
% }

% \thp{
% 010101011010111111111010110101111001101110000110010011100010101
% % 1110111001001011011001110001010100010
% }
% \\
%\midrule
% PATIENT: 
\textit{
Its all my fault. It's like getting hit in the stomach And trying to catch your breath. You can't catch it. You struggle, move around, You just can't get your breath. That just really knocks me off balance. 
You begin to generate this feeling of a kind of negativism. And that's why it really being hurt. I never allowed myself to think negative, accept everybody else. I am the only one giving back to the "be quiet time." I had to have something to make do with that.
}
\\
010100111100101111111010110101111001101110001110110011100010100
% 1110111101011011011001110001000000000
\\
\\
\thp{
% COUNSELOR: 
\textit{
OK. Maybe that fits into the whole pattern then.
}
}\\
\thp{
01110011010010111111000111111111100010101100110011
% 00
% 11100010110
% 0010111101010011011011110001100001000
}
\\
%\midrule
% CLIENT: 
% \textit{
% Well I talked to a friend of mine whom I think is promiscuous and she told me about a man that came to see her at her apartment. So I gave him my phone number. I don't have any hang up about morals. I don't know. I told a couple of my friends about this. I must admit I'm a little shy talking about it now.
% % [0:23:27.1]
% }
% \\
% 010100011010101111111010110101111001101110000110010011100010100
% % 1110111001011011011001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% I see. You mean it's embarrassing to tell me about it.
% }
% }
% \\
% \\
% \midrule
% % PT: 
% \textit{
% Yeah.  I didn't think she was going to die.
% }
% \\
% 01010001101010111111101011000111100100111000111001
% 00111000101011110111101001011011001110001000100010\\
% \\
% \thp{
% % DR: 
% \textit{
% Yeah.
% }
% }\\
% \thp{
% 01011001101110011111101011000111111010111110011001
% 10111100101111010111101010011010101110101010100010
% }
% \\
% 
% \midrule
% CLIENT: So I filed a bug report on Wednesday.\\
% \\
% THERAPIST: Yeah.\\
% 
% \midrule
% % PATIENT: 
% \textit{
% I'm sitting here just thinking about things. Should I think out loud? (chuckles)
% }
% \\
% 01010001111010111111001111011111110010111000011001
% 00111000101011110111001101011001001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% Sure. If you want to.
% }
% }
% \\
% \thp{
% 11010011001110111111001011011101110100111000111011
% 00111100101001110111101100011001001110001010000000}
% \\
% \midrule
% % CLIENT: 
% \textit{
% Because it's almost a year of my life.
% }
% \\
% 01010011110010111111001011010111101100101100110011
% 00111100101101110111101011011011011110001000100000\\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% All this is. It's a good chunk of time.
% }
% }\\
% \thp{
% 01010011010010111111001011010111101010101000110011
% 00111100101101110111101011011011001110001000100000
% }\\
% 
% \midrule
% % PATIENT: 
% \textit{
% Most of it is small bills. There's one 50 dollar check, and that's the only thing that's really large. The rest of it's like ten or twelve dollars each.
% }\\
% 0101001101001011111100101101111110011011110011001100111100101100110111101011011011011110001000101000\\
% \\
% \thp{
% % THERAPIST: 
% \textit{
% But it adds up.
% }
% }
% \\
% \thp{
% 0101011111101011111110111101011110001011100001100100111000101001110111101111011011001110001010100010
% }
% \\
\toprule
\end{tabular}
\vspace{-2.75mm}
\caption{
\csizenine
In this table, we show a pair of patient and therapist~(Blue) responses.
% , randomly sampled from different sessions.
% ; the responses of therapists are in red. 
For each response, we obtain a locality sensitive hashcode as its representation.
% , of 100 bits each. 
The hashcode of a patient response is used as feature representation to infer the hashcode of the corresponding therapist response.
% as multi-class labels.
}
\label{tab:therapy_session_hashcoded}
\vspace{-6mm}
\end{table}% 


==> Therapeutic Dialog Modeling via Hash Functions - AAAI20/word_embedding_eval.tex <==
\begin{table*}[tp!]
\centering
% \csize
% 
% \renewcommand{\tabcolsep}{10.75pt}
% 
\subtable[Depression Therapy Dataset]
{
\centering
\renewcommand{\arraystretch}{1.4}% Tighter
\renewcommand{\tabcolsep}{12.75pt}
\begin{tabular}{llllllllllll}
\toprule	
% \textbf{Datasets}
% 
% &
\textbf{Model}
& Average
& Greedy
& Extrema
% & DR
\\
% 
\toprule
%
% Depression Therapy Sessions&\\
% 
% 
% \midrule
% &
LSTM~\protect\cite{vinyals2015neural}
& 0.61$\pm$0.31
&\bf{0.58$\pm$0.29}
&0.28$\pm$0.16
\\
% 
\midrule
% &
HRED\protect\cite{serban2016building}
&0.48$\pm$0.23
&0.43$\pm$0.20
&0.29$\pm$0.16
\\
% 
\midrule
% &
VHRED\protect\cite{serban2017hierarchical}
&0.48$\pm$0.23
&0.43$\pm$0.20
&0.29$\pm$0.16
\\
% 
% 
% 
\toprule
% &
% Our Kernel-
LSH-RkNN
% 
% ~(M=300)
% &0.55$\pm$0.39
% &0.47$\pm$0.29
% &0.26$\pm$0.21
% % \\
%
% generative 100 bits RkNN
% 
&0.60$\pm$0.37
&\bf{0.58$\pm$0.34}
&\bf{0.37$\pm$0.24}
% % \\
%
% 
% 
% alpha=10
% &0.57$\pm$0.37
% &0.48$\pm$0.28
% &0.28$\pm$0.20
% \\
% 
% 
% % 
% \midrule
% % &
% % Our Kernel-
% \textbf{LSH-RkNN}
% % ~(PoS)
% % ~(M=300)
% % 
% &0.61$\pm$0.33
% &0.49$\pm$0.26
% &0.88$\pm$0.08
% 
% &0.62$\pm$0.34
% &0.52$\pm$0.28
% &0.88$\pm$0.07
% 
\\
% 
% 
\midrule
% &
% Our Kernel-
LSH-RMM
% ~(M=300)
% &{\bf 0.69$\pm$0.34}
% &{\bf 0.70$\pm$0.34}
% &{\bf 0.42$\pm$0.23}
% \\
%
&0.56$\pm$0.38
&0.53$\pm$0.33
&0.31$\pm$0.23
\\
% 
% 
% % 
% \midrule
% % &
% % Our Kernel-
% RMM~(PoS)
% % ~(M=300)
% &$\pm$
% &$\pm$
% &$\pm$
% \\
% 
% 
% 
% \midrule
% Our Kernel-RMM~(M=1000)
% &
% &
% &
% \\
% 
\midrule
% &
% Our Neural-
LSH-RLSTM
&\bf{0.64$\pm$0.37}
&0.51$\pm$0.28
&0.28$\pm$0.19
\\
% 
% 
\toprule
\end{tabular}
}
%
% \newline
% 
\subtable[
Twitter Dataset
]
{
\centering
\renewcommand{\arraystretch}{1.4}% Tighter
\renewcommand{\tabcolsep}{12.75pt}
\begin{tabular}{llllllllllll}
\toprule	
% \textbf{Datasets}
% 
% &
\textbf{Model}
& 
Average
& Greedy
& Extrema
% & DR
\\
% 
\toprule
%
% 
LSTM~\protect\cite{vinyals2015neural}
&
0.51
&0.39
&0.37
\\
% 
\midrule
HRED~\protect\cite{serban2016building}
&
0.50
&0.38
&0.36
\\
% 
\midrule
VHRED~\protect\cite{serban2017hierarchical}
&
0.53
&0.40
&\bf{0.38}
\\ 
% 
% 
\toprule
% Our Kernel-RkNN
% % ~(M=100)
LSH-RkNN
&
{\bf 0.61$\pm$0.17}
&0.40$\pm$0.13
&0.25$\pm$0.09
\\
% 
% 0.68$\pm$0.15
% &0.51$\pm$0.16
% &0.94$\pm$0.04
% \\
% 
% \midrule
% \\
% 
\midrule
% Our Kernel-RMM
% % ~(M=300)
LSH-RMM
&
\bf{0.61$\pm$0.17}
&\bf{0.41$\pm$0.13}
&0.25$\pm$0.09
\\
% 
% \midrule
% \\
% 
\midrule
% Our Neural-RLSTM
LSH-RLSTM
&
0.60$\pm$0.18
&0.39$\pm$0.13
&0.24$\pm$0.09
\\
% 
% 
\toprule
\end{tabular}
}
% 
% 
% \newline
% 
% 
\subtable[
Larry King Dataset
]
{
\centering
\renewcommand{\arraystretch}{1.4}% Tighter
\renewcommand{\tabcolsep}{12.75pt}
\begin{tabular}{llllllllllll}
\toprule	
% \textbf{Datasets}
% 
% &
\textbf{Model}
& 
Average
& Greedy
& Extrema
% & DR
\\
% 
\toprule
%
% 
% LSTM
% &
% 0.78$\pm$0.24
% &0.66$\pm$0.20
% &0.38$\pm$0.13
% \\
% 
% 
LSTM~\protect\cite{vinyals2015neural}
&
0.71$\pm$0.24
&0.60$\pm$0.20
&0.35$\pm$0.14
\\
% 
% 
\midrule
% 
% \bf{0.79$\pm$0.23}
% &\bf{0.81$\pm$0.22}
% &\bf{0.49$\pm$0.17}
% \\
%
% 
HRED~\protect\cite{serban2016building}
&
0.71$\pm$0.25
&0.61$\pm$0.20
&0.29$\pm$0.12
\\
% 
% 
\midrule
VHRED~\protect\cite{serban2017hierarchical}
&
0.70$\pm$0.24
&\bf{0.72$\pm$0.25}
&\bf{0.43$\pm$0.18}
\\ 
% 
% 
\toprule
% Our Kernel-RkNN
% % ~(M=100)
LSH-RkNN
&
{\bf 0.76$\pm$0.28}
&0.60$\pm$0.21
&0.34$\pm$0.15
\\
% 
% \midrule
% \\
% 
\midrule
% Our Kernel-RMM
% % ~(M=300)
% \bf{0.78}$\pm$0.26
% &0.61$\pm$0.20
% &0.35$\pm$0.15
% \\
%
LSH-RMM
&
0.73$\pm$0.28
&0.59$\pm$0.22
&0.35$\pm$0.16
\\
% 
% 
% \midrule
% \\
% 
\midrule
% Our Neural-RLSTM
LSH-RLSTM
&
\bf{0.76$\pm$0.27}
&0.58$\pm$0.21
&0.33$\pm$0.15
\\
% 
% 
\toprule
\end{tabular}
}
% 
% \vspace{-4mm}
% 
\caption{
Comparison between state-of-art neural network models (LSTM, HRED and VHRED) and the proposed hashing models (LSH-RkNN, LSH-RMM and LSH-RLSTM), on  three datasets -- Depression Therapy,  Twitter, and Larry King data -- using word embedding-based   similarity metrics between the actual and generated responses.       
% 
Mean and standard deviation across samples (response pairs) are reported for all metrics, for each test set except for Twitter results with prior art  models~(LSTM, HRED, VHRED) - we used the numbers reported in \protect\cite{serban2017hierarchical}, without rerunning the models; standard deviations were not  reported   in that paper.}
\label{tab:results}
% \vspace{-4.25mm}
\end{table*}


==> hashingAlgo.tex <==
\begin{algorithm}[tp!]
\caption{
\csize
% Generic 
Generalized Algorithm for Constructing
% ~(Kernel) 
Locality Sensitive Hash Functions, with Kernel Functions or Neural Networks}
\csizenine
\begin{algorithmic}[1]
\REQUIRE Reference set $\bs{S}^R$, of size $M$; sub-sampling parameter, $\alpha$; number of hash functions, $H$.
% 
% \COMMENT{Random subsets, fixed across structure inputs}
% 
\STATE $\bs{z} \gets \{ \bs{0}_{\alpha}, \bs{1}_{\alpha} \}$
% 
% \COMMENT{labels for hash code bit}
% 
% \STATE $\bs{K}_{RR} \gets$ computeKernel($\bs{S}^R$, $\bs{S}^R$)
% \COMMENT{kernel matrix of size $M \times M$}
\FOR{$l=1 \to H$}
% 
\STATE $\bs{S}^R_l \gets$ randomSubset($\bs{S}^R$, $2\alpha$)
% 
\COMMENT{random subset from $\bs{S}^R$ of size $2\alpha$, $\bs{S}^R_l$}
% 
\STATE $\cH_l(.) \gets$ TrainBinaryClassifierAsHashFunction$\left(\bs{S}^{R}_l, \bs{z}\right)$
\ENDFOR
% 
\RETURN $\bs{\cH(.)} = \{ \cH_1(.), \cdots, \cH_H(.) \}$
% 
\end{algorithmic}
\label{alg:our_algo_klsh_codes}
\end{algorithm}


==> intro_AISTATS.tex <==
\section{Introduction}
% 
Dialogue modeling and generation is an area of active research, and of great practical importance, as it provides a basis for building successful conversational agents in a wide range of applications.  While an open-domain dialogue remains a highly challenging open problem,  developing dialogue systems for particular applications can be more tractable,  due to specific properties of the application domain.

In our work, one of the motivating application is a fast-growing area of  (semi-)automated psychotherapy:  easily accessible, round-the-clock psychotherapeutic services provided by a conversational agent. According to recent estimates, mental health disorders affect one in four adult Americans, one in six adolescents, and one in eight children. Furthermore, as  predicted by the World Health Organization, by 2030 the amount of worldwide disability and life loss attributable to depression may become greater than for any other condition, including cancer, stroke, heart disease, accidents, and war. However, many people do not receive an adequate treatment; one of the major factors here is  limited availability of mental health care professionals, as compared to the number of potential patients. Thus, creating automated systems providing mental health services is becoming an increasingly important area of research and development; nevertheless, existing conversational systems in this domain are still primarily rule-based, and lack sophisticated dialogue modeling and generation capabilities based on actual text understanding.

\begin{table}
\centering
% \tabsize
% \csizeten
\csizenine
% \fontsize{8}{8}\selectfont
% \renewcommand{\arraystretch}{0.9}% Tighter
% \scriptsize
\begin{tabular}{p{7.75cm}}
\toprule
% % CLIENT: 
% But for the next person I mean. I deal with - that's part of what I do is I train people. I'm always - I'm either training people on this computer or what I like to do more is training people how to understand and train.
% And so I have - I feel bad when I give up on a trainer, you know. I just don't think she has it. It's - and I have met people who have had tremendous, tremendous abilities of being able to like grasp concepts and communicate them to others who I had more belief in, you know. [00:16:13]
% Does that make - I guess that...
% ((Crosstalk))\\
% 0101001111001011111110101101111111011011100011101100111000101011110111001001011011001110001010100100
% \\
% \\
% \thp{
% % THERAPIST: 
% For now it's just you don't - can't see like A, (inaudible at 00:16:25) a look at yourself and B, can't see her dealing well with anybody else.}\\
% \thp{
% 0101001111011011111100101101111110011011100001000100111100101000110111001001011111001110001000001000
% }
% \\
% \midrule
% % CLIENT: 
% My dad actually seems in, um, better shape health-wise than he has in a while. I was worried about him the last time I was down there, but the one thing I told him, I said, you know - we were - they had already been in town a few hours. I said, "You know, you haven't told me one story that you've already told me before." I said, "I don't know if you've changed your diet or something, but you're not as senile as you used to be." (Laughing.)\\
% % [00:03:27]\\
% 010100111100101111110010110111111001101110001100010011110010100
% % 1110111001101011111011110001000000000
% \\
% \\
% \thp{
% % THERAPIST: 
% (Laughing.)
% }
% \\
% \thp{
% 010110011011101111111011110011011010111111101111011011100010110
% % 1100011101010011011001110101000100000
% }
% \\
% \midrule
% PT:	
% I'll stay on the Restoril, I mean it takes me a while to go to sleep but I'll stay on the Restoril.
% \\
% 0101001111101111111110101101011110011010100011100101111000101011110111001001011011001110001010000110
% \\
% \\
% \thp{
% % DR:	
% Let's nudge the Pamelor up a little bit.  We could also check a blood level.
% }
% \\
% \thp{
% 0111001111001011111100101100111110011010110001001100111100101101010111001011011011111110001100000000
% }

% \thp{
% 010101011010111111111010110101111001101110000110010011100010101
% % 1110111001001011011001110001010100010
% }
% \\
%\midrule
% PATIENT: 
\textit{
Its all my fault. It's like getting hit in the stomach and trying to catch your breath. You can't catch it. You struggle, move around, you just can't get your breath. That just really knocks me off balance. You begin to generate this feeling of a kind of negativism...
%And that's why it really being hurt. I never allowed myself to think negative, accept everybody else. I am the only one giving back to the "be quiet time." I had to have something to make do with that.
}
\\
{\bf 0101001111001011111110101101011110011011100011101}
% 1001110
% 0010100
% 1110111101011011011001110001000000000
\\
\thp{
% COUNSELOR: 
\textit{
OK. Maybe that fits into the whole pattern then.
}
}\\
\thp{
0111001101001011111100011111111110001010110011001
% 1001110
% 0010110
% 0010111101010011011011110001100001000
}
\\
% \midrule
% CLIENT: 
% \textit{
% Well I talked to a friend of mine whom I think is promiscuous and she told me about a man that came to see her at her apartment. So I gave him my phone number. I don't have any hang up about morals. I don't know. I told a couple of my friends about this. I must admit I'm a little shy talking about it now.
% % [0:23:27.1]
% }
% \\
% 010100011010101111111010110101111001101110000110010011100010100
% % 1110111001011011011001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% I see. You mean it's embarrassing to tell me about it.
% }
% }
% \\
% \\
% \midrule
% % PT: 
% \textit{
% Yeah.  I didn't think she was going to die.
% }
% \\
% 010100011010101111111010110001111001001110001110010011100010101
% % 1110111101001011011001110001000100010
% \\
% \\
% \thp{
% % DR: 
% \textit{
% Yeah.
% }
% }\\
% \thp{
% 010110011011100111111010110001111110101111100110011011110010111
% % 1010111101010011010101110101010100010
% }
% \\
% 
% \midrule
% CLIENT: So I filed a bug report on Wednesday.\\
% \\
% THERAPIST: Yeah.\\
% 
% \midrule
% % PATIENT: 
% \textit{
% I'm sitting here just thinking about things. Should I think out loud? (chuckles)
% }
% \\
% 01010001111010111111001111011111110010111000011001
% 00111000101011110111001101011001001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% Sure. If you want to.
% }
% }
% \\
% \thp{
% 11010011001110111111001011011101110100111000111011
% 00111100101001110111101100011001001110001010000000}
% \\
% \midrule
% % CLIENT: 
% \textit{
% Because it's almost a year of my life.
% }
% \\
% 01010011110010111111001011010111101100101100110011
% 00111100101101110111101011011011011110001000100000\\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% All this is. It's a good chunk of time.
% }
% }\\
% \thp{
% 01010011010010111111001011010111101010101000110011
% 00111100101101110111101011011011001110001000100000
% }\\
% 
% \midrule
% % PATIENT: 
% \textit{
% Most of it is small bills. There's one 50 dollar check, and that's the only thing that's really large. The rest of it's like ten or twelve dollars each.
% }\\
% 010100110100101111110010110111111001101111001100110011110010110
% % 0110111101011011011011110001000101000
% \\
% \\
% \thp{
% % THERAPIST: 
% \textit{
% But it adds up.
% }
% }
% \\
% \thp{
% 010101111110101111111011110101111000101110000110010011100010100
% % 111011110
% % 1111011011001110001010100010
% }
% \\
\toprule
\end{tabular}
\vspace{-3.25mm}
\caption{
\small
% \fontsize{8}{8}\selectfont
An example of patient/therapist responses in a depression therapy session, with associated binary hashcodes; patient's hashcode will be used as a feature vector to predict the bits of the  therapist hashcode. 
%In this table, we show pairs of patient and therapist~(Blue) responses.
% , randomly sampled from different sessions.
% ; the responses of therapists are in red. 
%For each response, we obtain a locality sensitive hashcode as its representation.
% , of 100 bits each. 
%The hashcode of a patient response is used as feature representation to infer the hashcode of the corresponding therapist response.
% as multi-class labels.
}
\label{tab:therapy_session_hashcoded}
\vspace{-6mm}
\end{table}%
% 
% \input{tabResponseHashcodes.tex}

An interesting feature of therapeutic dialogues appears to be a classical pattern of a relatively long monologue of  a patient followed by a considerably shorter  response of  a therapist; this property is also shared with some other types of dialogues, e.g., TV show interviews such as Larry King dataset analyzed in this paper, where the guest of a show produces relatively long monologues, with the host inserting relatively short comments. Moreover, therapist's responses tend to be rather  high-level, generic statements, typically summarizing/confirming the patient's response, and can be viewed as a ``category label" being ``assigned" to a patient's text ``sample". Generating such a short, constrained  response can be a somewhat easier task than solving the open-domain dialogue challenge. 

Rather than  generating a specific response sentence directly, a more effective approach can be to first infer a conceptual, high-level representation reflecting the essence of the ``most relevant" response to the patient. Furthermore, it is desirable to optimize representation models with the objective of increasing relevance, or coherence, between the consecutive responses, as well as predictability of one response from another, to facilitate better dialog generation -- the objective likely to be  captured by the notion of {\em mutual information} between the responses.

Note that a fundamental concept in psychotherapy is the working alliance between the therapist and the patient or, more generally, the client seeking help~\cite{bordin1979generalizability}. The alliance involves several cognitive and emotional components of the relationship between these two agents, including the agreement on the goals to be achieved and the tasks to be carried out, and the bond, trust and respect to be established over the course of the therapy. While an encompassing formalization of working alliance is a challenging task, it is however reasonable to consider that the  mutual information criterion may capture, to some extent, the dynamics of agreement expected to develop in most therapies, and, more generally, in other types of dialogues.
            
Motivated by above considerations,  we  introduce here  a novel dialogue modeling framework where responses are represented as \emph{locality-sensitive binary hashcodes}~\cite{kulis2009kernelized,joly2011random,garg2018efficient}, and the hashing models are optimized using a {\em novel mutual-information lower bound}, as mutual information computation is intractable in high-dimensional spaces. Using hashcode representations may allow for 
a more tractable way of  predicting responses in a compressed, general representation space instead of direct generation of textual responses.
(Note that hashcode representations were  successfully applied in prior work on  information-extraction   \cite{garg2018efficient}). Furthermore, separating inference in representation space from text generation (based on inferred response representation) increases method's flexibility, while mutual information criterion facilitates better alignment between the responses of two parties and higher predictability of the proper response. While the  psychotherapy domain was our primary motivation, the proposed approach is generally   applicable to a wider range of   domains as demonstrated in empirical section. Overall, our  \emph{key contributions} include:
% 
(1) a novel  generic framework for dialogue modeling and generation using \emph{locality sensitive hash functions};
(2) a \emph{novel lower bound on the Mutual Information~(MI)} between the hashcodes of the responses from the two agents used as an optimization criterion for the locality sensitive hash functions;
(3) an extensive empirical evaluation on three different dialogue domains, from depression therapy to TV show interviews and Twitter data,  demonstrating competitiveness   of our approach when compared with the state-of-art neural network based dialog systems, and its clear superiority in case of relatively small datasets (e.g., therapy sessions), both in terms of the quality of generated responses and computational efficiency.
  

==> lstm.tex <==
\section{Neural Networks}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.46\textwidth]{LSTM_dialog.pdf}
    \caption{Hashcode generation using neural models: To generate hashcodes using neural models, we train the LSTM model to fit the labels for reference set of dialogs. Each dialog in the reference set is input as a sequence of individual word embeddings into an LSTM/GRU model with $k$ layers, each layer containing a specific number of LSTM units. The model is then evaluated on the rest of the dialogues to obtain a single bit in the hashcode. The process is repeated with different reference sets to generate the hashcode.}
    \label{fig:schema}
\end{figure}
In addition to kernel similarity functions, we explore using neural networks to generate hashcodes. For each reference set defined above, we learn a recurrent neural network model to predict the randomly assigned labels. The model learns a non-linear mapping which is then used to obtain a single hashcode bit for the remaining text. For kernel based methods we optimize the reference set of dialogs. However, for neural models, we optimize the hyperparameters of the model which consists of the number of layers and the number of neurons in each layer. For each configuration, we compute the mutual information of responses and use the parameters which generate the highest value. For simplicity, we do not vary the activation function and learning rate. We train our model using Adam~\cite{kingma2014adam} and the gradients are calculated using back propagation.
	
In our experiments, we vary the neural network model size. We test models with 1 to 3 layers. To determine the number of neurons for each layer, we perform a grid search over $[8, 16, 32, 64, 128]$. As the number of instances in our training data is very small, the above configurations suffice in capturing the data. We use a sigmoid layer for final prediction and a fixed learning rate of $10^{-3}$.

==> mainTable.tex <==
\begin{table*}[tp!]
\centering
\tabsize
% \renewcommand{\arraystretch}{0.8}% Tighter
\renewcommand{\tabcolsep}{2.0pt}
% 
\begin{tabular}{llllllllllll}
\toprule	
Hashing Func.&Hash Config.
% ~(Optimization)
&Model
& \textbf{MI LB}~(Shuffled)
&\textbf{Entropy UB}
% 
% &MI LBs Ratio
% 
&NMI LB (Shuffled)
% 
% &Marginal CE UB
% &\textbf{Inference}~(Marginal MI LB)
&Accuracy~(Baseline)
% Accuracy)\\
% &Marginal E.
% &TC Bound
\\
% 
\midrule
% 
% \textbf{
Kernel-RkNN&M=30, $\alpha$=10&
% }
\\
% \midrule
% &Random*&$82.61\pm17.85$~($77.84\pm20.55$)&$-13.83\pm1.57$&$33.49\pm0.12$&$17.45\pm1.54$&$29.88\pm0.12$\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% 
% 
% % &
% &$-14.6\pm2.6$
% &$15.3\pm2.6$
% % &$3.6\pm0.2$
% &$82.6\pm17.9$~($77.8\pm20.6$)
% %&$33.49\pm0.12$
% % &$18.22\pm2.55$
% % &$29.85\pm0.10$
% \\
% % 
% 
% &
&$-12.1\pm4.4$~($-12.1\pm2.4$)
&$5.1\pm4.6$
%
% &1.0
&N.A.
% 
% &$17.2\pm0.4$
% 
% &$1.7\pm0.5$
&$93.6\pm8.6$~($89.4\pm12.2$)
%&$18.87\pm0.36$
% &$13.14\pm4.69$
\\
% 
% 
% % &
% &$-8.2\pm5.3$
% &$19.5\pm5.3$
% % &$6.0\pm0.3$
% &$85.2\pm14.0$~($79.0\pm16.3$)
% %&$33.68\pm0.25$
% % &$14.17\pm5.27$
% % &$27.68\pm0.19$
% \\
% 
% 
% % &
% &$-9.7\pm1.0$
% &$5.6\pm1.0$
% % &$1.1\pm0.4$
% &$93.7\pm10.5$~($90.4\pm14.2$)
% %&$16.36\pm0.27$
% % &$10.78\pm0.98$
% % &$15.30\pm0.25$
% \\
% 
% 
% % &
% &$-11.7\pm0.8$
% &$17.2\pm0.9$
% % &$3.4\pm0.3$
% &$85.2\pm15.5$~($79.8\pm18.2$)
% %&$32.27\pm0.19$
% % &$15.06\pm0.91$
% % &$28.92\pm0.20$
% \\
%
% 
% &&$\pm$~($\pm$)&$-7.88\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$-9.38\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$-6.04\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% 
% \midrule
% 
% 
% &MI LB Opt~($\gamma=100,\beta=300$)&$87.27\pm15.80$~($82.90\pm18.51$)&$-6.66\pm0.39$&$27.22\pm0.25$&$10.72\pm0.42$&$23.16\pm0.27$&$16.5\pm$&$4.06\pm$\\
% % 
% % 
% &MI LB Opt~($\gamma=300,\beta=300$)&$90.42\pm11.44$~($85.75\pm14.88$)&$-4.71\pm0.65$&$24.10\pm0.25$&$9.26\pm0.64$&$19.55\pm0.20$&$14.84\pm$&$4.55\pm$\\
% % 
% % 
% &MI LB Opt~($\gamma=1000,\beta=300$)&$91.54\pm10.86$~($87.11\pm15.09$)&$-3.99\pm0.49$&$21.54\pm0.15$&$6.94\pm0.53$&$18.60\pm0.26$\\
% % 
% % 
% &MI LB Opt~($\gamma=300,\beta=1000$)&$\pm$~($\pm$)&$-4.65\pm1.11$&$\pm$&$\pm$&$\pm$\\
% 
% 
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{-4.2\pm1.2}$~($-9.5\pm0.2$)
&$\bs{30.2\pm1.1}$
% 
% &2.26
% 
&N.A.
% 
% &$34.5\pm0.2$
% 
% &$12.2\pm0.3$
&$\bs{75.3\pm16.5}$~($68.7\pm17.4$)
%&$46.62\pm0.17$
% &$16.57\pm0.75$
\\
% 
% 
% &MI Opt&&&&&\\
% 
\midrule
% 
Kernel-RkNN&M=100, $\alpha$=10\\
% \midrule
% &Random*&$83.13\pm15.76$~($78.57\pm17.38$)&$16.00\pm0.35$&$33.82\pm0.24$&$6.47\pm0.25$&$11.35\pm0.23$\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% 
% 
% % &
% &$16.0\pm0.3$
% &$27.4\pm0.4$
% % &$22.5\pm0.3$
% &$83.1\pm15.8$~($78.6\pm17.4$)
% % &$33.84\pm0.24$
% % &$6.49\pm0.27$
% % &$11.32\pm0.21$
% \\
% 
% 
% % &
% &$7.2\pm0.4$
% &$19.3\pm0.4$
% % &$13.5\pm0.3$
% &$87.6\pm15.8$~($84.3\pm17.4$)
% % &$25.58\pm0.19$
% % &$6.28\pm0.37$
% % &$12.13\pm0.17$
% \\
% % 
% 
% % &
% &$12.2\pm0.3$
% &$21.7\pm0.3$
% % &$16.8\pm0.2$
% &$87.6\pm14.6$~($83.9\pm16.8$)
% % &$26.19\pm0.17$
% % &$4.59\pm0.19$
% % &$9.42\pm0.14$
% \\
% % 
% 
% % &
% &$5.3\pm0.3$
% &$16.9\pm0.3$
% % &$9.8\pm0.4$
% &$90.5\pm13.5$~($87.2\pm15.9$)
% % &$21.35\pm0.27$
% % &$4.49\pm0.13$
% % &$11.53\pm0.23$
% \\
% 
% 
% &
&$9.9\pm0.4$~($4.3\pm0.2$)
&$19.9\pm0.3$
% 
% &2.3
% 
&0.50~(0.22)
% 
% &$10.0\pm0.2$
% 
% &$15.6\pm0.3$
&$88.3\pm13.9$~($84.7\pm16.0$)
% &$25.58\pm0.19$
% &$5.73\pm0.24$
\\
% 
% 
% \midrule
% 
% &MI LB Opt~($\gamma=100,\beta=300$)&$85.15\pm15.44$~($80.89\pm17.77$)&$7.43\pm0.90$&$30.46\pm0.19$&$9.43\pm0.88$&$13.60\pm$0.26&$21.03\pm$&$16.86\pm$\\
% % 
% % \midrule
% &MI LB Opt~($\gamma=300,\beta=300$)&$86.25\pm14.49$~($82.13\pm16.51$)&$11.26\pm0.48$&$29.17\pm0.21$&$7.45\pm0.46$&$10.46\pm0.12$&$21.72\pm$&$18.71\pm$\\
% % 
% % 
% &MI LB Opt~($\gamma=1000,\beta=300$)&$\pm$~($\pm$)&$8.03\pm0.28$&$\pm$&$\pm$&$11.59\pm$\\
% 
% 
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{13.5\pm0.4}$~($5.6\pm0.3$)
&$\bs{26.1\pm0.3}$
% 
% &2.4
% 
&0.52~(0.21)
% 
% &$12.6\pm0.2$
% 
% &$21.8\pm0.4$
&$82.7\pm16.2$~($78.4\pm17.3$)
% &$34.42\pm0.20$
% &$8.22\pm0.35$
\\
% 
% 
\midrule
% 
Kernel-RkNN&M=300, $\alpha$=10&\\
% \midrule
% &Random*&$87.61\pm15.24$~($84.11\pm17.02$)&$13.36\pm0.27$&$26.08\pm0.18$&$4.57\pm0.10$&$8.15\pm0.14$\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% % &
% &$13.4\pm0.2$
% &$21.6\pm0.2$
% % &$17.9\pm0.2$
% &$87.6\pm15.3$~($84.1\pm17.0$)
% % &$26.08\pm0.17$
% % &$4.51\pm0.13$
% % &$8.18\pm0.15$
% \\
% % 
% % &
% &$15.5\pm0.4$
% &$25.3\pm0.3$
% % &$22.6\pm0.3$
% &$84.0\pm15.6$~($79.6\pm17.3$)
% % &$32.45\pm0.17$
% % &$7.16\pm0.28$
% % &$9.82\pm0.24$
% \\
% % 
% &
&$\bs{15.3\pm0.2}$~($8.6\pm0.1$)
&$22.7\pm0.2$
%
% &1.8
% 
&\textbf{0.67~(0.38)}
% 
% &$7.4\pm0.2$
% 
% &$19.0\pm0.3$
&$87.6\pm14.7$~($83.9\pm16.6$)
% &$26.43\pm0.18$
% &$3.83\pm0.18$
\\
% 
% % &
% &$10.3\pm0.2$
% &$17.6\pm0.3$
% % &$14.2\pm0.3$
% &$90.6\pm12.1$~($87.3\pm14.8$)
% % &$21.49\pm0.20$
% % &$3.94\pm0.17$
% % &$7.28\pm0.16$
% \\
% % 
% % &
% &$15.3\pm0.5$
% &$24.6\pm0.5$
% % &$22.7\pm0.3$
% &$84.1\pm15.8$~($79.8\pm17.9$)
% % &$32.06\pm0.14$
% % &$7.43\pm0.47$
% % &$9.38\pm0.22$
% \\
% % 
% 
% \midrule
% &MI LB Opt~($\gamma=100,\beta=300$)&$82.97\pm17.36$~($79.03\pm19.01$)&$17.11\pm0.40$&$32.73\pm0.15$&$6.37\pm0.29$&$9.26\pm0.22$&$26.36\pm$&$23.47\pm$\\
% 
% 
% \midrule
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{15.7\pm0.3}$~($8.4\pm0.2$)
&$\bs{24.0\pm0.3}$
% 
% &1.9
% 
&0.65~(0.35)
% 
% &$8.3\pm0.2$
% 
% &$20.8\pm0.3$
&$85.8\pm16.0$~($82.0\pm17.6$)
% &$29.07\pm0.27$
% &$5.05\pm0.17$
\\
% 
% 
% \toprule
% \textbf{M=100}~(RMM, C=1.0)\\
% \midrule
% % &
% \textbf{Random}\\
% % Reference Set\\
% % 
% % &
% &$73.84\pm12.43$~($65.52\pm12.10$)&$21.63\pm0.62$
% &$52.10\pm0.25$&$13.97\pm0.68$&$16.50\pm0.40$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$23.89\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$23.55\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$24.00\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% % &
% &$\pm$~($\pm$)&$25.25\pm$
% &$\pm$&$\pm$&$\pm$
% % &$\pm$&$\pm$
% \\
% % 
% % 
% \midrule
% % 
% % &
% \textbf{MI LB Opt}
% % ~($\gamma=100,\beta=1000$)
% &$73.55\pm11.36$~($65.00\pm11.08$)&$21.72\pm0.89$&$52.85\pm0.23$&$14.32\pm0.68$&$16.82\pm0.40$\\
% % 
% % 
% 
\midrule
% 
% \toprule
Kernel-RMM&M=100, $\alpha$=10\\
% ~(RMM, C=0.1)\\
% \midrule
% &
&&Random Sel.
% \\
% Reference Set\\
% 
% % &
% &$10.9\pm0.3$
% &$24.5\pm0.5$
% % &$23.8\pm0.6$
% &$84.2\pm11.7$~($77.4\pm13.0$)
% % &$37.48\pm0.46$
% % &$12.94\pm0.26$
% % &$13.69\pm0.44$
% \\
% % 
% % 
% % &
% &$14.4\pm0.3$
% &$26.4\pm0.4$
% % &$25.2\pm0.5$
% &$83.7\pm13.1$~($77.3\pm14.2$)
% %&$37.16\pm0.40$
% % &$10.76\pm0.18$
% % &$11.97\pm0.31$
% \\
% % 
% 
% &
&$10.0\pm0.5$~($3.5\pm0.1$)
&$23.2\pm0.3$
% 
% &2.9
% 
&0.43~(0.15)
% 
% &$13.3\pm0.4$
% 
% &$21.3\pm0.6$
&$85.9\pm11.5$~($79.3\pm13.3$)
%&$34.50\pm0.45$
% &$11.28\pm0.28$
\\
% 
% % 
% % &
% &$8.4\pm0.4$
% &$21.7\pm0.5$
% % &$20.1\pm0.6$
% &$86.8\pm10.6$~($80.2\pm12.9$)
% %&$33.46\pm0.40$
% % &$11.73\pm0.26$
% % &$13.39\pm0.43$
% \\
% % 
% % 
% % &
% &$7.2\pm0.4$
% &$20.7\pm0.6$
% % &$20.2\pm0.7$
% &$86.6\pm10.9$~($80.1\pm13.2$)
% % &$33.64\pm0.49$
% % &$12.98\pm0.29$
% % &$13.44\pm0.46$
% \\
% % 
% 
% \midrule
% 
% &
&&MI LB Opt.
% ~($\gamma=100,\beta=1000$)
&$\bs{11.4\pm0.5}$~($2.8\pm0.2$)
&$\bs{26.0\pm0.6}$
% 
% &\textbf{4.1}
% 
&\textbf{0.44~(0.11)}
% 
% &$14.6\pm0.4$
% 
% &$26.4\pm0.6$
&$\bs{82.0\pm11.6}$~($74.5\pm13.2$)
%&$40.96\pm0.41$
% &$15.01\pm0.37$
\\
% 
\midrule
% 
% \toprule
Kernel-RMM&M=300, $\alpha$=10\\
% ~(RMM, C=0.1)\\
% \midrule
% &
&&Random Sel.
% 
&$10.3\pm0.4$~($3.6\pm0.1$)
&$22.1\pm0.3$
&0.47~(0.16)
&$86.2\pm11.9$~($79.9\pm14.0$)
\\
% 
% 
\toprule
% 
Neural-RLSTM
&M=76000, $\alpha$=50
% \\
% 
% &&[10]-Random Selection&$6.7\pm0.3$&$27.1\pm0.5$
% &$68.3\pm10.7$~($62.9\pm9.5$)
% \\
% % 
% % 
% &&[10,10]-Manual Fine Tuned&$\bs{19.8}\pm1.0$&$34.2\pm0.2$
% &$\bs{63.4}\pm11.8$~($56.6\pm9.2$)
\\
% 
&&
% % [20,20]-MI LB Optimal
% MI LB Optimal
% &$\bs{19.1\pm0.7}$~($-0.5\pm0.4$)
% &$\bs{32.3}\pm0.5$
% &$13.2\pm0.2$
% &$61.4\pm13.7$~($56.4\pm11.1$)
% 
% 
% [16, 64, 16, 8]-MI LB Optimal
% 
MI LB Opt.
&$\bs{17.2\pm0.3}$~($8.0\pm0.2$)
&$23.2\pm0.3$
% 
% &2.2
% 
&\textbf{0.74~(0.34)}
% 
% &$6.0\pm0.1$
% 
&$84.6\pm17.2$~($79.9\pm19.9$)
\\
\toprule
\end{tabular}
% \vspace{-3.5mm}
\caption{
Evaluating the quality inference of dialogue responses (hashcodes), for the depression psychotherapy dataset.
}
\label{tab:results}
% \vspace{-5.5mm}
\end{table*}


% \begin{table*}[tp!]
% \centering
% \tabsize
% % \tiny
% % \scriptsize
% % \renewcommand{\arraystretch}{0.85}% Tighter
% % \renewcommand{\tabcolsep}{3pt}
% % 
% \begin{tabular}{lllllllllll}
% \toprule	
% \textbf{Configurations}
% % ~(Optimization)
% &\textbf{MI LB}
% &\textbf{Quality}&\textbf{Inference}
% &Accuracy~(Random Baseline)
% % Accuracy)\\
% % &Marginal E.&TC Bound&C.E. Bound
% \\
% \toprule
% \textbf{M=30~(RkNN)}\\
% % \midrule
% % &Random*&$82.61\pm17.85$~($77.84\pm20.55$)&$-13.83\pm1.57$&$33.49\pm0.12$&$17.45\pm1.54$&$29.88\pm0.12$\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % 
% % 
% % &
% &$-14.59\pm2.62$
% &$15.27\pm2.55$&$3.64\pm0.16$
% &$82.60\pm17.86$~($77.84\pm20.55$)
% %&$33.49\pm0.12$&$18.22\pm2.55$&$29.85\pm0.10$
% \\
% % 
% % 
% % &
% &$-11.47\pm4.64$
% &$5.73\pm4.70$&$1.67\pm0.52$
% &$93.56\pm8.54$~($89.45\pm12.14$)
% %&$18.87\pm0.36$&$13.14\pm4.69$&$17.20\pm0.37$
% \\
% % 
% % 
% % &
% &$-8.16\pm5.25$
% &$19.51\pm5.28$&$6.0\pm0.31$
% &$85.22\pm13.97$~($79.01\pm16.25$)
% %&$33.68\pm0.25$&$14.17\pm5.27$&$27.68\pm0.19$
% \\
% % 
% % 
% % &
% &$-9.71\pm0.95$
% &$5.58\pm1.02$&$1.06\pm0.37$
% &$93.70\pm10.50$~($90.41\pm14.24$)
% %&$16.36\pm0.27$&$10.78\pm0.98$&$15.30\pm0.25$
% \\
% % 
% % 
% % &
% &$-11.72\pm0.79$
% &$17.21\pm0.93$&$3.35\pm0.28$
% &$85.16\pm15.54$~($79.79\pm18.21$)
% %&$32.27\pm0.19$&$15.06\pm0.91$&$28.92\pm0.20$
% \\
% %
% % 
% % &&$\pm$~($\pm$)&$-7.88\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$-9.38\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$-6.04\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% % &&$\pm$~($\pm$)&$\pm$&$\pm$&$\pm$&$\pm$\\
% % 
% \midrule
% % 
% % 
% % &MI LB Opt~($\gamma=100,\beta=300$)&$87.27\pm15.80$~($82.90\pm18.51$)&$-6.66\pm0.39$&$27.22\pm0.25$&$10.72\pm0.42$&$23.16\pm0.27$&$16.5\pm$&$4.06\pm$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=300,\beta=300$)&$90.42\pm11.44$~($85.75\pm14.88$)&$-4.71\pm0.65$&$24.10\pm0.25$&$9.26\pm0.64$&$19.55\pm0.20$&$14.84\pm$&$4.55\pm$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=1000,\beta=300$)&$91.54\pm10.86$~($87.11\pm15.09$)&$-3.99\pm0.49$&$21.54\pm0.15$&$6.94\pm0.53$&$18.60\pm0.26$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=300,\beta=1000$)&$\pm$~($\pm$)&$-4.65\pm1.11$&$\pm$&$\pm$&$\pm$\\
% % 
% % 
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$-4.41\pm0.77$
% &$30.05\pm0.77$&$12.16\pm0.28$
% &$75.27\pm16.48$~($68.73\pm17.42$)
% %&$46.62\pm0.17$&$16.57\pm0.75$&$34.46\pm0.22$
% \\
% % 
% % 
% % &MI Opt&&&&&\\
% \toprule
% \textbf{M=100~(RkNN)}\\
% % \midrule
% % &Random*&$83.13\pm15.76$~($78.57\pm17.38$)&$16.00\pm0.35$&$33.82\pm0.24$&$6.47\pm0.25$&$11.35\pm0.23$\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % 
% % 
% % &
% &$16.03\pm0.28$
% &$27.35\pm0.36$&$22.52\pm0.32$
% &$83.12\pm15.77$~($78.56\pm17.38$)
% % &$33.84\pm0.24$&$6.49\pm0.27$&$11.32\pm0.21$
% \\
% % 
% % 
% % &
% &$7.17\pm0.41$
% &$19.30\pm0.42$&$13.45\pm0.25$
% &$87.56\pm15.77$~($84.26\pm17.40$)
% % &$25.58\pm0.19$&$6.28\pm0.37$&$12.13\pm0.17$
% \\
% % 
% % 
% % &
% &$12.18\pm0.30$
% &$21.7\pm0.25$&$16.77\pm0.22$
% &$87.64\pm14.60$~($83.89\pm16.78$)
% % &$26.19\pm0.17$&$4.59\pm0.19$&$9.42\pm0.14$
% \\
% % 
% % 
% % &
% &$5.33\pm0.28$
% &$16.86\pm0.30$&$9.82\pm0.35$
% &$90.45\pm13.54$~($87.18\pm15.88$)
% % &$21.35\pm0.27$&$4.49\pm0.13$&$11.53\pm0.23$
% \\
% % 
% % 
% % &
% &$9.82\pm0.41$
% &$19.85\pm0.31$&$15.55\pm0.28$
% &$88.29\pm13.90$~($84.64\pm16.05$)
% % &$25.58\pm0.19$&$5.73\pm0.24$&$10.03\pm0.21$
% \\
% % 
% % 
% \midrule
% % 
% % &MI LB Opt~($\gamma=100,\beta=300$)&$85.15\pm15.44$~($80.89\pm17.77$)&$7.43\pm0.90$&$30.46\pm0.19$&$9.43\pm0.88$&$13.60\pm$0.26&$21.03\pm$&$16.86\pm$\\
% % % 
% % % \midrule
% % &MI LB Opt~($\gamma=300,\beta=300$)&$86.25\pm14.49$~($82.13\pm16.51$)&$11.26\pm0.48$&$29.17\pm0.21$&$7.45\pm0.46$&$10.46\pm0.12$&$21.72\pm$&$18.71\pm$\\
% % % 
% % % 
% % &MI LB Opt~($\gamma=1000,\beta=300$)&$\pm$~($\pm$)&$8.03\pm0.28$&$\pm$&$\pm$&$11.59\pm$\\
% % 
% % 
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$13.58\pm0.45$
% &$26.20\pm0.40$&$21.79\pm0.35$
% &$82.74\pm16.15$~($78.35\pm17.30$)
% % &$34.42\pm0.20$&$8.22\pm0.35$&$12.63\pm0.29$
% \\
% % 
% % 
% \toprule
% \textbf{M=300~(RkNN)}\\
% % \midrule
% % &Random*&$87.61\pm15.24$~($84.11\pm17.02$)&$13.36\pm0.27$&$26.08\pm0.18$&$4.57\pm0.10$&$8.15\pm0.14$\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % &
% &$13.39\pm0.24$
% &$21.57\pm0.21$&$17.90\pm0.23$
% &$87.62\pm15.27$~($84.11\pm17.03$)
% % &$26.08\pm0.17$&$4.51\pm0.13$&$8.18\pm0.15$
% \\
% % 
% % &
% &$15.48\pm0.35$
% &$25.29\pm0.33$&$22.63\pm0.29$
% &$83.99\pm15.60$~($79.59\pm17.33$)
% % &$32.45\pm0.17$&$7.16\pm0.28$&$9.82\pm0.24$
% \\
% % 
% % &
% &$15.19\pm0.26$
% &$22.6\pm0.25$&$19.02\pm0.26$
% &$87.60\pm14.74$~($83.87\pm16.59$)
% % &$26.43\pm0.18$&$3.83\pm0.18$&$7.41\pm0.19$
% \\
% % 
% % &
% &$10.28\pm0.23$
% &$17.55\pm0.26$&$14.21\pm0.26$
% &$90.63\pm12.11$~($87.32\pm14.77$)
% % &$21.49\pm0.20$&$3.94\pm0.17$&$7.28\pm0.16$
% \\
% % 
% % &
% &$15.26\pm0.49$
% &$24.63\pm0.49$&$22.68\pm0.26$
% &$84.05\pm15.77$~($79.79\pm17.89$)
% % &$32.06\pm0.14$&$7.43\pm0.47$&$9.38\pm0.22$
% \\
% % 
% % 
% \midrule
% % &MI LB Opt~($\gamma=100,\beta=300$)&$82.97\pm17.36$~($79.03\pm19.01$)&$17.11\pm0.40$&$32.73\pm0.15$&$6.37\pm0.29$&$9.26\pm0.22$&$26.36\pm$&$23.47\pm$\\
% % 
% % 
% % \midrule
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$15.71\pm0.27$
% &$24.02\pm0.32$&$20.77\pm0.32$
% &$85.82\pm16.03$~($82.04\pm17.56$)
% % &$29.07\pm0.27$&$5.05\pm0.17$&$8.30\pm0.18$
% \\
% % 
% % 
% % \toprule
% % \textbf{M=100}~(RMM, C=1.0)\\
% % \midrule
% % % &
% % \textbf{Random}\\
% % % Reference Set\\
% % % 
% % % &
% % &$73.84\pm12.43$~($65.52\pm12.10$)&$21.63\pm0.62$
% % &$52.10\pm0.25$&$13.97\pm0.68$&$16.50\pm0.40$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$23.89\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$23.55\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$24.00\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % % &
% % &$\pm$~($\pm$)&$25.25\pm$
% % &$\pm$&$\pm$&$\pm$
% % % &$\pm$&$\pm$
% % \\
% % % 
% % % 
% % \midrule
% % % 
% % % &
% % \textbf{MI LB Opt}
% % % ~($\gamma=100,\beta=1000$)
% % &$73.55\pm11.36$~($65.00\pm11.08$)&$21.72\pm0.89$&$52.85\pm0.23$&$14.32\pm0.68$&$16.82\pm0.40$\\
% % % 
% % % 
% % 
% \toprule
% % 
% % \toprule
% \textbf{M=100~(RMM)}\\
% % ~(RMM, C=0.1)\\
% \midrule
% % &
% Random\\
% % Reference Set\\
% % 
% % &
% &$10.85\pm0.26$
% &$24.54\pm0.53$&$23.79\pm0.64$
% &$84.23\pm11.66$~($77.36\pm13.04$)
% % &$37.48\pm0.46$&$12.94\pm0.26$&$13.69\pm0.44$
% \\
% % 
% % 
% % &
% &$14.43\pm0.33$
% &$26.4\pm0.44$&$25.19\pm0.51$
% &$83.74\pm13.10$~($77.30\pm14.18$)
% %&$37.16\pm0.40$&$10.76\pm0.18$&$11.97\pm0.31$
% \\
% % 
% % 
% % &
% &$9.97\pm0.50$
% &$23.22\pm0.53$&$21.25\pm0.62$
% &$85.92\pm11.49$~($79.35\pm13.28$)
% %&$34.50\pm0.45$&$11.28\pm0.28$&$13.25\pm0.43$
% \\
% % 
% % 
% % &
% &$8.35\pm0.40$
% &$21.73\pm0.48$&$20.07\pm0.59$
% &$86.78\pm10.57$~($80.18\pm12.92$)
% %&$33.46\pm0.40$&$11.73\pm0.26$&$13.39\pm0.43$
% \\
% % 
% % 
% % &
% &$7.23\pm0.44$
% &$20.66\pm0.57$&$20.20\pm0.67$
% &$86.58\pm10.90$~($80.09\pm13.16$)
% % &$33.64\pm0.49$&$12.98\pm0.29$&$13.44\pm0.46$
% \\
% % 
% % 
% \midrule
% % 
% % &
% MI LB Opt
% % ~($\gamma=100,\beta=1000$)
% &$11.35\pm0.48$
% &$25.95\pm0.55$&$26.36\pm0.60$
% &$81.99\pm11.62$~($74.53\pm13.21$)
% %&$40.96\pm0.41$&$15.01\pm0.37$&$14.60\pm0.44$
% \\
% % 
% % % 
% % 
% % 
% \toprule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Evaluation of
% % for our approach of 
% inferencing dialog responses as hashcodes.
% }
% \label{tab:results}
% \vspace{-6.5mm}
% \end{table*}


==> proofsContent.tex <==
% \section{Theorems for Information Theoretic Bounds}
% \begin{theorem}[Lower Bound for Mutual Information]
% Mutual information between two hashcode distributions, $\cI(\bs{\cC_t}: \bs{\cC_p}; M_h)$, is lower bounded as,     
% % 
% % 
% % \vspace{-3mm}
% \begin{align}
% &
% % \csizenine
% \cI(\bs{\cC_t}: \bs{\cC_p}; M_h)
% % \nonumber
% % \\
% % &
% % &
% \ge
% % \nonumber
% % \\
% % &
% % \csizenine
% % \underbrace{
% \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% -
% \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% % }_{\text{quality of hashcodes as representations}}
% \nonumber
% \\
% &
% % \csizenine
% +
% % \underbrace{
% \sum\limits_j{\left\langle \log q(\bs{\cC_t}(j)|\bs{\cC_p}; M_h)
% \right\rangle_{p(\bs{\cC_t}(j),\bs{\cC_p}; M_h)}}.
% % }_{\text{inference of each hashcode bit}}
% \label{eqn:mi_lb}
% % \vspace{-4mm}
% \end{align}
% % 	
% \noindent The lower bound is cheaper and more accurately computable than the criterion itself.
% % 
% % \vspace{-3mm}
% \begin{align}
% \bs{\cY^*}
% \gets
% \mathop{\arg\max}
% \limits_{\bs{\cY}:|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t}:\bs{\cY}; M_h)
% \label{eqn:corex_opt_thm}
% % \vspace{-4.5mm}
% \end{align}
% % 
% % 
% Herein, $\cT\cC(\bs{\cC_t}:\bs{\cY}; M_h)$ describes the amount of \emph{Total Correlations~(Multi-variate Mutual Information)}~\footnote{The ``total correlation" quantity, also called as multi-variate Mutual Information, or multi-information, was defined in \cite{watanabe1960information,studeny1998multiinformation,kraskov2005hierarchical}.} within $\bs{\cC_t}$ that can be explained by a latent variables representation $\bs{\cY}$; $q(\bs{\cC_t}(j)|\bs{\cC_p}; M_h)$ is a proposal conditional distribution for the $j_{th}$ bit of therapist hashcodes built using a classifier, like a random forest, neural network, etc.
% % 
% % 
% % 
% % \todo{explain the other terms as well.}
% % ~\cite{greg2014discovering}.
% \label{thm:mi_lb}
% % \vspace{-3mm}
% \end{theorem}
	
% % An interesting aspect of the quantity $\cT\cC(\bs{\cC}: \bs{\cY}; M_h)$ is that one can compute $\cT\cC(\bs{\cC}: \bs{\cY}; M_h)$ efficiently 
% % % if $\bs{\cY}$ is such that it maximizes the quantity, i.e., when
% % for optimized $\bs{\cY}$ that explains maximum possible Total Correlations present in $\bs{\cC}$; see \cite{greg2014discovering} for more details on the optimization.
	
% % % In this scenario, $p(\bs{c}|\bs{y}; M_h)$ factorizes, as per the \emph{Naive Bayes} model $p(\bs{c}|\bs{y}; M_h)=\prod_{j}p(\bs{c}(j)|\bs{y}; M_h)$, thus making the optimization of the quantity computationally tractable in \eqnref{eqn:corex_opt_thm}~\cite{greg2014discovering}.
	
% % % \todo{maximizing the lower bound, expecting that the actual quantity should also increase. In certain conditions, if the bound is not tight, mutual information may not increase. however, the good thing is that the lower bound itself is a good objective function, characterizing our goals for the hashing model.}

% % As we observed for the mutual information criterion above, we can also see different terms in the mutual information lower bound having varying roles for the optimization; for instance, the first two terms in \eqnref{eqn:mi_lb} contribute to improve the quality of hashcodes as representations, i.e. maximizing entropy of each hashcode bit while discouraging redundancies between the bits, and the last term of conditional entropies is for improving inference of hashcode bits individually.
	
% % % From the above discussion, we understand that it is very challenging to compute mutual information between two high dimensional variables in practice which is why we proposed a novel lower bound on the mutual information criterion as the objective function to optimize a hashing model for the dialog modeling problem. 
% % % 
% % We argue to use the proposed MI lower bound, for not only optimizing hashing for dialog modeling, but also as an \emph{evaluation metric quantifying the representation quality as well as the inference of hashcodes}. Further, for evaluating representation quality of hashcodes separately,  
% % % 
% % % the lower bound expression involves terms  which can be used for evaluating individually, (i) the inference of hashcodes, and (ii) the representation quality of hashcodes. 
% % % 
% % % \textbf{Evaluating Representation Quality of Hashcodes: 
% % % with Our Tight Upper Bound on Entropy
% % % }
% % % 
% % in \thmref{thm:entropy_ub} below,
% % we present a novel tight upper bound for joint entropy of hashcodes.
% % % 
% % on the therapist hashcodes which we propose to use as a metric for evaluating the representation quality of hashcodes.
% % ~(a surrogate to the entropy term). 
% \begin{theorem}[Upper Bound for Entropy]
% % The expression, $\sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% % -
% % \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)$, that corresponds to the first two terms in the lower bound in \thmref{thm:mi_lb},
% % % representing the quality of hashcodes, 
% % is an upper bound on the 
% % 
% Joint entropy of hashcodes, $\cH(\bs{\cC_t}; M_h)$, is upper bounded as,
% % 
% % with the gap between the bound and the entropy term itself, equal to the conditional total correlation term, $\cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)$.
% % 
% % \vspace{-2mm}
% \begin{align*}
% \cH(\bs{\cC_t}; M_h)
% \leq
% \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% -
% \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% ;
% \\
% \bs{\cY^*}
% \gets
% \mathop{\arg\max}
% \limits_{\bs{\cY}:|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t}:\bs{\cY}; M_h)
% % 
% % \vspace{-4mm}
% \end{align*}
% % 
% % \begin{proof}
% % From the definition of Total Correlation above, we have the following.
% % % 
% % \begin{align*}
% % &
% % \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% % -
% % \cT\cC(\bs{\cC_t}; M_h)
% % =
% % \cH(\bs{\cC_t}; M_h)
% % \\
% % &
% % \cT\cC(\bs{\cC_t}; M_h)
% % =
% % \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% % +
% % \cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)
% % \end{align*}
% % 
% % From these two equations above, we can easily derive the expression as below.
% % % 
% % \begin{align*}
% % &
% % \sum\limits_j{\cH(\bs{\cC_t}(j); M_h)}
% % -
% % \cT\cC(\bs{\cC_t}:\bs{\cY^*}; M_h)
% % \\
% % &=
% % \cH(\bs{\cC_t}; M_h)
% % +
% % \cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)
% % \end{align*}
% % % 
% % From this derived expression, we can simply obtain the upper bound and the corresponding gap.
% % \end{proof}
% \label{thm:entropy_ub}
% % \vspace{-4.5mm}
% \end{theorem}
% % 
% % Note the similarities between the expressions for proposed the mutual information lower bound, and the joint entropy upper bound; the first two terms match between the two expressions.
% % % 
% % For $\cT\cC(\bs{\cC_t}|\bs{\cY^*}; M_h)=0$, i.e. when a latent representation $\bs{\cY^*}$ is learned which explains all the total correlations in $\bs{\cC_t}$, the upper bound becomes equal to the entropy term; practically, for the case of hashcodes, learning such a representation should not be too difficult, so the bound should be very tight. This is quite interesting as we are able to judge the representation quality of hashcodes, that we proposed to quantify via the entropy of hashcodes in the above, through the tight upper bound in \thmref{thm:entropy_ub} which is much easier and cheap/accurate to compute than the entropy term itself. Besides the mutual information lower bound, for more detailed analysis, \emph{we propose to use the upper bound as an evaluation metric} for the dialog problem when modeling via hashing functions. 

% % % It is important to 
% % % Note that 
% % The proposed information theoretic bounds are generically applicable for any high dimensional variables.
% % % , beyond the domains of hashcodes, NLP, psychiatry which we considered in this paper.

% % See supplementary material for derivation of the bounds. Next, in  \secref{sec:opt_hash_details}, we discuss details on how to optimize a kernel- or neural-hashing, as per \algoref{alg:our_algo_klsh_codes}, by maximizing the MI LB.
% % \vspace{-2mm}
% 
% 
% 
\section{Derivations of the Information Theoretic Bounds
% LB and Entropy UB
% Derivation
}
\label{sec:bounds_deriv}
% \vspace{-2mm}
% 
Before the discussion of our novel lower bound of mutual information, we introduce the information-theoretic quantity called \textit{Total Correlation}~($\mathcal{TC}$), which captures non-linear correlation among the dimensions of a random variable $\bs{C}$, i.e., 
% 
% \vspace{-2mm}
\begin{align}
&
\cT\cC(\bs{C}) = \sum\limits_j \cH(C_j) - \cH(\bs{C});
\vspace{-4mm}
\end{align}
% 		
For a 2-D random variable, total correlation corresponds to mutual information quantity itself. 
And, $\cT\cC(\bs{C}: \bs{Y})$ is defined as,
% 
\vspace{-3mm}
\begin{align}
\nonumber
\\
&
\cT\cC(\bs{C}: \bs{Y}) = \cT\cC(\bs{C}) - \cT\cC(\bs{C}|\bs{Y}).
\label{eqn:corex}
% \vspace{-4mm}
\end{align}
% 
Intuitively, \eqnref{eqn:corex} describes the amount of information within $\bs{C}$ that can be explained by $\bs{Y}$.
% 
% The interesting aspect of this quantity $\cT\cC(\bs{\cX}: \bs{\cY}; M_h)$ is that one can compute $\cT\cC(\bs{\cX}: \bs{\cY}; M_h)$ efficiently for $\bs{\cY}$ is such that it maximizes the quantity, i.e., when $\bs{\cY}$ explains all the correlations present in $\bs{\cX}$. In this scenario, $p(\bs{x}|\bs{y}; M_h)$ factorizes, as per the \emph{Naive Bayes} model $p(\bs{x}|\bs{y}; M_h)=\prod_{j}p(\bs{x}(j)|\bs{y}; M_h)$, thus making the computations cheap~\cite{greg2014discovering}. 

Along these lines, the mutual information quantity between the hashcodes can be decomposed as in \lmaref{lma:mi_decompose} below.
% 	
% \vspace{-1mm}
\begin{lemma}[Mutual Information Decomposition]
\label{lma:mi_decompose}
Mutual Information between $\bs{C^t}$ and $\bs{C^p}$ is decomposed as follows:
% 
% \vspace{-3mm}
\begin{align}
&
\cI(\bs{C^t}: \bs{C^p})
% \nonumber
% \\
% &
% = \cH(\bs{\cC_t}; M_h) - \cH(\bs{\cC_t} | \bs{\cC_p}; M_h)
% 
% \nonumber\\
% &= \sum\limits_i {\cH(\bs{\cC_t}(i))}-\sum\limits_i {\cH(\bs{\cC_t}(i) | \bs{\cC_p})} \nonumber \\
% &~~~~
% + \cH(\bs{\cC_t}) - \cH(\bs{\cC_t} | \bs{\cC_p}) \nonumber \\
% &~~~~
% - \sum\limits_i {\cH(\bs{\cC_t}(i))}
% +
% \sum\limits_i {\cH(\bs{\cC_t}(i) | \bs{\cC_p})} \nonumber \\
% &
% = \sum\limits_i {\cI(\bs{\cC_t}(i): \bs{\cC_p})} - (\cT\cC(\bs{\cC_t}) - \cT\cC(\bs{\cC_t}|\bs{\cC_p})) 
\nonumber 
\\
&
= \sum\limits_j {\cI(C^t_j: \bs{C^p})} -
\cT\cC(
\bs{C^t}: \bs{C^p}).
\label{eqn:deco_mi}
% \vspace{-3mm}
\end{align}
% \vspace{-4.5mm}
\begin{proof}
\begin{align*}
\cI(\bs{C^t}: \bs{C^p})
&
= \cH(\bs{C^t}) - \cH(\bs{C^t} | \bs{C^p})
\nonumber \\
&
= 
\sum\limits_j
\cH(C^t_j) 
- 
\sum\limits_j
\cH(C^t_j | \bs{C^p})
+ \cH(\bs{C^t}) 
\nonumber \\
&
- \cH(\bs{C^t} | \bs{C^p})
- \sum\limits_j {\cH(C^t_j)}
+
\sum\limits_i {\cH(C^t_i | \bs{C^p})} \nonumber \\
&
= \sum\limits_j {\cI(C^t_j: \bs{C^p})} - (\cT\cC(\bs{C^t}) - \cT\cC(\bs{C^t}|\bs{C^p}))
\nonumber 
\\
&
= \sum\limits_j {\cI(C^t_j: \bs{C^p})} -
\cT\cC(
\bs{C^t}: \bs{C^p}).
\end{align*}
\end{proof}
\end{lemma}
% 	
% \noindent wherein $\bs{\cC_t}(j)$ denotes the $j_{th}$ dimension of $\bs{\cC_t}$ in \eqnref{eqn:deco_mi}.
% 		
Looking at the first term of RHS in \eqnref{eqn:deco_mi}, it is the mutual information between a one-dimensional and multi-dimensional random variable. 

For these terms, since one of the variables is only 1-D, we can use the existing technique of variational bounds for an approximation, as in \lmaref{lma:variational_lb_mi} below.
% 					
% \vspace{-1.0mm}
\begin{lemma}
\label{lma:variational_lb_mi}
Marginal mutual information for each bit in therapist hashcodes, $\cI(C^t_j: \bs{C^p})$, is lower bounded as,
% 
% \vspace{-3mm}
\begin{align}
% &
\cI(C^t_j: \bs{C^p}) 
\ge 
% \nonumber
% \\
% &
\cH(C^t_j)
+
\left\langle \log q(C^t_j|\bs{C^p})
\right\rangle_{p(C^t_j,\bs{C^p})}.
\label{eqn:vmi}
% \vspace{-3mm}
\end{align}
% 
% \todo{mention, we simply use a variational upper bound on the marginal conditional entropy term. Mention the bound gap.}
% 
\label{lma:marginal_mi_lb}
% \vspace{-5.5mm}
\end{lemma}
% 	
\noindent Herein, $\cH(C^t_j)$ is easy to compute because $C^t_j$ is a one-dimensional binary variable. For each of the proposal distributions $q(C^t_j|\bs{C_p})$, we propose to use a Random Forest~(RF) classifier~\cite{gao2016variational}.
            		
In reference to the second term of RHS in \eqnref{eqn:deco_mi}, 
% as mentioned above, 
it is computationally intractable to compute the total correlation expression $\cT\cC(\bs{C^t}:\bs{C^p})$, which denotes the total correlations between bits of $\bs{C^t}$, explainable by $\bs{C^p}$. So, we would also like to obtain an upper bound of $\cT\cC(\bs{C^t}:\bs{C^p})$, which is cheap to compute, that would give us a lower bound for the second term in \eqnref{eqn:deco_mi} because of the negative sign.
% 		
\begin{lemma}
$\cT\cC(\bs{C^t}:\bs{C^p})$ is upper bounded as: 
% \vspace{-2mm}
\begin{align}
\cT\cC(\bs{C^t}:\bs{C^p})
\leq
\cT\cC(\bs{C^t}:\bs{Y^*})
\label{eqn:corex_lb}
% \vspace{-4mm}
\end{align}
% 	
% \begin{align}
% \bs{\cY^*}
% \gets
% \mathop{\arg\max}
% \limits_{\bs{\cY}:|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t}:\bs{\cY}; M_h),
% \label{eqn:corex_opt}
% \end{align}
% 	
% To obtain the upper bound, we aim to solve the optimization problem in \eqnref{eqn:corex_opt} and obtain,
% 	
% 				
\noindent wherein $|.|$ denotes the dimensionality of a random variable.
% in \eqnref{eqn:corex_lb}. 
\label{lma:tc_ub}
% \vspace{-4mm}
\end{lemma}
% 		
% As mentioned previously, 
Although it is intractable to compute the original term $\cT\cC(\bs{C^t}:\bs{C^p})$, it is possible to compute $\cT\cC(\bs{C^t}:\bs{Y^*})$ for a latent variable representation $\bs{Y^*}$ of $\bs{C^t}$ that maximally explains the Total Correlations in $\bs{C^t}$.
% ~\eqnref{eqn:corex_opt}.

% 	
% We discuss more details on obtaining such latent representation in the following.
% 
% 	
We can think of the computation of the upper bound as an unsupervised learning problem. We propose to use an existing algorithm, \emph{CorEx}, for the unsupervised learning of latent random variables representation $\bs{Y^*}$~\cite{greg2014discovering}.
	
% \begin{align}
% \cI(\bs{\cC_t}: \bs{\cC_p}) \ge \sum\limits_i{\cH(\bs{\cC_t}(i)) + \left\langle \log q(\bs{\cC_t}(i)|\bs{\cC_p})\right\rangle_{p(\bs{\cC_t}(i),\bs{\cC_p})}} 
% \\
% - \mathop{\max }\limits_{|\bs{\cY}|=|\bs{\cC_p}|} \cT\cC(\bs{\cC_t};\bs{\cY})
% \label{eqn:mi_lb}
% \end{align}

% We can view the last term of RHS in Eq.~\ref{eqn:mi_lb} 
		
It is important to note some practical considerations about the upper bound. In the case of a suboptimal solution to the maximization of $\cT\cC(\bs{C^t}:\bs{Y})$ above, the optimized quantity may not be an upper bound of $\cT\cC(\bs{C^t}:\bs{C^p})$, but rather an approximation. Also, the upper bound would not be tight if $\bs{C^p}$ doesn't explain much of total correlations in $\bs{C^t}$. Further, for even more computation cost reductions during the learning, the dimension of the latent representation $\bs{Y}$ can be kept much smaller than the dimension of hashcodes, i.e. $|\bs{Y}| \ll |\bs{C^p}|$ for $|\bs{C^p}| \gg 1$; this is because even a small number of latent variables should explain most of the total correlations for practical purposes as demonstrated by \cite{greg2014discovering}, and observed in our experiments on hashcodes as well.
		
% \todo{we can keep size of $\cY$ small as many of the remaining latent variables would contribute very low value.}
	
Combining \eqnref{eqn:vmi} and \eqnref{eqn:corex_lb} into \eqnref{eqn:deco_mi}, we get the lower bound in \thmref{thm:mi_lb}.
		    
% \input{theorem_milb.tex}

Along same lines, we can derive the tight upper bound on joint entropy of hashcodes so as to obtain the normalization of the MI LB.
% 
From the definition of Total Correlation above~\eqnref{eqn:corex}, we have the following,
% 
% \vspace{-2.5mm}
\begin{align*}
&
\sum\limits_j{\cH(C^t_j)}
-
\cT\cC(\bs{C^t})
=
\cH(\bs{C^t}),
\\
&
\cT\cC(\bs{C^t})
=
\cT\cC(\bs{C^t}:\bs{Y^*})
+
\cT\cC(\bs{C^t}|\bs{Y^*}),
% \vspace{-4mm}
\end{align*}
% 
and finally the expression below.
% 
% \vspace{-3mm}
\begin{align*}
&
\sum\limits_j{\cH(C^t_j)}
-
\cT\cC(\bs{C^t}:\bs{Y^*})
\\
&=
\cH(\bs{C^t})
+
\cT\cC(\bs{C^t}|\bs{Y^*})
% \vspace{-3mm}
\end{align*}
% 
From this derived expression, we can simply obtain the upper bound and the corresponding gap.
        
\textbf{Previous Lower Bounds for Mutual Information: 
% outside Dialog Modeling Settings
}
Variational lower bounds on the mutual information criterion have been proposed in the past ~\cite{barber2003algorithm,chalk2016relevant,gao2016variational,chen2016infogan,alemi2017deep,garg2018efficient}.
% for settings where one of the two variables is fixed~(say class labels).
% 
% In these settings, for the mutual information lower bound, one needs to only obtain a variational upper bound on the conditional entropy term, while ignoring the entropy term as a constant. This simplifies the derivation significantly, compared to our setting. In our setting, we can not ignore the entropy term as it is a variable. 
% 
% % The idea of variational lower bound for our mutual information objective would not work as such, since neither of the two high-dimensional variables is fixed, but instead functionals of the hashing model, as we explain in the following.
% % ; we will now describe  the computation of the variational lower bound.
% % 
% % 
% % 
% % 	
% % The mutual information  is expressed in terms of the entropy of $\bs{\cC_t}$, and the conditional  entropy of $\bs{\cC_t}$ given the hash codes of patients $\bs{\cC_p}$. 
% For high-dimensional hashcodes, computing $p(\bs{\cC_t}|\bs{\cC_p}; M_h)$ is intractable, and so the computing the conditional entropy term, $\cH(\bs{\cC_t}|\bs{\cC_p}; M_h)$. However, one can use instead a \emph{proposal distribution}, $q(\bs{\cC_t}|\bs{\cC_p}; M_h)$, approximating  $p(\bs{\cC_t}|\bs{\cC_p}; M_h)$, that is cheaper to compute. This leads to the variational lower bound, with tightness of the bound depending upon KL-divergence between the proposal distribution and the true conditional distribution.
% % 
% \begin{align*}
% &
% \cI(\bs{\cC_t}: \bs{\cC_p}; M_h) = \cH(\bs{\cC_t}; M_h) - \cH(\bs{\cC_t} | \bs{\cC_p}; M_h)
% \\
% &
% = \cH(\bs{\cC_t}; M_h) + \left\langle \log p(\bs{\cC_t}|\bs{\cC_p}; M_h)\right\rangle_{p(\bs{\cC_t},\bs{\cC_p}; M_h)}
% \\
% &
% % \cI(\bs{\cC_t}: \bs{\cC_p}; M_h) 
% \geq 
% \cH(\bs{\cC_t}; M_h) 
% + 
% \left\langle \log q(\bs{\cC_t}|\bs{\cC_p}; M_h)
% \right\rangle_{p(\bs{\cC_t},\bs{\cC_p}; M_h)}
% \end{align*}
% 
% 
Their lower bounds works only when one of the variables is fixed, say if $\bs{C^t}$ were fixed. In our objective, not only $\bs{C^t}$ is a functional of the hashing model that we are learning, it is high dimensional. Unless we have a lower bound for the entropy term $\cH(\bs{C^t})$ as well, which should be hard to obtain, we can not use the above mentioned variational lower bounds for our problem as such.
% 
% However, if we apply the variational lower bound directly, the entropy term $\cH(\bs{\cC_t})$ involves high-dimensional variables and is not easy to compute. 
Besides, it is also non-trivial to find an appropriate proposal distribution $q(\bs{C^t}|\bs{C^p})$. Therefore, we adopt a different approach for obtaining a novel lower bound on the mutual information quantity, as described above.

\section{Pseudo Code of Algorithms To Optimize LSH for Dialog Modeling}
% 

In the following, we discuss the optimization of the reference set.
		
{ \bf Optimizing Reference Set. \\}
% 	
\begin{algorithm*}[th]
\caption{
% \small
\csizenine
Optimizing Reference Set in LSH-RkNN or LSH-RMM for Dialogue Modeling 
% by Maximizing Our MI LB
}
% \scriptsize
% \csize
% \small
\csizenine
% 
\begin{algorithmic}[1]
\REQUIRE Training set $\bar{\bs{S}} = \{\bs{S}^p,\bs{S}^t\}$; initial and final size of reference set, $I$ and $M$ respectively; $\beta$ and $\gamma$ are the number of samples, as candidates for the reference set, and for computing the lower bound, respectively.
% \\
% \STATE $\bar{\bs{S}} = \{ S_1^p, \cdots, S_N^p, S_1^t, \cdots, S_N^t \}$
% \COMMENT{patient \& therapist responses in same set as candidates for the reference set}
% % 
% \\
% \STATE $\bs{S}^p = \{ S_1^p, \cdots, S_N^p \}$
% \COMMENT{patient responses}
% % 
% \\
% \STATE $\bs{S}^t = \{ S_1^t, \cdots, S_N^t \}$
% \COMMENT{therapist responses}
% 
\\
\STATE $\bs{r}^d$ $\gets$ randomSubset($2N$, $I$)
\COMMENT{random subset of indices, of size $I$, from $\{ 1, \cdots, 2N \}$ for initialization of reference set}
\\
\COMMENT{optimizing the reference set up to size $M$ greedily}
\FOR{$j=1 \to M$}
% 
% \\
% \COMMENT{Optimize $j^{th}$ element in the reference set}
% 
\IF{$j > I$}
\STATE $\bs{r}^d \gets \{ \bs{r}^d, randomSubset($2N$, 1) \}$
\COMMENT{adding one more element in the reference set, that is to be optimized}
\ENDIF
% 
\STATE $\bs{r}^{ref}$ $\gets$ randomSubset($2N$, $\beta$)\COMMENT{subset of the structures as candidates for the reference set}
% 
\STATE $\bs{r}^{lb}$ $\gets$ randomSubset($N$, $\gamma$)\COMMENT{subset of patient/therapist responses pairs for computing the MI lower bound}
% 
\STATE $\bs{K}^p \gets$ computeKernel($\bs{S}^p(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{d})$)
\COMMENT{$\gamma \!\!\times\!\! j$ size}
% 
\STATE $\bs{K}^t \gets$ computeKernel($\bs{S}^t(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{d})$)
\COMMENT{$\gamma \!\!\times\!\! j$ size}
% 
\STATE $\bar{\bs{K}}^p \gets$ computeKernel($\bs{S}^p(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{ref})$)
\COMMENT{$\gamma \!\!\times\!\! \beta$ size}
% 
\STATE $\bar{\bs{K}}^t \gets$ computeKernel($\bs{S}^t(\bs{r}^{lb})$, $\bar{\bs{S}}(\bs{r}^{ref})$)
\COMMENT{$\gamma \!\!\times\!\! \beta$ size}
% 
% \STATE $\bs{mi}_{lb}$ $\gets$ $\bs{0}$
% 
\STATE $\bs{mi}_{lb}$ $\gets$ computeMILowerBound($\bs{K}^p, \bs{K}^t, \bar{\bs{K}}^p, \bar{\bs{K}}^t$)
\COMMENT{compute the MI lower bound for all the candidates $\bar{\bs{S}}(\bs{r}^{ref})$, using the kernel matrices, via computation of hashcodes}
% 
% \FOR{$l=1 \to \beta$}
% 
% \STATE $\bs{C}^p \gets$ computeKernelHashcodes($\bs{K}^p$)
% 
% \STATE $\bs{C}^t \gets$ computeKernelHashcodes($\bs{K}^t$)
% 
% \STATE $\bs{mi}_{lb}(l)$ $\gets$ computeMILowerBound($\bs{S}(\bs{r}^{lb})$)
% 
% \ENDFOR
% 
\STATE $\bs{r}^{d}(j)$ $\gets$ maxMILBDataIndex($\bs{mi}_{lb}$, $\bs{r}^{ref}$)
\COMMENT{choose the index with maximum value of MI lower bound, from the set of candidate indices $\bs{r}^{ref}$}
% 
\ENDFOR
% 
\RETURN $\bar{\bs{S}}(\bs{r}^d)$
% 
\end{algorithmic}
\label{alg:opt_ref}
\end{algorithm*}
% 
For hashing models LSH-RkNN and LSH-RMM described in the main paper, we can optimize the reference set, $\bs{S}^R$, for dialog modeling as described in the following.
 
For the selection of elements in $\bs{S}^R$, we use a greedy algorithm maximizing the proposed mutual information lower bound~(in \thmref{thm:mi_lb}); see the pseudo code in \algoref{alg:opt_ref}. We initialize a reference set of small size $I \ll M$, by randomly selecting responses from the training set of patient/therapist responses, i.e. $\bar{\bs{S}} = \{ S_1^p, \cdots, S_N^p, S_1^t, \cdots, S_N^t \}$; though, as noted before, the superset $\bar{\bs{S}}$ for the random selection can be any set of sentences/paragraphs, not necessarily coming from a dataset of patient/therapist responses. First, each element in the initial reference set is optimized greedily, and then more elements are added one by one until the reference set size grows to $M$. When optimizing each element in the set, for computing the MI lower bound, we sample $\gamma$ number of response pairs from the training set of patient/therapist responses pairs, $\{ (S_i^p, S_i^t) \}_{i=1}^N$. For computational efficiency, we adopt the idea of sampling for the candidate set as well, in each greedy optimization step, by sampling a subset of candidates of size $\beta$ from the set $\bar{\bs{S}}$.
	
% 	
The computation cost in the optimization is dominated by the number convolution kernel similarities, i.e. $O(\gamma(M^2+M\beta))$. In practice, we can keep low values of $\gamma$ as well as $\beta$; in our experiments, we use $\beta=1000, \gamma=100$, and vary the value of $M$ from $30$ upto $300$. A similar procedure can be used to optimize kernel parameters. 

	 	
{\bf Optimizing Neural Network Architecture. \\}
% 
% \input{algoNNPseudoCode.tex}
\begin{algorithm*}[tp!]
\caption{
% \small
\csizenine
Optimizing Neural Architecture in LSH-RLSTM for Dialog Modeling
% Neural-Hashing Model for Dialogue Modeling by Maximizing Our MI LB   - {\bf TODO Shorten the title}
}
% 
\csizenine
% 
\begin{algorithmic}[1]
\REQUIRE Training dataset $\{\bs{S}^p$, $\bs{S}^t\}$, with $N$ pairs; maximum number of layers in neural language models, $L$; the number of samples for computing the MI lower bound, $\gamma$; values for units in a layer, $\bs{u} =$ \{4, 8, 16, 32, 64, None\}. 
% \\
% \STATE $\bar{\bs{S}} = \{ S_1^p, \cdots, S_N^p, S_1^t, \cdots, S_N^t \}$
% \COMMENT{patient \& therapist responses in same set as the reference set}
% % 
% \\
% \STATE $\bs{S}^p = \{ S_1^p, \cdots, S_N^p \}$
% \COMMENT{patient responses}
% % 
% \\
% \STATE $\bs{S}^t = \{ S_1^t, \cdots, S_N^t \}$
% \COMMENT{therapist responses}
% 
% \STATE $\bs{r}^d$ $\gets$ randomSubset($2N$, $I$)
% \COMMENT{random subset of indices, of size $I$, from $\{ 1, \cdots, 2N \}$ for initialization of reference set}
% \\
% \STATE $NN \gets [10, None]$\COMMENT{initialization of neural network with 10 units in the first layer}
% 
% \STATE $NU \gets \{10, 20, 40, 80, None\}$\COMMENT{choices for number of units 
% in a layer
% }
\\
\COMMENT{optimizing up to $L$ layers greedily}
\FOR{$j=1 \to L$}
% 
% 
\STATE $\bs{r}^{lb}$ $\gets$ randomSubset($N$, $\gamma$)\COMMENT{subset of patient/therapist responses pairs for computing the MI LB to optimize $j_{th}$ layer}
% \\
% 
% 
\COMMENT{Number of units in $j_{th}$ layer, None not applicable for $1_{st}$ layer}
\FOR{$l \in \bs{u}$}
% 
\STATE $\bs{n}(j) \gets l$\COMMENT{$l$ units in $j_{th}$ layer of neural network}
% 
\STATE $\bs{C}^p \gets$ computeHashcodes($\bs{S}^p(\bs{r}^{lb}), \bs{n}$)
% 
\STATE $\bs{C}^t \gets$ computeHashcodes($\bs{S}^t(\bs{r}^{lb}), \bs{n}$)
% 
\STATE $\bs{mi}_{lb}(l)$ $\gets$ computeMILowerBound($\bs{C}^p, \bs{C}^t$)
% 
% \STATE $\bs{mi}_{lb}$ $\gets$ computeMILowerBound($\bs{K}^p, \bs{K}^t, \bar{\bs{K}}^p, \bar{\bs{K}}^t$)
% \COMMENT{compute the MI lower bound for all the candidates $\bar{\bs{S}}(\bs{r}^{ref})$, using the kernel matrices, via computation of hashcodes}
% 
\ENDFOR
% 
\STATE $\bs{n}(j)$ $\gets$ maxMILBIndex($\bs{mi}_{lb}$, $\bs{u}$)
\COMMENT{choose the units with maximum value of MI LB}
% 
\STATE \textbf{if} $\bs{n}(j)$ is None \textbf{then} break out of loop \textbf{end if}
% 
\ENDFOR
% 
\RETURN $\bs{n}$
% 
\end{algorithmic}
\label{alg:opt_nn_layers}
\end{algorithm*}

% 
For neural networks based LSH~(LSH-RLSTM), we can optimize the number of layers and the units in each layer, by maximizing the proposed MI LB; see pseudo code in \algoref{alg:opt_nn_layers}. 

\section{Experimental Details on LSH Models}
% 
LSTM models for each hash function in \emph{LSH-RLSTM}  are  trained using Adam~\cite{kingma2014adam}, with the learning rate $1e-3$, amsgrad=True, and $l_1$, $l_2$ regularization coefficients set to   $1e-4$.  We initialize a word in a response and its POS tag with a random  vector of size 30; for a single time step processing with in LSTM, word vectors of 10 adjacent words, along with their POS tags, are appended into a vector of size 600; this is required to avoid vanishing gradients since patient responses can be of length up to 8,000 words in the training dataset. For the $H$ number of LSTM models as neural-hash functions, same neural architecture, i.e., same number of layers and units, are used in each model. When optimizing the architecture of the LSTM models with \algoref{alg:opt_nn_layers} by maximizing our proposed MI LB~(\emph{MI LB Optimal}), we add layers one by one greedily up to maximum possible 5 layers~($L=4, \gamma=1000$), and try out different possible numbers of normal units in each layer, i.e., 4, 8, 16, 32, 64. (We keep the number of units small, since $\alpha$ is small. Also, during the optimization, we use $H=30$). When optimizing the Reference set with \algoref{alg:opt_ref}, we keep $\beta=1000, \gamma=100, I=20$.

{\em Similarity metric}. In case of \emph{kernel-hashing}, we use subsequence kernels~\cite{mooney2005subsequence} for computing similarity between two responses (subsequences of length up to 16 are matched), while similarity between a pair of words is computed as cosine between their word vector representations.

\subsection{Subsequence Kernel}
% 
Let $S_i$ and $S_j$ be two sequences of tokens~(words), the convolution kernel similarity between $S_i$ and $S_j$ is defined as below~\cite{mooney2005subsequence}.
            
\begin{align*}
\csizeten
K(S_i, S_j)
=
\sum_{e=1}^{16}
\sum_{\boldsymbol{i}, \boldsymbol{j}: |\boldsymbol{i}|=|\boldsymbol{j}|=e}
\prod_{k=1}^{|\boldsymbol{i}|}
k(S_i(\bs{i}_k), S_j(\bs{j}_k))
\lambda^{l(\boldsymbol{i})+l(\boldsymbol{j})}.
\end{align*}

Here, $k(S_i(\bs{i}_k), S_j(\bs{j}_k))$ is the similarity between the $k_{th}$ tokens in the subsequences $\boldsymbol{i}$ and $\boldsymbol{j}$, of equal length~(up to value 16); $l(.)$ is the actual length of a subsequence in the corresponding sequence, i.e., the difference between the end index and start index~(subsequences do not have to be contiguous); $\lambda \in (0, 1)$ is used to penalize the long subsequences. Dynamic programming is used for efficient computation of the subsequence kernel.
    
We use the following expression for computing the kernel similarity, $k(a,b)$, between two tokens $a$ and $b$ using their respective word vector representations~(real valued column vectors), $\bs{w}_a$ and $\bs{w}_b$.
            
\begin{align}
k(a, b)
=
cs
\left(
1-
\frac{(1-cs)}{(1-\zeta)}
\right)_{+};
\ \ \ 
cs = \frac{\bs{w}_a^T \bs{w}_b}{||\bs{w}_a||_2||\bs{w}_b||_2},
\end{align}

Herein, $cs$ is cosine similarity between the two word vectors, $\bs{w}_a$ and $\bs{w}_b$; $()_{+}$ represents the positive part function; $\zeta \in [-1,1]$ is a parameter for \emph{compact support} of the kernel function.

The parameters $\lambda, \zeta$ are optimized by maximizing the proposed MI LB criterion in our dialog model.

\section{Additional Experiment Details}

\begin{table*}[tp!]
\centering
\tabsize
\begin{tabular}{p{16.75cm}}
\toprule
% 
\patient{I did lose three pounds, did you notice that?}
\\
\therapist{That's great, I did notice that.}
\\
\rmm{Yes, you did.}
% {\bf RMM:} Yes, you did.
\\
\rknn{To help you with your diet?}
\\
\rlstm{Okay what's the explanation?}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of the way
\\
{\bf HRED:} Yeah. you
\\
{\bf VHRED:} Uh-huh. you
\\
% 
% 
% 
\toprule
% 
\patient{Well, first of all, we've never been able to, when I first come to see you in July you highly recommended and I refused to go into this day treatment or some type of a hospital and I refused and you put me on medicine. And the medicine helped a great, great deal. I have been to 4 different psychiatrists and they've put me on Lithium and they've done other things and none of that stuff worked. And when I come to see you I was real skeptic but I was reaching out for help.}
\\
\therapist{Um-hum.}
\\
\rmm{I see.}
\\
\rknn{It does?}
\\
\rlstm{You mean its puzzling why? I suppose it's very depressing too.}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of the way
\\
{\bf HRED:} Okay. you
\\
{\bf VHRED:} Uh-huh.
\\
% 
% 
% 
\toprule
% 
% 
\patient{Which is stupid because like, ya know, (sniffles) I guess if it's not what they like, then it's not what they like and they can like do something else, but like (sniffles) ya know there's some psychiatrists who charge like \$300 an hour. If you did that you would really have to work like...if you worked an hour a day five days a week that would be fifteen hundred dollars a week. Like...you wouldn't have to work at all...like barely. I mean, though, most psychiatrists probably don't charge \$300 an hour...yeah...it's just kinda ridiculous that...}
\\
\therapist{I'm sorry you're having such trouble getting...getting access to the care that you need (pause).}
\\
\rmm{You got to do.}
\\
\rknn{Oh yeah, you never tried Lithium?}
\\
\rlstm{And you ought not to just shove it away out of your life because you will need it again.}
\\
{\bf LSTM:} Uh-huh. you
\\
{\bf HRED:} Yeah. you
\\
{\bf VHRED:}  Uh-huh. you
\\
% 
% 
% 
\toprule
% 
% 
% 
% 
\patient{I don't... I guess that's the problem right now. I guess that's what I'm grappling with. I guess that's what I'm amazed about. I think, you know, the hypothesis that you just presented about what I'm doing probing, you know, fucking you over, you know, all of these things (PAUSE) it's plausible to me. And that's freaky because my experience of it is just, you know, just being pinned to the wall.}
\\
\therapist{Right. So... (PAUSE) Maybe the (PAUSE) sort of... (PAUSE) If I think about the sort of world that that one part is living in, the sort of fucking me over part, I imagine it's a world where that goes both ways, where you can be coming here for months and months and trying and not getting anywhere with this. And, you know, getting up and doing your part and paying money sort of or, you know, you know what I mean. And, you know, and still get nothing. Which is how you felt at some moments recently.}
\\
\rmm{Could be.}
\\
\rknn{Because nobody's helping you.}
\\
\rlstm{The thing, the thing I'm trying to get a feel for is what happened that was good? What happened?}
\\
{\bf LSTM:} Okay, you
\\
{\bf HRED:} M-hmm. you
\\
{\bf VHRED:} Okay, you
\\
% 
% 
% 
\toprule
% 
% 
% 
\patient{Yeah. I mean, it'll start, yknow, like right now, I mean, you're familiar with the weather patterns and things like that. It's not getting, I mean, the light is going to start to diminish, but the cold and having to be stuck in the house and everything all day isn't going to start for another month. Yknow, I'm still fine right now. Um, would you want me to call you then when I was going to start to take the 200 to let you know the beginning of it?}
\\
\therapist{Yeah, of course. Of course, you could do that.}
\\
\rmm{Yeah you probably could.}
\\
\rknn{So you get a little.}
\\
\rlstm{Right? And so just something to think about. It doesn't mean that it has to happen that way, but it can. And so the times where I may think that applies, I may bring it up. Because it's about relating your past relationships to your present relationships. And even how you relate in here with me. And so we may talk about that at some point.}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot
\\
{\bf HRED:} Yeah. you
\\
{\bf VHRED:} Okay. you
\\
% 
% 
% 
\toprule
% 
% 
% 
\patient{The fact that I wanted to do things that he didn't and then he felt guilty and I was like, \"Well, I mean it's not your fault because you're depressed and disappointed, too, and couldn't not be disappointed and stuff, too. Instead just focus on cuddling.}
\\
\therapist{That's not satisfying for you.}
\\
\rmm{Such as?}
\\
\rknn{Yeah.}
\\
\rlstm{One more thing, you just don't look at them enough.}
\\
{\bf LSTM:} Uh-huh. you
\\
{\bf HRED:} M-hmm. you
\\
{\bf VHRED:} Uh-huh. you
\\
% 
% 
\toprule
% 
% 
% 
% 
\patient{ Well I guess because there's truth to it when you go (ph), \"Okay, well what are you avoiding?\" in essence. I mean, there's truth to that. Because I ... because working in here, I agree, that's a thing I want to do is be focused on how I'm feeling. This whole thing with my family not being able to show feelings. By the way, I just have to drive over this scenic outlook and tell you that I, you know, I did talk to my mother about ...}
\\
\therapist{Now why are you doing that now?}
\\
\rmm{It's up to you.}
\\
\rknn{Yeah, people get really provocative.}
\\
\rlstm{How so?}
\\
{\bf LSTM:} I don't want to be a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of the way
\\
{\bf HRED:} M-hmm. you
\\
{\bf VHRED:} Uh-huh. you
\\
% 
% 
\toprule
% 
% 
% 
% 
\patient{I hope so, I don't know what the heck that is, I don't' have any idea what that is, oh well, okay.}
\\
\therapist{Okay.}
\\
\rmm{And doing something that feels more like you.}
\\
\rknn{And you felt like that was - somehow you just couldn't do it I think.}
\\
\rlstm{You thought about that.}
\\
{\bf LSTM:} is a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of a lot of
\\
{\bf HRED:} Okay. you
\\
{\bf VHRED:} Okay, you
\\
% 
% 
\toprule
% 
\end{tabular}
\caption{
Textual responses generated by different systems for Depression Therapy dataset, along with ground truth patient and therapist responses.
}
\label{tab:gen_responses}
\end{table*}


\begin{table*}[tp!]
\centering
\csize
\begin{tabular}{p{16.75cm}}
\toprule
Yeah, here's hoping.\\
It's going to keep on being a struggle.\\
There isn't any, really anyone (ph) inside?\\
The Petition is the part that—\\
No, I don't. I really don't except that partly it's a fear of being further condemned by her. I mean, she condemns me for everything I am and everything I do.\\
So that there was again the concern with the - with [NAME].\\
Yeah. And so we didn't talk all the way home at all. And as we didn't talk, I think we were both growing angry. And so then we sat and we did talk for a long time. And that was good. Well, it was good. It was more...we talked more deeply about ourselves and our feelings than we were in the past without being angry at each other.\\
Yeah.\\
You've got your mother and sister.\\
Maybe if things are still horrible. I am hoping by next week they will be\\
When I told you that, did you remember what you felt?\\
And how to use that too.\\
You know people nearby pretty much though is you know? Also I think it's also he cannot ... he's been already like conditioned into, if he gets angry or has any ill feelings towards certain members of the family that's going to be it. Because he is no longer going be, you know ...\\
Well, that's what we're going to talk about.\\
From where?\\
I mean, you've been, I think it's great, you going every week to see [NAME OTHER], just about?\\
What's that, hon?\\
Yes.\\
Well yeah, like they didn't want their kids to be the real dummies in the neighborhood (laughter). But it's not - my father, it's not that he likes to brag on his kids if their not there. I mean he'd never say anything nice about us in front of us. But I guess it's the teachers that really bother me. I mean why get a kid an answer book. I can't - I mean, of course, I could have not cheated, but i And everything else I've done was very easy. My clarinet lessons; [I had beef cattle] (ph); I was in girl scouts. And, I mean, all I had to do was pick them out. I never had do any work. The boys always did the work, and then I went to the fair and got the purple ribbons.\\
Was it like defense-type stuff?\\
When you think of that moment in the car, how true do the words, "I can go on and thrive" feel on a 1-7 scale, with 1 being completely false and 7 being completely true?\\
I'm not seeing anybody right now.  I've got to, I've got to worry about me first.\\
I don't know. I thought of that all the time. Like how I've seen have big boxes of Kleenex usually expect the girls to cry.\\
It's easier with the groups you so about.\\
And same at your church I think.\\
Yeah.\\
Okay.\\
And with that sort of a person.  But because he is your biological father, there's a certain obligation and you are kind enough to do what has to be done.  That for you to have feelings wouldn't make much sense to me.  Of course, where, where are the feelings to come from?  The feelings would come from the acts of kindness and caring, compassion.  If they were not there, what should you feel?  But you are, nevertheless, kind enough to do the decent thing.  So, so that's one thing.  But how do you feel about that?  What I've just said?\\
I want a safe place out there.\\
No.  I had it during finals my first year of grad school and during my second year probably for like four months towards the end.\\
Yeah. I get that.\\
Okay, that's okay.\\
Once they send you the check -\\
It all seems so bad to you, it's a disillusion.\\
Yeah.\\
I said you don't want what I'm thinking on your tape.\\
So after I took one half at night, I was able to get up in the morning.\\
If I had asked you beforehand what they were going to do...?\\
You drink because you're lonely.\\
That's all right.\\
Yeah, in other words maybe I shouldn't have gotten so upset. Whereas it wasn't the most pleasant thing I should do. And like he was trying to say, you know, can't you just stay here tonight and leave tomorrow for college, see your girlfriend. And I've forgotten, it wasn't until like I just got the mail just before I came here and I was really, I didn't want to open it. It was just two Valentine's. It didn't say anything, you know, except love, Daddy and [NAME] and love, [NAME], but...\\
You went out\\
Um-hum.\\
Let's just pretend for a moment. Let's pretend that I'm your boss.\\
Okay. How old are you now?\\
Right. Well, a lot of it was like, before Christmas I was really, really snowed under with stuff and I had to work every day and I had to work late almost every day, and somehow even just the hour coming here was really a lot. Plus, I was really functioning on, 'let me just get through with work' because I had so many hours that I had to get through by Christmas or I couldn't go home for Christmas, and it was sort of, 'let me just get through that and think about things later'.\\
I was starting, you know, itching, it's almost for a month, a month and a half, I keep itching a lot over here in my face.\\
I feel like I've lost credentials and hope over...\\
Will you try out something again right now what you would find to be a response to Shelley given the fact of last week for example?\\
The rapport was good enough for that.\\

\toprule
\end{tabular}
% \vspace{-3mm}
\caption{
% \csize
We show first 50 responses~(in raw text format) that are selected greedily for the reference set~($\bs{S}^R$) in \emph{LSH-RkNN} model, out of 76,000 responses from the train set, with \algoref{alg:opt_ref}.}
\label{tab:reference_responses}
% \vspace{-1.5mm}
\end{table*}


% \input{dialogueGenerated.tex}

% \input{refSetRMM.tex}



==> tab_response_hashcodes.tex <==
\begin{table}
\centering
\tabsize
% \fontsize{8}{8}\selectfont
% \renewcommand{\arraystretch}{0.9}% Tighter
% \scriptsize
\begin{tabular}{p{7.75cm}}
\toprule
% % CLIENT: 
% But for the next person I mean. I deal with - that's part of what I do is I train people. I'm always - I'm either training people on this computer or what I like to do more is training people how to understand and train.
% And so I have - I feel bad when I give up on a trainer, you know. I just don't think she has it. It's - and I have met people who have had tremendous, tremendous abilities of being able to like grasp concepts and communicate them to others who I had more belief in, you know. [00:16:13]
% Does that make - I guess that...
% ((Crosstalk))\\
% 0101001111001011111110101101111111011011100011101100111000101011110111001001011011001110001010100100
% \\
% \\
% \thp{
% % THERAPIST: 
% For now it's just you don't - can't see like A, (inaudible at 00:16:25) a look at yourself and B, can't see her dealing well with anybody else.}\\
% \thp{
% 0101001111011011111100101101111110011011100001000100111100101000110111001001011111001110001000001000
% }
% \\
% \midrule
% % CLIENT: 
% My dad actually seems in, um, better shape health-wise than he has in a while. I was worried about him the last time I was down there, but the one thing I told him, I said, you know - we were - they had already been in town a few hours. I said, "You know, you haven't told me one story that you've already told me before." I said, "I don't know if you've changed your diet or something, but you're not as senile as you used to be." (Laughing.) [00:03:27]\\
% 0101001111001011111100101101111110011011100011000100111100101001110111001101011111011110001000000000
% \\
% \\
% \thp{
% % THERAPIST: 
% (Laughing.)
% }
% \\
% \thp{
% 0101100110111011111110111100110110101111111011110110111000101101100011101010011011001110101000100000
% }
% \\
% \midrule
% PT:	
% I'll stay on the Restoril, I mean it takes me a while to go to sleep but I'll stay on the Restoril.
% \\
% 0101001111101111111110101101011110011010100011100101111000101011110111001001011011001110001010000110
% \\
% \\
% \thp{
% % DR:	
% Let's nudge the Pamelor up a little bit.  We could also check a blood level.
% }
% \\
% \thp{
% 0111001111001011111100101100111110011010110001001100111100101101010111001011011011111110001100000000
% }

% \thp{
% 010101011010111111111010110101111001101110000110010011100010101
% % 1110111001001011011001110001010100010
% }
% \\
%\midrule
% PATIENT: 
\textit{
Its all my fault. It's like getting hit in the stomach And trying to catch your breath. You can't catch it. You struggle, move around, You just can't get your breath. That just really knocks me off balance. 
You begin to generate this feeling of a kind of negativism. And that's why it really being hurt. I never allowed myself to think negative, accept everybody else. I am the only one giving back to the "be quiet time." I had to have something to make do with that.
}
\\
010100111100101111111010110101111001101110001110110011100010100
% 1110111101011011011001110001000000000
\\
\\
\thp{
% COUNSELOR: 
\textit{
OK. Maybe that fits into the whole pattern then.
}
}\\
\thp{
01110011010010111111000111111111100010101100110011
% 00
% 11100010110
% 0010111101010011011011110001100001000
}
\\
%\midrule
% CLIENT: 
% \textit{
% Well I talked to a friend of mine whom I think is promiscuous and she told me about a man that came to see her at her apartment. So I gave him my phone number. I don't have any hang up about morals. I don't know. I told a couple of my friends about this. I must admit I'm a little shy talking about it now.
% % [0:23:27.1]
% }
% \\
% 010100011010101111111010110101111001101110000110010011100010100
% % 1110111001011011011001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% I see. You mean it's embarrassing to tell me about it.
% }
% }
% \\
% \\
% \midrule
% % PT: 
% \textit{
% Yeah.  I didn't think she was going to die.
% }
% \\
% 01010001101010111111101011000111100100111000111001
% 00111000101011110111101001011011001110001000100010\\
% \\
% \thp{
% % DR: 
% \textit{
% Yeah.
% }
% }\\
% \thp{
% 01011001101110011111101011000111111010111110011001
% 10111100101111010111101010011010101110101010100010
% }
% \\
% 
% \midrule
% CLIENT: So I filed a bug report on Wednesday.\\
% \\
% THERAPIST: Yeah.\\
% 
% \midrule
% % PATIENT: 
% \textit{
% I'm sitting here just thinking about things. Should I think out loud? (chuckles)
% }
% \\
% 01010001111010111111001111011111110010111000011001
% 00111000101011110111001101011001001110001010100010
% \\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% Sure. If you want to.
% }
% }
% \\
% \thp{
% 11010011001110111111001011011101110100111000111011
% 00111100101001110111101100011001001110001010000000}
% \\
% \midrule
% % CLIENT: 
% \textit{
% Because it's almost a year of my life.
% }
% \\
% 01010011110010111111001011010111101100101100110011
% 00111100101101110111101011011011011110001000100000\\
% \\
% \thp{
% % COUNSELOR: 
% \textit{
% All this is. It's a good chunk of time.
% }
% }\\
% \thp{
% 01010011010010111111001011010111101010101000110011
% 00111100101101110111101011011011001110001000100000
% }\\
% 
% \midrule
% % PATIENT: 
% \textit{
% Most of it is small bills. There's one 50 dollar check, and that's the only thing that's really large. The rest of it's like ten or twelve dollars each.
% }\\
% 0101001101001011111100101101111110011011110011001100111100101100110111101011011011011110001000101000\\
% \\
% \thp{
% % THERAPIST: 
% \textit{
% But it adds up.
% }
% }
% \\
% \thp{
% 0101011111101011111110111101011110001011100001100100111000101001110111101111011011001110001010100010
% }
% \\
\toprule
\end{tabular}
\vspace{-2.75mm}
\caption{
\csizenine
In this table, we show a pair of patient and therapist~(Blue) responses.
% , randomly sampled from different sessions.
% ; the responses of therapists are in red. 
For each response, we obtain a locality sensitive hashcode as its representation.
% , of 100 bits each. 
The hashcode of a patient response is used as feature representation to infer the hashcode of the corresponding therapist response.
% as multi-class labels.
}
\label{tab:therapy_session_hashcoded}
\vspace{-6mm}
\end{table}% 

